Maximizing Utilitarian and Egalitarian Welfare of Fractional Hedonic Games on Tree-like Graphs

Fractional hedonic games are coalition formation games where a player's utility is determined by the average value they assign to the members of their coalition. These games are a variation of graph hedonic games, which are a class of coalition formation games that can be succinctly represented. Due to their applicability in network clustering and their relationship to graph hedonic games, fractional hedonic games have been extensively studied from various perspectives. However, finding welfare-maximizing partitions in fractional hedonic games is a challenging task due to the nonlinearity of utilities. In fact, it has been proven to be NP-hard and can be solved in polynomial time only for a limited number of graph classes, such as trees. This paper presents (pseudo)polynomial-time algorithms to compute welfare-maximizing partitions in fractional hedonic games on tree-like graphs. We consider two types of social welfare measures: utilitarian and egalitarian. Tree-like graphs refer to graphs with bounded treewidth and block graphs. A hardness result is provided, demonstrating that the pseudopolynomial-time solvability is the best possible under the assumption P$\neq$NP.

==> chapter03.tex <==
\section{Block split graphs}
%この章では，スプリットグラフをさらに限定したグラフクラスであるブロックスプリットグラフにおけるPoSについて，ペンダント点を持たないクリーク内の頂点数$z$に着目して，新たな上界を与える．
In this section, we give a new upper bound for PoS on block split graphs. To show this, we focus on the number of vertices in the clique which are not adjacent to any pendant vertices.

\subsection{Characterization of a social optimum}\label{subsection:opt:blocksplit}
%本節では，社会効用最大提携構造の総効用を見積もるために，ブロックスプリットグラフにおける社会効用最大提携構造の特徴付けを行う．ブロックスプリットグラフにおける社会効用最大提携構造について，次の補題が成り立つ．
In this subsection, we characterize a social optimum on a block split graph in order to estimate the social welfare of the social optimum. 
Let $G=(K\cup I,E)$ be a block split graph whose vertex set can be partitioned to a clique $K$ and an independent set $I$. 
%The following Lemma holds for the social optimum on a block split graph.

\begin{lemma}\label{lem1}
%クリーク内の頂点を3つ以上含む提携を$C$とする．$C$がペンダント点を含むとすると，社会効用を減らすことなくクリーク部分とペンダント点部分に分割することができる．
Let $C$ be a coalition containing at least three vertices in $K$. If $C$ contains pendant vertices, it can be partitioned into a coalition which induces a clique and a coalition which induces pendant vertices without reducing social welfare.
\end{lemma}

\begin{proof}
%提携構造$\C$において，クリーク内の頂点を3つ以上含み，かつ隣接するペンダント点を1つ以上含む提携を$C$とする．提携$C$において，クリークに含まれる頂点数を$x\ (\ge 3)$，ペンダント点の数を$y\ (\ge 1)$とする．このとき，$\sw(C)=\left(2\binom{x}{2}+2y\right)/(x+y)$である．一方，提携$C$をクリーク部分$C_1$とペンダント点部分$C_2$に分割した提携構造$\C'=\C\setminus \{C\}\cup (\{C_1\}\cup \{C_2\})$を考える．すると，$\sw(\C')-\sw(\C)=\sw(C_1)+\sw(C_2)-\sw(C)$となる．提携$C_2$はペンダント点のみからなる集合であり，孤立点集合となるので$\sw(C_2)=0$である．また，$C_1$はクリークなので，$\sw(C_1)=2\binom{x}{2}/x$である．よって，$x\ge 3, y\ge 1$であることに注意すると，
Let $C$ be a coalition in the coalition structure $\C$ that contains at least three vertices in clique $K$ and at least one adjacent pendant vertex. Let $x\ (\ge 3)$ be the number of vertices in $C \cap K$ and $y\ (\ge 1)$ be the number of pendant vertices in $C$. 
Then, the social welfare of $C$ is $\sw(C)=\left(2\binom{x}{2}+2y\right)/(x+y)$. 
On the other hand, let $C_1=C \cap K$ and $C_2=C\setminus C_1$. 
considering coalition structure $\C'=\C\setminus \{C\}\cup (\{C_1\}\cup \{C_2\})$ , the difference between $\sw(\C')$ and $\sw(\C)$ is $\sw(\C')-\sw(\C)=\sw(C_1)+\sw(C_2)-\sw(C)$. Moreover, since $C_2$ is a set of pendant vertices and it is an independent set, $\sw(C_2)=0$. Also, by Lemma \ref{prop:Bilo}, $\sw(C_1)=2\binom{x}{2}/x$. Thus, note that $x\ge 3, y\ge 1$, we obtain
\begin{align*}
    \sw(\C')-\sw(\C) &= \frac{2\binom{x}{2}}{x} -\frac{ \left(2\binom{x}{2}+2y\right)}{x+y}\\
    &=\frac{2\binom{x}{2}(x+y) - \left(2\binom{x}{2}+2y\right)x}{x(x+y)}\\
    &=\frac{y(x-3)}{x+y}\ge 0. 
\end{align*}

%ゆえに，提携がクリーク内の頂点を3つ以上含むとき，社会効用を減らすことなくクリーク部分$C_1$とペンダント点部分$C_2$に分割することができる．
Thus, when a coalition contains at lease three vertices in clique $K$, it can be split into a clique $C_1=C \cap K$ and a set of pendant vertices $C_2=C\setminus C_1$ without reducing social welfare. 
\end{proof}

%次に，補題\ref{lem1}よりブロックスプリットグラフにおいて各提携がクリーク，スター，孤立点のいずれかになる社会効用最大提携構造が存在することを示す．
Next, we show that there exists a social optimum in which each coalition is either a clique of size at least 2, a star, or an isolated vertex from the lemma \ref{lem1}.

\begin{lemma}\label{lem:opt:structure}
%各提携がクリーク，スター，孤立点のいずれかになる社会効用最大提携構造が存在する．
There exists a social optimum in which each coalition induces a clique of size at least 2 
or a star or isolated vertex.
\end{lemma}
\begin{proof}
%提携内に含まれるクリーク内の頂点数に着目する．
We focus on the number of vertices in clique $K$ contained within the coalition. 
%補題\ref{lem1}より，クリーク内の頂点を3つ以上含む提携はクリークであるような社会効用最大提携構造が存在する．クリーク内の頂点を含まない提携は，孤立点集合となる．そのような提携は，社会効用を変えることなく，孤立点1つのみからなる提携に分割できる．
From Lemma \ref{lem1}, there exists a social optimum such that each coalition that contains at least three vertices in $K$ is a clique.
Each coalition that does not contain any vertices in $K$ is an independent set and such coalition can be split into coalitions consisting of only one isolated vertex without changing the social welfare.

%クリーク内の頂点をただ1つ含む提携は，ペンダント点を持たない場合，孤立点となる．また，ペンダント点を持つとき，隣接するペンダント点と提携を形成すると社会効用が最大となるので，提携はスターになる．ここで，葉の数を$l$とすると社会効用は$2l/(l+1)$で表されるので，葉の数が多いスターほど社会効用は大きくなる．よって，提携は隣接するペンダント点をすべて含んだスターとなる．
Each coalition that contains only one vertex in $K$ is a isolated vertex if the vertex has no pendant vertex. 
When it has some pendant vertices, the coalition is a star because the social welfare is maximized when the only one vertex in $K$ forming a coalition with neighboring pendant vertices. Let $\ell$ be the number of leaves, the social welfare of the star is $2\ell/(\ell+1)$. So the more leaves a star has, the greater its social welfare. Therefore, the coalition is a star that includes all adjacent pendant vertices.

%クリーク内の頂点を2つ含む提携に関して，2点ともペンダント点を持たない場合，提携はクリークになる．片方のクリーク内の頂点のみにペンダント点が隣接する場合，提携はスターになる．その他の場合，つまり，2点ともペンダント点を持つ場合について考える．提携に含まれるクリーク内の2点を$v_1, v_2$，それぞれに隣接するペンダント点の数を$p_1, p_2$とする．$v_1, v_2$に隣接する各ペンダント点は提携に含まれない場合，効用が0になる．また，提携内にペンダント点を$x_1+x_2\ (0\le x_1\le p_1,\ 0\le x_2\le p_2)$個含むときの社会効用は，$2(x_1+x_2+1)/(x_1+x_2+2)=2-2/(x_1+x_2+2)$となる．ゆえに，$x_1=p_1,\  x_2=p_2$のとき社会効用が最大となるので，2点ともペンダント点を持つ場合，提携はクリーク内の2点に隣接するペンダント点をすべて含んだダブルスターになる．
For each coalition containing two vertices in $K$, the coalition is a clique if neither of the two vertices has any pendant vertices. If only one of the vertices in $K$ has pendant vertices, the coalition is a star. 
We consider the other case, i.e., when both vertices have pendant vertices. 
Let $v_1$ and $v_2$ be the two vertices in $K$ included in the coalition and $p_1$ and $p_2$ be the number of pendant vertices adjacent to $v_1$ and $v_2$ respectively. Each pendant vertex adjacent to $v_1$ and $v_2$ has zero utility if it is not form a coalition with $v_1$ and $v_2$ respectively. 
We consider the case where $v_1$ and $v_2$ form a coalition which induce a double star. Let $x_1$ and $x_2$ be the number of pendant vertices of $v_1$ and $v_2$ which contain the double star. Then, the social welfare when $x_1+x_2\ (0\le x_1\le p_1,\ 0\le x_2\le p_2)$ pendant vertices are included in the double star is $2(x_1+x_2+1)/(x_1+x_2+2)=2-2/(x_1+x_2+2)$. Hence, since the social welfare is maximized when $x_1=p_1,\ x_2=p_2$, if both vertices have pendant vertices, the coalition is a double star containing all pendant vertices adjacent to the two vertices in $K$.
%このとき，社会効用は$2(p_1+p_2+1)/(p_1+p_2+2)$，ダブルスターを$v_1$，$v_2$を中心点とする2つのスターに分割したときの社会効用は，$2p_1/(p_1+1)+2p_2/(p_2+1)$である．ここで，$p_1,p_2\ge 1$のとき，$2p_1/(p_1+1)+2p_2/(p_2+1)\ge 2(p_1+p_2+1)/(p_1+p_2+2)$であるため，ダブルスターは社会効用を減少させることなくスターに分割できる．したがって，各提携がクリーク，スター，孤立点のいずれかになる社会効用最大提携構造が存在する．
The social welfare of the double star is $2(p_1+p_2+1)/(p_1+p_2+2)$, and the social welfare when the double star is divided into two stars whose centers are $v_1$ and $v_2$ is $2p_1/(p_1+1)+2p_2/(p_2+1)$. 
Since $2p_1/(p_1+1)+2p_2/(p_2+1)\ge 2(p_1+p_2+1)/(p_1+p_2+2)$ when $p_1,p_2\ge 1$, the double star can be split into two stars without reducing the social welfare. Thus, there exists a social optimal in which each coalition induces a clique of size at least 2 or a star or isolated vertex.
\end{proof}

%ここで，ペンダント点のみからなる提携を含まない社会効用最大提携構造が存在することを示す．ペンダント点を持たないクリーク内の頂点の集合を$C_0$，ペンダント点を持つクリーク内の頂点の集合を$K\setminus C_0$で表す．
Furthermore, we show that there exists a social optimum that does not contain any coalitions consisting of only pendant vertices. We denote with $Z$ the set of vertices in $K$ which are not adjacent to any pendant vertices, and denote with $K\setminus Z$ the set of vertices in $K$ which are adjacent to some pendant vertices.

%また，各$v_i \in K\setminus Z$に対して提携$C_i$を$C_i=\{v_i\}\cup(N(v_i)\cap I)$とする．
%$v_i\in K\setminus Z$が持つペンダント点の数を$p_i$とする．

%以下書き換えました．

\begin{lemma}\label{lem:pendant:star}
%クリーク部分とペンダント点部分で分割した提携構造が，$K\setminus C_0$内の頂点はそれぞれを中心点としたスターに，$Z$内の頂点は一つの提携にまとめた提携構造より社会効用が大きくなることはない．
The social welfare of the coalition structure in which vertices in $K$ are partitioned into a clique and pendant vertices are partitioned into a single coalition is no greater than the social welfare of the coalition structure in which each vertex in $K\setminus Z$ is the center of a star, and the vertices in $Z$ are partitioned into a clique.
\end{lemma}

\begin{proof}
%$K\setminus Z$に属する$h$個の頂点$v_1, v_2, \ldots, v_h$と，$Z$に属する$z$個の頂点からなる提携を$C_1$とする．また，$v_1, v_2, \ldots, v_h$に隣接するペンダント点集合からなる提携を$C_2$とする．提携構造$\C$を$\C=\{C_1\}\cup \{C_2\}$とする．このとき，提携$C_1$はサイズ$h+z$のクリークである．一方，提携$C_2$は孤立点集合であり，$\sw(C_2)=0$なので，$\sw(\C)=\sw(C_1)+\sw(C_2)=h+z-1$である．
Let $C_1$ be the coalition consisting of $h$ vertices $v_1, v_2, \ldots, v_h$ belonging to $K\setminus Z$ and $z$ vertices belonging to $Z$. Let $C_2$ be the coalition consisting of the set of pendant vertices adjacent to $v_1, v_2, \ldots, v_h$. Let the coalition structure $\C$ be $\C=\{C_1\}\cup \{C_2\}$.
Then, $C_1$ is a clique of size $h+z$ and $C_2$ is a set of isolated vertices. So, $\sw(C_2)=0$ and $\sw(\C)=\sw(C_1)+\sw(C_2)=h+z-1$.

%はじめに，$z=0$のときの$G[C_1\cup C_2]$について考える．$v_1, v_2, \ldots, v_h$をそれぞれ中心点として提携$C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$に分割すると，$v_i$が持つペンダント点の数を$p_i=|N(v_i)\cap I|$として，社会効用は$\sum_{i=1}^{h}(2p_i/(p_i+1))\ge h>h-1=\sw(\C)$となる．よって，$z=0$のとき，クリーク部分とペンダント点部分で分割した提携構造よりも，クリーク内の頂点をそれぞれ中心点としたスターに分割した提携構造の方が社会効用が大きくなる．次に，$z\ge1$のときについて考える．$G[C_1\cup C_2]$においてペンダント点を持つクリーク内の頂点$v_i$は$C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$に分割し，$Z$に属する$z$個の頂点は一つの提携にまとめた提携構造を$\C'$とする．すなわち，$\C'$は$h$個のスターとサイズ$z$のクリークからなる提携構造である．$\C'$の社会効用を考えると，$\sum_{i=1}^{h}(2p_i/(p_i+1))\ge h$より，$\sw(\C')=\sum_{i=1}^{h}(2p_i/(p_i+1))+z-1\ge h+z-1=\sw(\C)$となる．
First, we consider $G[C_1\cup C_2]$ when $z=0$. 
Let $p_i=|N(v_i)\cap I|$ be the number of pendant vertices of $v_i$. 
When each vertex in $v_1, v_2, \ldots, v_h$ is partitioned into coalition $C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$ with $v_i$ as a center of the star respectively, the social welfare is $\sum_{i=1}^{h}(2p_i/(p_i+1))\ge h>h-1=\sw(\C)$. Thus, when $z=0$, the social welfare is larger for the star partition than for the coalition structure in which vertices in $K$ are partitioned into a clique and pendant vertices are partitioned into a single coalition. 
Next, we consider the case when $z\ge1$.
In $G[C_1\cup C_2]$, let $\C'$ be the coalition structure in which each vertex $v_i$ in $K$ which is adjacent to some pendant vertices is divided into $C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$ and the $z$ vertices belonging to $Z$ are partitioned into a clique. That is, $\C'$ is a coalition structure consisting of $h$ stars and a clique of size $z$. Considering the social welfare of $\C'$, since $\sum_{i=1}^{h}(2p_i/(p_i+1))\ge h$, $\sw(\C')=\sum_{i=1}^{h}(2p_i/(p_i+1))+z-1\ge h+z-1=\sw(\C)$.

%したがって，クリーク部分とペンダント点部分で分割した提携構造が，$K\setminus Z$内の頂点はそれぞれを中心点としたスターに，$Z$内の頂点は一つの提携にまとめた提携構造より社会効用が大きくなることはない．
Therefore, the social welfare of the coalition structure in which vertices in $K$ are partitioned into a clique and pendant vertices are partitioned into a single coalition is no greater than the social welfare of the coalition structure in which each vertex in $K\setminus Z$ is the center of a star, and the vertices in $Z$ are partitioned into a clique.
\end{proof}

%次に，$K\setminus Z$に属する各頂点がそれぞれスターの中心点となるような社会効用最大提携構造が存在することを示す．
Next, we show that there exists a social optimum such that each vertex belonging to $K\setminus Z$ is the center of a star.

\begin{lemma}\label{lem3}
%$K\setminus Z$に属する各頂点がそれぞれスターの中心点となるような社会効用最大提携構造が存在する．
There exists a social optimum such that each vertex in $K\setminus Z$ is the center of a star.
\end{lemma}

\begin{proof}
%社会効用最大提携構造において，$K\setminus Z$に属する各頂点がどのような提携に属するかを考える．補題\ref{lem:opt:structure}より，各提携がクリーク，スター，孤立点のいずれかになる社会効用最大提携構造が存在する．このとき，クリーク内の頂点を1つまたは2つ含む提携において，$K\setminus Z$に属する各頂点はスターの中心点となっている．また，クリーク内の頂点を3つ以上含む提携はクリークになっている．一方，補題\ref{lem:pendant:star}より，クリーク部分とペンダント点部分で分割した提携構造が，$K\setminus Z$内の頂点はそれぞれを中心点としたスターに，$Z$内の頂点は一つの提携にまとめた提携構造より社会効用が大きくなることはない．よって，クリーク内の頂点を3つ以上含む提携に$K\setminus Z$に属する頂点が含まれるとすると，$K\setminus Z$内の頂点をそれぞれ中心点としたスターと，$Z$内の頂点をまとめた提携に社会効用を減らすことなく分割することができる．ゆえに，$K\setminus Z$に属する各頂点がそれぞれスターの中心点となるような社会効用最大提携構造が存在する．
We consider what kind of coalition each vertex in $K\setminus Z$ belongs to in a social optimum.
From the lemma \ref{lem:opt:structure}, there exists a social optimum in which each coalition induces a clique of size at least 2 or a star or isolated vertex. 
In a coalition that contains one or two vertices in $K$, each vertex belonging to $K\setminus Z$ is the center of a star. Also, a coalition containing at least three vertices in $K$ is a clique. 
On the other hand, by Lemma \ref{lem:pendant:star}, the social welfare of the coalition structure in which vertices in $K$ are partitioned into a clique and pendant vertices are partitioned into a single coalition is no greater than the social welfare of the coalition structure in which each vertex in $K\setminus Z$ is the center of a star, and the vertices in $Z$ are partitioned into a clique.
Thus, if a coalition containing at least three vertices in $K$ includes a vertex belonging to $K\setminus Z$, it can be partitioned into stars whose centers are each vertex in $K\setminus Z$ respectively and a coalition that contains vertices in $Z$ without reducing the social welfare. Therefore, there exists a social optimum such that each vertex in $K\setminus Z$ is the center of a star.
\end{proof}


%また，$z\ge2$のとき，社会効用最大提携構造において$Z$内の頂点がどのような提携に属するかを考えるにあたり，次の補題が成り立つことを示す．
We also show that Lemma \label{lem2} holds to consider what kind of coalition each vertex in $Z$ belongs to in a social optimum when $z\ge2$.

\begin{lemma}\label{lem2}
%$v\in K\setminus Z$，$v$を含む提携を$C_v$とする．このとき，$C_v$が$Z$内の頂点を高々1つしか含まないような社会効用最大提携構造が存在する．
Let $v$ be a vertex in $K\setminus Z$, and $C_v$ be the coalition containing $v$. There exists a social optimum such that $C_v$ contains at most one vertex in $Z$.
\end{lemma}

\begin{proof}
%ある社会効用最大提携構造において，提携$C_v$が$Z$内の頂点を$t\ (\ge2) $個含むとする．補題\ref{lem1}より，クリーク内の頂点を3つ以上含む提携はクリークであるような社会効用最大提携構造が存在する．よって，$C_v$は大きさ$t+1$のクリークとなり，$v$のペンダント点集合$P_v=N(v)\cap I$は孤立点集合となっている．
Assume that $C_v$ contains $t\ (\ge2)$ vertices in $Z$ in a social optimum. From Lemma \ref{lem1}, there exists a social optimum such that each coalition that contains at least three vertices in $K$ is a clique. Thus, $C_v$ is a clique of size $t+1$ and the set of pendant vertices of $v$ denoted with $P_v=N(v)\cap I$ is an independent set.
%ここで，補題\ref{lem:pendant:star}より，クリーク部分とペンダント点部分で分割した提携構造が，$K\setminus Z$内の頂点はそれぞれを中心点としたスターに，$Z$内の頂点はクリークにまとめた提携構造より社会効用が大きくなることはないので，社会効用を下げることなく$C_v\cup P_v$をスターおよびクリークに分割することができる．したがって，$v$を含む提携が$Z$内の頂点を含まないような，別の社会効用最大提携構造が存在する．よって，$v\in K\setminus Z$，$v$を含む提携を$C_v$として，$C_v$が$Z$内の頂点を高々1つしか含まないような社会効用最大提携構造が存在する．
Here, from Lemma \ref{lem:pendant:star}, the social welfare of the coalition structure in which vertices in $K$ are partitioned into a clique and pendant vertices are partitioned into a single coalition is no greater than the social welfare of the coalition structure in which each vertex in $K\setminus Z$ is the center of a star, and the vertices in $Z$ are partitioned into a clique. Therefore, we can split $C_v\cup P_v$ into a star and a clique without reducing social welfare. Thus, there exists another social optimal coalition structure such that the coalition containing $v$ does not contain a vertex in $Z$. Therefore, there exists a social optimum such that $C_v$ contains at most one vertex in $Z$.
\end{proof}

%これらの補題を用いて，ペンダント点を持たないクリーク内の頂点数$z$に応じて社会効用最大提携構造を考える．以降では，ペンダント点を持つクリーク内の頂点$v\in K\setminus Z$に対して，提携$C_v$は$C_v=\{v\}\cup (N(v)\cap I)$を表すものとする．
Using these Lemmas, we consider a social optimum depending on the value of $z$ which is the number of vertices not adjacent to any pendant vertices. In the following, the coalition $C_v$ denote $C_v=\{v\}\cup (N(v)\cap I)$ for the vertex $v\in K\setminus Z$.

%はじめに，$z\ge2$のとき，提携構造$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$が社会効用最大提携構造であることを示す．
First, we prove that the coalition structure $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimum when $z\ge2$.

\begin{lemma}\label{lem:opt}
%$z\ge 2$であるブロックスプリットグラフ$G=(K\cup I, E)$において，提携構造$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$は社会効用最大提携構造である．
On a block split graph $G=(K\cup I, E)$ with $z\ge 2$, the coalition structure $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimum.
\end{lemma}

\begin{proof}
%$z\ge2$とし，ペンダント点を持つクリーク内の頂点を$V_h=\{v_1,v_2,\ldots, v_h\}$，ペンダント点を持たないクリーク内の頂点を$Z=\{v_{h+1},v_{h+2},\ldots,  v_{h+z}\}$とする．すなわち，$K=V_h\cup Z$である．
Let $z\ge2$, $V_h=\{v_1,v_2,\ldots, v_h\}$ be the vertices in $K$ which are adjacent to some pendant vertices and $Z=\{v_{h+1},v_{h+2},\ldots, v_{h+z}\}$ be vertices in $K$ which are not adjacent to any pendant vertices. That is, $K=V_h\cup C_0$.

%補題\ref{lem3}より，$V_h$に属する各頂点がそれぞれスターの中心点となるような社会効用最大提携構造$\C^*$が存在する．以下では，そのような$\C^*$において$Z$内の頂点がどのような提携に属するかを考える．$Z$内の頂点はペンダント点を持たずスターの中心点になることはないので，補題\ref{lem:opt:structure}より，この社会効用最大提携構造$\C^*$において$Z$内の頂点$v_{h+1},v_{h+2},\ldots,v_{h+z}$はスターの葉，孤立点，クリークの一部のいずれかになる．
From Lemma \ref{lem3}, there exists a social optimum $\C^*$ such that each vertex belonging to $V_h$ is the center of a star.
In the following, we consider what kind of coalition the vertices in $Z$ belong to in such $\C^*$.
Since each vertex in $Z$ does not have pendant vertices and cannot be the center of a star, by Lemma \ref{lem:opt:structure}, each vertex in $v_{h+1},v_{h+2},\ldots,v_{h+z}$ is a leaf of a star, an isolated vertex, or a part of a clique in $\C^*$ .

%はじめに，$Z$内の頂点がクリークの一部または孤立点となる場合を考える．$Z$内の頂点すべてで1つのクリークを形成したときの社会効用は$z-1$である．一方，クリークの社会効用はクリークのサイズを$x$として$2\binom{x}{2}/x=x-1$で表されるので，$Z$内の頂点を複数のクリークに分割したときの社会効用は$z-1$より小さくなる．また，孤立点とサイズ$x$のクリークの社会効用を考えると，$0+(x-1)=x-1$となる．この孤立点がサイズ$x$のクリークに加わると社会効用は$(x+1)-1=x$となるので，$Z$内の頂点は孤立点となるよりもクリークの一部となった方が全体の効用は大きくなる．よって，$Z$内の頂点がクリークの一部または孤立点となる場合を考えると，$Z$内の頂点すべてがまとまってサイズ$z$のクリークを形成するとき，社会効用は最大となる．
First, we consider the case where a vertex in $Z$ becomes either part of a clique or an isolated vertex. The social welfare of a clique formed by all the vertices in $Z$ is $z-1$. On the other hand, by Property \ref{property:clique}, the social welfare of a clique of size $k$ is $k-1$, so the social welfare when the vertices in $Z$ are divided into multiple cliques is smaller than $z-1$.
Also, the social welfare of an isolated vertex and a clique of size $k$ is $0+(k-1)=k-1$. When the isolated vertex is added to the clique of size $k$, the social welfare becomes $(k+1)-1=k$. Thus, the total utility of the vertex in $Z$ is greater when each vertex in $Z$ is a part of a clique than when it is an isolated vertex. Therefore, considering the case where each vertex in $Z$ becomes part of a clique or an isolated vertex, the social welfare is maximized when all vertices in $Z$ collectively form a clique of size $z$.

%次に，$Z$内の頂点がスターの葉となることを考える．ここで，$V_h$に属する各頂点は提携$C_{v_i}=\{v_i\}\cup (N(v_i)\cap I)$を形成し，$Z$内の頂点$z$個のうち$t$個（$v_{h+1},v_{h+2},\ldots,v_{h+t}$）がそれぞれ$C_{v_1},C_{v_2},\ldots,C_{v_t}$にスターの葉として加わり，残りの$z-t$個が1つのクリークを形成しているとする．このとき，$t\le z$であり，補題\ref{lem2}より$v_i\in V_h$を含む提携$C_{v_i}$が$Z$内の頂点を高々1つしか含まないような社会効用最大提携構造が存在するので，$t \le h$である．
Next, we consider the case where some vertices in $Z$ become a leaf of a star respectively.
Assume that each vertex belonging to $V_h$ forms a coalition $C_{v_i}=\{v_i\}\cup (N(v_i)\cap I)$, and $t$ vertices in $Z$ denoted by $v_{h+1},v_{h+2},\ldots,v_{h+t}$ add into $C_{v_1},C_{v_2 },\ldots,C_{v_t}$ as a leaf of the star respectively and the remaining $z-t$ vertices form a clique.
Note that $t \le h$ because $t\le z$ and there exists a social optimum such that each $C_{v_i}$ which contains $v_i\in V_h$ contains at most one vertex in $Z$ by Lemma \ref{lem2}.

%$z>h$のとき，$z>t$すなわち$z-t>0$であり，$v_i\in V_h$が持つペンダント点の数を$p_i=|N(v_i)\cap I|$とするとこのときの社会効用は，$\sum_{i=1}^t 2(p_i+1)/(p_i+2) + \sum_{i=t+1}^h 2p_i/(p_i+1)+(z-t)-1$である．スターの葉として加わっている$Z$内の$t$個の頂点のうちの1頂点$v_{h+t}$がスターの葉を抜けクリークに加わると社会効用は，$\sum_{i=1}^{t-1} 2(p_i+1)/(p_i+2) + \sum_{i=t}^h 2p_i/(p_i+1)+(z-(t-1))-1$となる．よって社会効用の差を考えると，$Z$内の1頂点がスターの葉を抜けクリークに加わることにより，
When $z>h$, $z>t$ i.e. $z-t>0$.
Let $p_i=|N(v_i)\cap I|$ be the number of pendant vertices that $v_i\in V_h$ has. Then the social welfare of the partation is $\sum_{i=1}^t 2(p_i+1)/(p_i+2) + \sum_{i=t+1}^h 2p_i/(p_i+1)+(z-t)-1$. 
If $v_{h+t}$ which is one of the $t$ vertices in $Z$ joined as a leaf of a star deviates from the star to the clique of size $z-t$, the social welfare becomes $\sum_{i=1}^{t-1} 2(p_i+1)/(p_i+2) + \sum_{i=t}^h 2p_i/(p_i+1)+(z-(t-1))-1$. Thus, the difference of the social welfare by the deviation is 
\begin{align*}
    &\sum_{i=1}^{t-1} \frac{2(p_i+1)}{p_i+2} + \sum_{i=t}^h \frac{2p_i}{p_i+1}+(z-(t-1))-1\\
    &-\left(\sum_{i=1}^{t} \frac{2(p_i+1)}{p_i+2} + \sum_{i=t+1}^h \frac{2p_i}{p_i+1}+(z-t)-1\right)\\
    &=-\frac{2(p_t+1)}{p_t+2}+\frac{2p_t}{p_t+1}+1\\
    &=1-\frac{2}{(p_t+2)(p_t+1)}\ge2/3.
\end{align*}
%だけ社会効用は増加する．したがって$z>h$のとき，$Z$内の頂点は提携$C_{v_i}$にスターの葉として加わるよりもクリークを形成した方が社会効用は大きくなる．
Therefore, when $z>h$, the social welfare is greater when vertices in $Z$ forms a clique together than when they join the coalition $C_{v_i}$ as a leaf of a star respectively.

%$z\le h$のとき，$z-t=0$になり得るので，$t=z$と$t=0$の社会効用を比較する．前者の社会効用は$\sum_{i=1}^z 2(p_i+1)/(p_i+2) + \sum_{i=z+1}^h 2p_i/(p_i+1)$．後者の社会効用は$\sum_{i=1}^h 2p_i/(p_i+1)+z-1$．よって社会効用の差は，
Next, we compare the social welfare when $t=z$ and when $t=0$, since when $z\le h$, it can be $z-t=0$. The social welfare in the former case is $\sum_{i=1}^z 2(p_i+1)/(p_i+2) + \sum_{i=z+1}^h 2p_i/(p_i+1)$. The social welfare in the latter case is $\sum_{i=1}^h 2p_i/(p_i+1)+z-1$. Thus, the difference in social welfare is
\begin{align*}
    &\sum_{i=1}^h \frac{2p_i}{p_i+1}+z-1-\left(\sum_{i=1}^z \frac{2(p_i+1)}{p_i+2} + \sum_{i=z+1}^h \frac{2p_i}{p_i+1}\right)\\
    &=z-1+2\sum_{i=1}^z \left(\frac{1}{p_i+2}-\frac{1}{p_i+1}\right)\\
    &\ge z-1+2z\min_{i=1,\ldots,z}\left(\frac{1}{p_i+2}-\frac{1}{p_i+1}\right)\ge \frac{2}{3}z-1
\end{align*}
%となり，$z\ge2$では正の値となる．
and this value is positive for $z\ge2$.
%したがって，$z\le h$のときも，$z\ge2$であれば$Z$内の頂点は提携$C_{v_i}$にスターの葉として加わるよりも，クリークを形成した方が社会効用が大きくなる．
Thus, when $z\le h$ and $z\ge2$, the social welfare is greater when vertices in $Z$ form a clique than when they join the coalition $C_{v_i}$ as a leaf of a star respectively.

%以上より，$z \ge2$のとき，提携構造$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$は社会効用最大提携構造である．
Therefore, when $z\ge 2$, the coalition structure $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimum.
\end{proof}

%次に，$z=0$または$1$のとき，すべての提携がスターとなる社会効用最大提携構造$\C^*$が存在することを示す．
Next, we show that when $z=0$ or $1$, there exists a social optimum $\C^*$ in which each coalition is a star.
\begin{lemma}\label{lem:opt:structure:star}
%$z=0$または$1$のとき，すべての提携がスターとなる社会効用最大提携構造$\C^*$が存在する．
When $z=0$ or $1$, there exists a social optimum $\C^*$ in which each coalition is a star.
\end{lemma}

\begin{proof}
%はじめに，$z=0$のときを考える．このとき，$Z=\emptyset$である．補題\ref{lem3}より，クリークに属する各頂点がそれぞれスターの中心点となるような社会効用最大提携構造が存在する．よって，$z=0$のとき，$\C^*=\{C_v\mid v\in K\}$は社会効用最大提携構造である．
First, we consider the case when $z=0$. In this case, $Z=\emptyset$. From Lemma \ref{lem3}, there exists a social optimum such that each vertex belonging to $K\setminus Z$ is the center of a star. Thus, when $z=0$, $\C^*=\{C_v\mid v\in K\}$ is a social optimum.

%次に$z=1$のときについて考える．補題\ref{lem3}より，$K\setminus Z$に属する各頂点がそれぞれスターの中心点となるような社会効用最大提携構造$\C^*$が存在する．$Z=\{v_{h+1}\}$とする．以下では，そのような$\C^*$において$v_{h+1}$がどのような提携に属するかを考える．
Next, consider the case when $z=1$. From Lemma \ref{lem3}, there exists a social optimum such that each vertex belonging to $K\setminus Z$ is the center of a star and denote it $\C^*$. Let $Z=\{v_{h+1}\}$. In the following, we consider what kind of coalition $v_{h+1}$ belongs to in $\C^*$.
%補題\ref{lem:opt:structure}より，各提携がクリーク，スター，孤立点のいずれかになる社会効用最大提携構造が存在するが，$v_{h+1}$はペンダント点を持たず，スターの中心点にはならない．また，$v_{h+1}$は$Z$に属するただ1つの頂点であるため，クリークを形成することもない．よって，$v_{h+1}$がスターの葉または孤立点となる社会効用最大提携構造が存在する．$v\in K\setminus Z$を任意に1つ選び，提携$C_v$と$v_{h+1}$に着目する．提携構造$\C=\{C_v\}\cup\{v_{h+1}\}$とする．$v_{h+1}$が孤立点になるときの効用は$0$なので，$v$が持つペンダント点の数を$p_v=|N(v)\cap I|$とすると，$\sw(\C)=\sw(C_v)+0=2p_v/(p_v+1)$．一方で，$v_{h+1}$がスターの葉として提携$C_v$に加わると社会効用は，$2(p_v+1)/(p_v+2)>2p_v/(p_v+1)$．よって，$v_{h+1}$は孤立点になるよりも，スターの葉として加わった方が全体の効用は大きくなる．
From Lemma \ref{lem:opt:structure}, there exists a social optimum in which each coalition induces a clique of size at least 2 or a star or an isolated vertex, but since $v_{h+1}$ does not have a pendant vertex, it cannot be the center of a star. 
Also, since $v_{h+1}$ is the only vertex belonging to $Z$, it does not form a clique. Thus, there exists a social optimum where $v_{h+1}$ is a leaf of a star or an isolated vertex. 
We arbitrarily choose one vertex $v\in K\setminus Z$ and focus on the coalition $C_v$ that $v$ belongs to as the center of a star and the vertex $v_{h+1}$. 
Let the coalition structure $\C$ be $\C=\{C_v\}\cup\{v_{h+1}\}$ and $p_v=|N(v)\cap I|$ be the number of pendant vertices that $v$ has. Since $C_v$ is a star and the utility when $v_{h+1}$ is an isolated vertex is $0$, $\sw(\C)=\sw(C_v)+0=2p_v/(p_v+1)$. 
On the other hand, if $v_{h+1}$ is added to the $C_v$ as a leaf, the social welfare becomes $2(p_v+1)/(p_v+2)>2p_v/(p_v+1)$. Thus, the social welfare is greater when $v_{h+1}$ is added as a leaf than when it becomes an isolated vertex.
%また，$v_{h+1}$がスターの葉として加わったことによる社会効用の増加量は，$2(p_v+1)/(p_v+2)-2p_v/(p_v+1)=2/(p_v+1)(p_v+2)$．よって，$v_{h+1}$が葉の数が最も小さいスターの葉として加わるとき増加量は最大となるので，社会効用が最大となる．ゆえに，$z=1$のとき，$v_{h+1}$は葉の数が最も小さいスターの葉として加わる．
The amount of increase in social welfare due to the addition of $v_{h+1}$ as a leaf of a star is $2(p_v+1)/(p_v+2)-2p_v/(p_v+1)=2/(p_v+1)(p_v+2)$. 
Thus, the amount of increase is largest when $v_{h+1}$ is added as a leaf of a star with the lowest number of leaves, and we can maximize the social welfare. Hence, when $z=1$, $v_{h+1}$ is added as a leaf to a star with the lowest number of leaves.

%したがって，$z=0$または$1$のとき，すべての提携がスターとなる社会効用最大提携構造$\C^*$が存在する．
Therefore, when $z=0$ or $1$, there exists a social optimum $\C^*$ in which each coalition is a star.
\end{proof}

\begin{lemma}\label{lem:blocksplit:opt}
%任意のブロックスプリットグラフ$G=(K\cup I, E)$において，各提携がクリークまたはスターのいずれかになるような社会効用最大提携構造が存在する．
For any block split graph $G=(K\cup I, E)$, there is a social optimum in which each coalition induces a clique of size at least 2 or a star.
\end{lemma}




\subsection{Price of Stability}
\subsubsection{When $z\le2$}\label{subsection:PoS:012}
%本節では，ペンダント点を持たないクリーク内の頂点数$z$に応じて，\ref{subsection:opt:blocksplit}節で示した社会効用最大提携構造を用いて$\PoS$の新たな上界を与える．はじめに，$z=0$または$1$のとき，全ての提携がスターとなる社会効用最大提携構造$\C^*$が存在し，$\C^*$が安定であることから$\PoS$が1となることを示す．次に，$z=2$のとき，$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$は社会効用最大提携構造であり，$\C^*$は安定とは限らないが，安定である別の提携構造を考えることで，2が$\PoS$の上界となることを示す．
In this subsection, we give a new upper bound for $\PoS$ using the social optimum shown in the subsection \ref{subsection:opt:blocksplit} depending on the number of $z$ that represents the number of vertices in $K$ which has no pendant vertices. 
First, we show that when $z=0$ or $1$, the social optimum $\C^*$ shown in the subsection \ref{subsection:opt:blocksplit} is also stable. It implies that $\PoS$ is 1. 
Next, when $z=2$, $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimal and $\C^*$ is not necessarily stable. However, we can construct an efficient stable coalition structure from $\C^*$ by merging some coalitions. Then we show that $\PoS$ is at most 2.

\paragraph{When $z=0$}
%本節では，クリーク内の頂点すべてがペンダント点を持つとき，すなわち$z=0$のときについて考える．このとき，補題\ref{lem:opt:structure:star}で示した社会効用最大提携構造$\C^*$は安定であり，$\PoS=1$であることを示す．
%In this section, we consider the case where $z=0$. Then, the social optimum $\C^*$ shown in the section \ref{subsection:opt:blocksplit} is also stable, and $\PoS$ is 1. 
\begin{theorem}\label{thm:blocksplit:upper:0}
%クリーク内の頂点すべてがペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS=1$．
For any block split graph $G=(K\cup I, E)$ such that each vertex in $K$ has at least one pendant vertex, $\PoS=1$.
\end{theorem}

\begin{proof}
%クリーク内の頂点集合を$K=\{v_1,v_2,\ldots v_h\}$とし，$v_i\in K$ が持つペンダント点の個数を$p_i=|N(v_i)\cap I|$とする．$z=0$のとき$Z=\emptyset$であり，補題\ref{lem:opt:structure:star}より，$C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$として提携構造$\C^*=\{C_{v_i}\mid v_i\in K\}$は社会効用最大提携構造である．
Let $K=\{v_1,v_2,\ldots v_h\}$ be the vertices in the clique and $p_i=|N(v_i)\cap I|$ be the number of pendant vertices that each $v_i\in K$ has.
When $z=0$, by $Z=\emptyset$ and Lemma \ref{lem:opt:structure:star}, the coalition structure $\C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$ is social optimum.
%また，$\C^*$は安定である．はじめに，各ペンダント点の効用は$1/(p_i+1)$であり，提携を移動するとその効用は$0$になるので，ペンダント点が別の提携に移ることはない．そして，$v_i\in K$の効用は$U(v_i,C_{v_i})=p_i/(p_i+1) \geq 1/2$であり，$v_i$がクリーク内の別の頂点$v_j$を中心点とするスターに移動すると，$U(v_i,C_{v_j}\cup\{v_i\})=1/(p_j+2) \leq 1/3$となる．よって，クリーク内の各頂点も提携を移らない．ゆえに，$\C^*$は安定である．
Also, $\C^*$ is stable.
First, under the coalition structure $\C^*$, the utility of each pendant vertex is $1/(p_i+1)$ and its utility becomes $0$ when it deviates from the coalition they belong to another. Thus pendant vertices never moves to another coalition.
The utility of $v_i$ in coalition $C_{v_i}$ is $U(v_i,C_{v_i})=p_i/(p_i+1) \geq 1/2$, and if $v_i$ deviates to a star whose center is another vertex $v_j\in K$, the utility of $v_i$ becomes $U(v_i,C_{v_j}\cup\{v_i\})=1/(p_j+2) \leq 1/3$.
Hence, each vertex in $K$ also does not deviate its coalition and $\C^*$ is stable.

%以上より，$\C^*$は社会効用最大提携構造かつ安定提携構造であるので，クリーク内の頂点すべてがペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS=1$である．
Therefore, since $\C^*$ is a social optimum and also stable, for any block split graph $G=(K\cup I, E)$ such that every vertex in $K$ has at least one pendant vertex, $\PoS=1$.
\end{proof}

\paragraph{When $z=1$}
%本節では，クリーク内の頂点のうち1つがペンダント点を持たないとき，すなわち$z=1$のときについて考える．このとき，補題\ref{lem:opt:structure:star}で示した社会効用最大提携構造$\C^*$は安定であり，$\PoS=1$であることを示す．
%In this section, we consider the case where $z=1$. Then, the social optimum $\C^*$ shown in the section \ref{subsection:opt:blocksplit} is also stable, and $\PoS$ is 1. 
\begin{theorem}\label{thm:blocksplit:upper:1}
%クリーク内の頂点のうち1つのみがペンダント点を持たず，その他はペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS=1$．
For any block split graph $G=(K\cup I, E)$ such that only one vertex in $K$ has no pendant vertices and other vertices in $K$ have at least one pendant vertex, $\PoS=1$.
\end{theorem}

\begin{proof}
%ペンダント点を持つクリーク内の頂点集合を$V_h=\{v_1,v_2,\ldots v_h\}$，ペンダント点を持たないクリーク内の頂点を$Z=\{v_{h+1}\}$とする．$K=V_h\cup Z$である．また，$v_i\in K\setminus Z$が持つペンダント点の個数を$p_i=|N(v_i)\cap I|$とする．$z=1$のとき，補題\ref{lem:opt:structure:star}より，各提携がそれぞれ$V_h$に属する頂点を中心点としたスターとなる社会効用最大提携構造$C^*$が存在する．このとき，$C^*$において$v_{h+1}$は$v\in\argmin_{v_i\in V_h} \{p_i\}$を中心点とするスターの葉になっていることに注意する．
Let $V_h=\{v_1,v_2,\ldots v_h\}$ be the set of vertices in $K$ which have pendant vertices and $Z=\{v_{h+1}\}$ be the vertex in $K$ which has no pendant vertices. Then $K=V_h\cup Z$.
Let $p_i=|N(v_i)\cap I|$ be the number of pendant vertices that $v_i\in K\setminus Z$ have.
When $z=1$, by the lemma \ref{lem:opt:structure:star}, there exists a social optimum $\C^*$ such that each coalition is a star whose center is the vertex belonging to $V_h$ respectively. Note that $v_{h+1}$ is a leaf of a star in $C^*$ whose center is $v\in\argmin_{v_i\in V_h} \{p_i\}$.

%また，$\C^*$は安定である．はじめに，$v_{h+1}$について考える．$\C^*$において，$v_{h+1}$は$v\in\argmin_{v_i\in V_h} \{p_i\}$を中心点とするスターの葉になっているので，その提携を$C_{v_i}$とすると，$U(v_{h+1},C_{v_i})=1/(p_i+2)$．$v_{h+1}$が別の$v_j\in V_h$を中心点としたスターとなっている提携$C_{v_j}$に移動すると，$p_i\le p_j$に注意して，$U(v_{h+1},C_{v_j}\cup\{v_{h+1}\})=1/(p_j+2)\le 1/(p_i+2)$．よって，$v_{h+1}$が別の提携に移動することはない．その他の頂点についても$z=0$のときの議論と同様に別の提携に移ることはない．よって，$\C^*$は安定である．
Then we show that $\C^*$ is stable. 
First, we consider $v_{h+1}$. In $\C^*$, $v_{h+1}$ is a leaf of a star with $v\in\argmin_{v_i\in V_h} \{p_i\}$ as its center, and denote the star by $C_{v_i}$. 
Then the utility of $v_{h+1}$ is $U(v_{h+1},C_{v_i})=1/(p_i+2)$. 
Considering the case where $v_{h+1}$ deviates from $C_{v_i}$ to a coalition $C_{v_j}\ (j\neq i)$ which is another star whose center is $v_j\in V_h$. 
Since $p_i\le p_j$, the utility of $v_{h+1}$ becomes $U(v_{h+1},C_{v_j}\cup\{v_{h+1}\})=1/(p_j+2)\le 1/(p_i+2)$. Hence, $v_{h+1}$ does not move to another coalition. For the other vertices, they do not move to another coalition as in the case in $z=0$. Therefore, $\C^*$ is stable.

%以上より，$\C^*$は社会効用最大提携構造かつ安定提携構造であるので，クリーク内の頂点のうち1つのみがペンダント点を持たず，その他はペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS=1$である．
Therefore, since $\C^*$ is a social optimal and also stable, for a block split graph $G=(K\cup I, E)$ such that only one vertex in $K$ has no pendant vertex and other vertices in $K$ have at least one pendant vertex, $\PoS=1$.
\end{proof}

\paragraph{When $z=2$}\label{subsubsection:PoS:z=2}
%本節では，ペンダント点を持たないクリーク内の頂点が2つのとき，すなわち$z=2$のときについて考える．このとき，補題\ref{lem:opt}より，$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$は社会効用最大提携構造である．しかし，$\C^*$は必ずしも安定ではない．これは，$p_i=1$となる$v_i\in K\setminus Z$が存在するとき，$v_i$は$Z=\{v_{h+1},v_{h+2}\}$からなる提携に移動することによって効用が上がるためである．そこで，$p_i=1$となる$v_i\in K\setminus Z$に注目して，安定である別の提携構造を考えることで，2が$\PoS$の上界であることを示す．
In this subsection, we consider the case where $z=2$. 
In this case, $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimum by Lemma \ref{lem:opt}. 
However, $\C^*$ is not necessarily stable. This is because when there exists $v_i\in K\setminus Z$ with $p_i=1$, $v_i$ can increase its utility by deviating to a coalition consisting of $Z=\{v_{h+1},v_{h+2}\}$. 
Then, by focusing on $v_i\in K\setminus Z$ with $p_i=1$ and considering another coalition structure that is stable, we show that $\PoS$ is at most 2.

\begin{theorem}\label{thm:blocksplit:upper:2}
%クリーク内の頂点のうち2つがペンダント点を持たず，その他はペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS\le2$．
For any block split graph $G=(K\cup I, E)$ such that two vertices in $K$ have no pendant vertices and other vertices in $K$ have at least one pendant vertex, $\PoS\le2$.
\end{theorem}

\begin{proof}
%ペンダント点を持つクリーク内の頂点集合を$V_h=\{v_1,v_2,\ldots v_h\}$，ペンダント点を持たないクリーク内の頂点集合を$Z=\{v_{h+1},v_{h+2}\}$ とする．$K=V_h\cup Z$である．また，$v_i\in K\setminus Z$が持つペンダント点の個数を$p_i=|N(v_i)\cap I|$とする．$z=2$のとき，補題\ref{lem:opt}より，$C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$として$\C^*=\{C_{v_i} \mid v_i\in V_h\} \cup \{Z\}$は社会効用最大提携構造である．ここで，$C_Z=Z$とする．$\C^*$の例を図\ref{fig:star}に示す．
Let $V_h=\{v_1,v_2,\ldots v_h\}$ be the set of vertices in $K$ which have pendant vertices and $Z=\{v_{h+1},v_{h+2}\}$ be the set of vertices in $K$ which has no pendant vertices. Then $K=V_h\cup Z$.
Let $p_i=|N(v_i)\cap I|$ be the number of pendant vertices that $v_i\in K\setminus Z$ have.
When $z=2$, by Lemma \ref{lem:opt}, $\C^*=\{C_{v_i} \mid v_i\in V_h\} \cup \{Z\}$ is a social optimum where $C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$. Let $C_Z$ be the coalition structure consisting of vertices in $Z$. Figure \ref{fig:star} shows an example of $\C^*$.

%$\C^*$の安定性について考える．
Now, we consider the stability of $\C^*$.
%任意の$v_i\in V_h$について$p_i\ge2$が成り立つとき，$\C^*$は安定であり，$\PoS=1$である．はじめに，提携$C_{v_i}\ (v_i\in V_h)$に着目すると，$\C^*$における$v_i\in V_h$の効用は，$U(v_i,C_{v_i})=p_i/(p_i+1)\ge 2/3$．$v_i$が別の$v_j\in V_h$を中心点としたスターとなっている提携$C_{v_j}$に移動することを考える．このとき$v_i$の効用は，$U(v_i,C_{v_j}\cup \{v_i\})=1/(p_j+2)\le 1/4$となる．よって，このような移動は起こらない．また，$v_i$が$Z$内の頂点からなる提携$C_Z$に移動すると，効用は，$U(v_i,C_Z\cup \{v_i\})=2/3\le U(v_i,C_{v_i})$となる．よって，$v_i\in V_h$が提携を移動することはない．また，ペンダント点は明らかに提携を移動しない．ゆえに提携$C_{v_i}\ (v_i\in V_h)$側からの頂点の移動は生じない．次に，提携$C_Z$について，$Z$内の頂点の効用は，$U(v_{h+1},C_Z)=U(v_{h+2},C_Z)=1/2$である．提携$C_{v_i}$側へ移ったときの効用は最大でも$1/(p_i+2)=1/4$なので，提携$C_Z$に属する頂点が提携を移ることはない．よって，任意の$v_i\in V_h$について$p_i\ge2$が成り立つとき，$\C^*$は安定であり，$\PoS=1$である．
When $p_i\ge2$ holds for any $v_i\in V_h$, $\C^*$ is stable and $\PoS=1$. At first, focusing on the coalition $C_{v_i}\ (v_i\in V_h)$, the utility of $v_i\in V_h$ in $\C^*$ is $U(v_i,C_{v_i})=p_i/(p_i+1)\ge 2/3$. We consider that $v_i$ deviates from $C_{v_i}$ to the $C_{v_j}$, which is a star whose center is another vertex $v_j\in V_h$. Then the utility of $v_i$ becomes $U(v_i,C_{v_j}\cup \{v_i\})=1/(p_j+2)\le 1/4$. Hence, such a deviation does not occur. 
If $v_i$ deviates from $C_{v_i}$ to $C_Z$, its utility becomes $U(v_i,C_Z\cup \{v_i\})=2/3\le U(v_i,C_{v_i})$. Hence, $v_i\in V_h$ does not deviate their coalition. Also, the pendant vertices obviously do not deviate their coalition. 
Therefore, no vertex in $C_{v_i}\ (v_i\in V_h)$ deviates from their coalition. 
Next, for coalition $C_Z$, the utility of a vertex in $C_Z$ is $U(v_{h+1},C_Z)=U(v_{h+2},C_Z)=1/2$. Since the utility when the vertex in $C_Z$ deviates to the coalition $C_{v_i}$ is at most $1/(p_i+2)=1/4$, vertices belonging to $Z$ never deviate. Therefore, $\C^*$ is stable and $\PoS=1$ when $p_i\ge2$ holds for any $v_i\in V_h$.

%一方，$p_i=1$となる$v_i\in V_h$が存在するとき，$\C^*$において$U(v_i,C_{v_i})=1/2$であり，提携$C_Z$に移ると，$U(v_i,C_Z\cup \{v_i\})=2/3>1/2$となるので，$\C^*$は安定ではない．そのため，安定提携構造として次の$\C$を考える．提携構造$\C$は，
On the other hand, when there exists $v_i\in V_h$ with $p_i=1$, since $U(v_i,C_{v_i})=1/2$ in $\C^*$ and $v_i$'s utility becomes $U(v_i,C_Z\cup \{v_i\})=2/3>1/2$ when $v_i$ deviates from $C_{v_i}$ to $C_Z$. Thus $\C^*$ is not stable. Therefore, we consider the following coalition structure $\C$ as a stable coalition structure. $\C$ is constructed to satisfy the following conditions: 
\begin{itemize}
    %\item $p_i\geq2$となるような$v_i$は，それぞれ$C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$に分割する
    %\item 残りの頂点は$C'_Z=Z\cup\{\{v_i\}\cup(N(v_i)\cap I)\mid p_i=1\}$として一つの提携にまとめる
    \item Each $v_i\in V_h$ such that $p_i\geq2$ is partitioned into $C_{v_i}=\{v_i\}\cup(N(v_i)\cap I)$ respectively.
    \item The remaining vertices are partitioned into one coalition as $C'_Z=Z\cup\{\{v_i\}\cup(N(v_i)\cap I)\mid p_i=1\}$.
\end{itemize}
%とする．
%その例を図\ref{fig:stable}に示す．
%\begin{figure}[htb]
%\begin{tabular}{cc}
%\begin{minipage}{0.45\hsize}
%\centering
%\includegraphics[keepaspectratio,width=0.7\hsize]{opt.png}
%\caption{社会効用最大提携構造$\C^*$の例}\label{fig:star}
%\end{minipage}
%\begin{minipage}{0.45\hsize}
%\centering
%\includegraphics[keepaspectratio,width=0.7\hsize]{nash.png}
%\caption{安定提携構造$\C$の例}\label{fig:stable}
%\end{minipage}
%\end{tabular}
%\end{figure}

%提携構造$\C$が安定であることを示す．$p_i=1$を満たす$v_i\in V_h$の数を$l$，$p_i\ge2$を満たす$v_i\in V_h$の数を$h-l$とする．はじめに，$p_i\ge2$を満たす$v_i\in V_h$を中心点とするスターとなっている提携$C_{v_i}$に着目する．各スターの葉は提携を移動すると効用が0になるので別の提携に移動することはない．また，提携$C_{v_i}$において$v_i$の効用は，$U(v_i,C_{v_i})=p_i/(p_i+1)\geq2/3$．よって，$U(v_i,C_{v_i})=2/3$のときに$v_i$が提携を移らないことを示せばよい．$v_i$が別の$v_j\in V_h$を中心点としたスターとなっている提携$C_{v_j}$に移動することを考える．このとき$v_i$の効用は，$U(v_i,C_{v_j}\cup \{v_i\})=1/(p_j+2)\le 1/4$となる．よって，このような移動は起こらない．$v_i$が提携$C'_Z$に移ることを考える．このとき，$C'_Z$に移った後の$v_i$の効用は，$U(v_i,C'_Z\cup\{v_i\})=(l+2)/(2l+3)$．ここで，$f(l)=(l+2)/(2l+3)$とすると，$f'(l) < 0$より$f(l)$は単調減少であり，$f(1) = 3/5 < 2/3$．よって，$v_i$が提携$C'_Z$に移ったとき，$U(v_i,C'_Z\cup\{v_i\})<2/3$となるので$v_i$が提携$C'_Z$に移ることもない．
We show that coalition structure $\C$ is stable. 
Let $l$ be the number of vertices $v_i\in V_h$ satisfying $p_i=1$ and $h-l$ be the number of vertices $v_i\in V_h$ satisfying $p_i\ge2$. 
First, we focus on the coalition $C_{v_i}$ that is a star whose center is $v_i\in V_h$ satisfying $p_i\ge2$. The leaves of the star do not deviate to another coalition because their utility become 0 when they deviate from the coalition they belong to to another coalition. In addition, the utility of $v_i$ in the coalition $C_{v_i}$ is $U(v_i,C_{v_i})=p_i/(p_i+1)\geq2/3$. Thus, it is sufficient to show that $v_i$ does not deviate to another coalition when $U(v_i,C_{v_i})=2/3$. 
We consider the case where $v_i$ deviates to another star coalition $C_{v_j}$ whose center is $v_j\in V_h (v_i\neq v_j)$. In this case, the utility of $v_i$ is $U(v_i,C_{v_j}\cup \{v_i\})=1/(p_j+2)\le 1/4$. Therefore, such deviation does not occur. 
We also consider the case where $v_i$ deviates to $C'_Z$. In this case, the utility of $v_i$ after deviating to $C'_Z$ is $U(v_i,C'_Z\cup\{v_i\})=(l+2)/(2l+3)$. Denote with $f(l)=(l+2)/(2l+3)$, $f(l)$ is monotonically decreasing because $f'(l) < 0$ and $f(1) = 3/5 < 2/3$. Therefore, since 
 $U(v_i,C'_Z\cup\{v_i\})<2/3$, $v_i$ does not deviate to $C'_Z$ either.

%次に，$C'_Z$に属する頂点について考える．各ペンダント点が提携を移動しないことは明らかである．各$v\in C'_Z\cap K$について，$U(v,C'_Z)\ge (l+1)/(2l+2)=1/2$．一方，提携$C'_Z$を逸脱して提携$C_{v_i}$側へ移ると効用は最大で$1/4$．よって，$C'_Z$に属する頂点が提携を移動することはない．従って，提携構造$\C$は安定である．
Next, we consider the vertices belonging to $C'_Z$. It is obvious that each pendant vertex does not deviate to another coalition. For each $v\in C'_Z\cap K$, $U(v,C'_Z)\ge (l+1)/(2l+2)=1/2$. On the other hand, if each $v\in C'_Z\cap K$ deviates from $C'_Z$ to another star coalition $C_{v_i}$ where $v_i\in V_h$ satisfying $p_i\ge2$, its utility becomes at most $1/4$. Hence, no vertices belonging to $C'_Z$ deviate from $C'_Z$. Therefore, $\C$ is stable.

%ここで，社会効用最大提携構造$\C^*$と安定提携構造$\C$において，$p_i\ge2$を満たす$v_i\in V_h$はそれぞれを中心点として$h-l$個のスターに分割され，それらの提携の社会効用は社会効用最大提携構造と安定提携構造で変化しない．したがって，社会効用最大提携構造と安定提携構造においてともにスターに分割される頂点集合の効用の和を$c$とすると，
Here, we compare the social optimum $\C^*$ and the stable coalition structure $\C$. 
In both coalition structures, each $v_i\in V_h$ satisfying $p_i\ge2$ is divided into $h-l$ stars with its pendant vertices respectively, and the sum of the social welfare of these coalitions does not change. Therefore, denote the sum of the social welfare of these $h-l$ stars with $c$, 
\begin{align*}
\PoS\le\frac{\sw(\C^*)}{\sw(\C)}=\frac{c+l+1}{c+((l+2)(l+1)+2l)/(2l+2)} = \frac{c+l+1}{c+(l^2+5l+2)/(2l+2)}.
\end{align*}
%である．
%ここで，$l+1\ge ((l+2)(l+1)+2l)/(2l+2)$より，上式は$c=0$で最大値をとる．よって，
Since $l+1\ge ((l+2)(l+1)+2l)/(2l+2)$, the above equation takes its maximum value when $c=0$. Hence, we obtain
\begin{align*}
\PoS\le\frac{c+l+1}{c+(l^2+5l+2)/(2l+2)}&\le\frac{l+1}{(l^2+5l+2)/(2l+2)}\\
&=\frac{2(l^2+2l+1)}{l^2+5l+2}=2-\frac{6l+2}{l^2+5l+2}\le2.
\end{align*}
%が成り立つ．
%したがって，クリーク内の頂点のうち2つがペンダント点を持たず，その他はペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS\le2$である．
Therefore, for any block split graph $G=(K\cup I, E)$ such that two vertices in $K$ have no pendant vertices and other vertices in $K$ have at least one pendant vertex, $\PoS\le2$.
\end{proof}

\subsubsection{When $z\ge3$}\label{subsection:PoS:3}

%\ref{subsection:PoS:012}節では，ペンダント点を持たないクリーク内の頂点数が0または1のとき1が，ペンダント点を持たないクリーク内の頂点数が2のとき2が，$\PoS$の上界であることを示した．しかし，ペンダント点を持たないクリーク内の頂点が$z\ (\ge3) $個の場合\ref{subsubsection:PoS:z=2}節と同様にペンダント点を$z-1$個以下だけ持つようなクリーク内の頂点の数に注目して$\PoS$の上界を考えると，同様の枠組みではPoSを定数で抑えることができない．そこで，本節ではペンダント点を持たないクリーク内の頂点が3つ以上の場合について安定性の十分条件を考え，3が$\PoS$の上界であることを示す．
%In subsection \ref{subsection:PoS:012}, we prove 1 is the upper bound of $\PoS$ when $z=0,1$, and 2 is the upper bound when $z=2$. 
%However, 
When $z\ (\ge3) $, we cannot bound the upper bound of $\PoS$ in the same framework as when $z=2$. 
In this subsection, we consider another stable coalition structure and its sufficient condition for stability. Then we can show that $\PoS$ is at most 3.

%$|Z|=z\left(\ge3\right)$とする．さらに，$Y \subseteq K \setminus Z$を適当にとり$|Y|=y$とし，$x=|N(Y)\cap I|-z$とおく．また，クリーク内の頂点$v$が持つペンダント点の個数を$p_v=|N(v)\cap I|$で表す．ここで，各$v\in K\setminus (Y\cup Z)$に対して提携$C_v=\{v\}\cup(N(v)\cap I)$を定義する．また，$C_Z=Z \cup Y \cup (N(Y)\cap I)$とする．提携構造$\C$を，$\C=\{C_v\mid v\in K\setminus(Y\cup Z)\}\cup \{C_Z\}$とする．提携構造$\C$の例を図\ref{fig.nash:suf}に示す．このとき，提携構造$\C$が安定となる十分条件を考える．
%Let $|Z|=z\left(\ge3\right)$. 
Choose $Y \subseteq K \setminus Z$ appropriately and let $|Y|=y$ and $x=|N(Y)\cap I|-z$. 
Let $p_v=|N(v)\cap I|$ be the number of pendant vertices that $v$ in $K\setminus Z$ has. For each $v\in K\setminus (Y\cup Z)$, we define the coalition $C_v=\{v\}\cup(N(v)\cap I)$. Also, we define the coalition $C_Z$ as $C_Z=Z \cup Y \cup (N(Y)\cap I)$. 
Let the coalition structure $\C=\{C_v\mid v\in K\setminus(Y\cup Z)\}\cup \{C_Z\}$.
Figure \ref{fig.nash:suf} shows an example of $\C$. 
First, we consider the sufficient condition for the stability of $\C$.
%\begin{figure}[htb]
%\centering
%\includegraphics[keepaspectratio,width=0.38\hsize]{5-3.png}
%\caption{$z=4$のときの提携構造$\C$の例} \label{fig.nash:suf}
%\end{figure}

\paragraph{The sufficient condition for stability}
%本節では，各$v\in K\setminus (Y\cup C_0)$に対して定義した提携$C_v$と提携$C_Z=Z \cup Y \cup (N(Y)\cap I)$に着目して，提携構造$\C$が安定となる十分条件を考える．そして，提携構造$\C$が安定となる十分条件を満たすときの$\C$の社会効用を求めることで，$\PoS$の値を見積もる．
In this part, we consider the sufficient condition for $\C$ to be stable by focusing on the $C_v$ defined for each $v\in K\setminus (Y\cup Z)$ and $C_Z$ . Then, we estimate the value of $\PoS$ by computing the social welfare of $\C$ when $\C$ satisfies the sufficient condition for stability.

\begin{lemma}\label{lem:nash:suf}
%$y-1\le x \le z+2y-3$が成り立つとき，提携構造$\C$は安定である．
The coalition structure $\C$ is stable when $y-1\le x \le z+2y-3$.
\end{lemma}

\begin{proof}
%まず，提携$C_v$側からの頂点の移動が起こらないことを示す．$C_v$において，ペンダント点は別の提携に移ると効用が0になるので，ペンダント点が提携を移ることはない．$v\in K\setminus (Y\cup Z)$について，$U(v,C_v)=p_v/(p_v+1)\ge 1/2$であり，$K\setminus (Y\cup Z)$に属する別の頂点を中心点としたスターに移動したときの効用は最大でも$1/3$なので，このような移動は起こらない．
First, we show that no vertices in $C_v$ deviate $C_v$. In $C_v$, the pendant vertices do not deviate from their coalition to another coalition because the utility of them become 0 by deviating. 
For $v\in K\setminus (Y\cup Z)$, $U(v,C_v)=p_v/(p_v+1)\ge 1/2$, and the utility when it deviates to another star whose center is another vertex belonging to $K\setminus (Y\cup Z)$ is at most $1/3$. Thus such deviation does not occur. 
%また，提携$C_Z$へ移ることを考える．$x\ge y-1$のとき，$x+z\ge z+y-1$が成り立つ．$|N(Y)\cap I|=x+z$より，$|N(Y)\cap I|\ge|Z|+|Y|-1$と変形でき, $2(|Z|+|Y|)\le |Z|+|Y|+|N(Y)\cap I|+1$が成り立つ．よって，$v\in K\setminus (Y\cup Z)$に対して，
Also we consider that the vertex in $C_v$ deviates to the $C_Z$. 
When $x\ge y-1$, $x+z\ge z+y-1$ holds. Since $|N(Y)\cap I|=x+z$, we can get $|N(Y)\cap I|\ge|Z|+|Y|-1$ and $2(|Z|+|Y|)\le |Z|+|Y|+|N(Y)\cap I|+1$ holds. 
Therefore, for $v\in K\setminus (Y\cup Z)$,
\begin{align*}
U(v,C_Z\cup \{v\})=\frac{|Z|+|Y|}{|Z|+|Y|+|N(Y)\cap I|+1}\le \frac{1}{2}\le \frac{p_v}{p_v+1}=U(v,C_v)
\end{align*}
%を満たす．ゆえに，提携$C_Z$に移動することもなく，提携$C_v$側からの頂点の移動は起こらない．
holds.
Hence, there is no deviation to the coalition $C_Z$ and no deviation of vertices from the coalition $C_v$.

%次に，提携$C_Z$について考える．まず，$v'\in Z$に着目する．$z+2y-3\ge x$のとき，$2z+2y-3\ge x+z$が成り立ち，$3(|Z|+|Y|-1)\ge|Z|+|Y|+|N(Y)\cap I|$と変形できる．よって，
Next, we consider the deviation from $C_Z$. 
First, we focus on $v'\in Z$. When $z+2y-3\ge x$, $2z+2y-3\ge x+z$ holds and $3(|Z|+|Y|-1)\ge|Z|+|Y|+|N(Y)\cap I|$. Hence,
\begin{align*}
 U(v',C_Z)=\frac{|Z|+|Y|-1}{|Z|+|Y|+|N(Y)\cap I|}\ge \frac{1}{3}
\end{align*}
%を満たす．一方，$v'\in Z$が提携$C_v$に移動すると，その効用は，
holds. On the other hand, when $v'\in Z$ deviates to coalition $C_v$, its utility becomes
\begin{align*}
    U(v',C_v\cup \{v'\})=\frac{1}{p_v+2}\le \frac{1}{3}.
\end{align*}
%となる．よって，$v'\in Z$が別の提携に移動することはない．
Therefore, $v'\in Z$ does not deviate to another coalition.
%ここで，ペンダント点は他の提携に移ると効用が0になるので提携を移ることはない．また，$v^{\prime\prime}\in Y$の効用については，
Futhermore, each pendant vertex in $C_Z$ does not deviate from $C_Z$ because its utility becomes 0 when it deviates to another coalition. 
Also, the utility of $v^{\prime\prime}\in Y$ is
\begin{align*}
U(v^{\prime\prime},C_Z)=\frac{|Z|+|Y|-1+p_{v^{\prime\prime}}}{|Z|+|Y|+|N(Y)\cap I|}> \frac{|Z|+|Y|-1}{|Z|+|Y|+|N(Y)\cap I|}=U(v',C_Z).
\end{align*}
%が成り立つ．よって，$v^{\prime\prime}\in Y$の効用は$v'\in Z$の効用より大きいので，$v^{\prime\prime}\in Y$が別の提携に移動することはない．ゆえに，提携$C_Z$側からの頂点の移動も起こらない．
Hence, since the utility of $v^{\prime\prime}\in Y$ is greater than that of $v'\in Z$, $v^{\prime\prime}\in Y$ does not deviate to another coalition. Thus, there is also no deviation from $C_Z$.

%以上より，$y-1\le x \le z+2y-3$を満たすとき，提携構造$\C$は安定である．
Therefore, $\C$ is stable when $y-1\le x \le z+2y-3$. 
\end{proof}

%以降では，不等式$y-1\le x \le z+2y-3$を安定性の十分条件と呼ぶ．ここで，$c=\sum_{v\in K\setminus (Y\cup Z)} 2p_v/(p_v+1)$と定義する．提携構造$\C$が安定性の十分条件を満たすとき，安定提携構造$\C$の社会効用は，
We call the inequality $y-1\le x \le z+2y-3$ the sufficient condition for stability. 
We define $c=\sum_{v\in K\setminus (Y\cup C_0)} 2p_v/(p_v+1)$. When $\C$ satisfies the sufficient condition for stability, the social welfare of $\C$ is
\begin{align*}
\sw(\C)=c+\sw(C_Z)=c+\frac{2|N(Y)\cap I|+(|Y|+|Z|)(|Y|+|Z|-1)}{|Z|+|Y|+|N(Y)\cap I|}= c+\frac{2(x+z)+(y+z)(y+z-1)}{x+y+2z}.
\end{align*}
%と表せる．一方，補題\ref{lem:opt}より，$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$は社会効用最大提携構造である．よって，社会効用最大提携構造の総効用は，
On the other hand, by Lemma \ref{lem:opt}, $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimal coalition structure. Thus, the social welfare of the social optimum is
\begin{align*}
\sw(\C^*)=c+\sum_{v\in Y} \frac{2p_v}{p_v+1}+|Z|-1=c+2\left(y-\sum_{v\in Y} \frac{1}{p_v+1}\right)+z-1.
\end{align*}
%すなわち，
That is
\begin{align*}
\PoS\le\frac{\sw(\C^*)}{\sw(\C)}=\frac{c+2(y-\sum_{v\in Y} 1/ (p_v+1))+z-1}{c+(2(x+z)+(y+z)(y+z-1))/(x+y+2z)}.
\end{align*}
%である．
%ここで，$2(y-\sum_{v\in Y} 1/ (p_v+1))+z-1\ge (2(x+z)+(y+z)(y+z-1))/(x+y+2z)$より，上式は$c=0$で最大値をとるので，
Since $2(y-\sum_{v\in Y} 1/ (p_v+1))+z-1\ge (2(x+z)+(y+z)(y+z-1))/(x+y+2z)$, the above equation has the maximum value when $c=0$. Then we can bound the value of $\PoS$ by
\begin{align}\label{align:PoS}
f(x,y,z)=\frac{(2(y-\sum_{v\in Y} 1/ (p_v+1))+z-1)(x+y+2z)}{2(x+z)+(y+z)(y+z-1)}.
\end{align}
%で$\PoS$を抑えることができる．次節以降では，PoSの上界を示すために$K\setminus Z$に属する頂点が持つペンダント点の数に注目して，場合分けを行う．場合分けの様子を図\ref{fig:case}に示す．
In the folowing, we will divide the cases by focusing on the number of pendant vertices that each vertex belonging to $K\setminus Z$ has in order to show the upper bound of $\PoS$.
The case classification is shown in Figure \ref{fig:case}. 
%\begin{figure}[htb]
%\centering
%\includegraphics[keepaspectratio,width=0.7\hsize]{case.png}
%\caption{ペンダント点の数による場合分けの様子} \label{fig:case}
%\end{figure}



\paragraph{When $p_v\ge z$ holds for any $v\in K\setminus Z$}
%本節では，任意の$v\in K\setminus Z$について$p_v\ge z$が成り立つときについて考える．このとき，補題\ref{lem:opt}で示した社会効用最大提携構造$\C^*$は安定であり，$\PoS=1$であることを示す．
In this part, we consider the case where $p_v\ge z$ holds for any $v\in K\setminus Z$. In this case, since the social optimum $\C^*$ shown in Lemma \ref{lem:opt} is also stable, $\PoS=1$.

\begin{lemma}\label{lem:y=emptyset}
%任意の$v\in K\setminus Z$について$p_v\ge z$が成り立つとき，$\PoS=1$．
When $p_v\ge z$ for any $v\in K\setminus Z$, $\PoS=1$.
\end{lemma}
\begin{proof}
%任意の$v\in K\setminus Z$について$p_v\ge z$が成り立つとする．補題\ref{lem:opt}より，提携構造$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$は社会効用最大提携構造である．このとき，$\C^*$が安定提携構造であることを示す．ここで，提携$C_Z=Z$とする．はじめに，提携$C_v\ (v\in K\setminus Z)$に注目すると，$\C^*$における$v\in K\setminus Z$の効用は，
Suppose that $p_v\ge z$ holds for any $v\in K\setminus Z$. By Lemma \ref{lem:opt}, $\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$ is a social optimum. We show that $\C^*$ is also stable. 
First, focusing on the coalition $C_v\ (v\in K\setminus Z)$, the utility of $v\in K\setminus Z$ in $\C^*$ is
\begin{align*}
U(v,C_v)=\frac{p_v}{p_v+1}\ge \frac{z}{z+1}=U(v,C_Z\cup\{v\}). 
\end{align*}
%よって，$v\in K\setminus Z$が提携$C_Z$に移ることはない．
Hence, each $v\in K\setminus Z$ does not deviate to $C_Z$.
%また$K\setminus Z$に属する別の頂点を中心点としたスターへの移動を考えると，提携を移ったあとの$v$の効用は最大でも$1/(z+2)<z/(z+1)\le U(v,C_v)$なので，このような移動は起こらない．ペンダント点については，明らかに提携を移ることはない．ゆえに，提携$C_v$側からの頂点の移動は起こらない．次に，提携$C_Z$に注目する．$v'\in Z$の効用は，
Also, considering a deviation to a star whose center is another vertex belonging to $K\setminus Z$, such a deviation does not occur because the utility of $v$ after deviating the coalition is at most $1/(z+2)<z/(z+1)\le U(v,C_v)$. 
For each pendant vertex in $C_v$, there is obviously no deviating form its coalition. Hence, no vertex deviate from the coalition $C_v$ for any $v\in K\setminus Z$. 
Next, we focus on the coalition $C_Z$. Then the utility of $v'\in Z$ is
\begin{align*}
U(v',C_Z)=\frac{z-1}{z}> \frac{1}{z+2}\ge\frac{1}{p_v+2}=U(v',C_v\cup\{v'\}).
\end{align*}
%よって，提携$C_Z$側からの頂点の移動も起こらない．
Hence, no vertex deviate from the coalition $C_Z$.

%ゆえに，任意の$v\in K\setminus Z$について$p_v\ge z$が成り立つとき，$\C^*$は社会効用最大提携構造かつ安定提携構造なので，$\PoS=1$である．
Therefore, if $p_v\ge z$ holds for any $v\in K\setminus Z$, since $\C^*$ is a social optimum and also stable, $\PoS=1$.
\end{proof}

\paragraph{When there exists $v\in K\setminus Z$ such that $0<p_v<z$}
%本節では，$0<p_v<z$となる$v\in K\setminus Z$が存在するときについて考える．このとき，社会効用最大提携構造提携構造$\C^*=\{C_v \mid v\in K\setminus Z\} \cup \{Z\}$における$0<p_v<z$を満たすような$v\in K\setminus Z$の効用について，$U(v,C_v)=p_v/(p_v+1)< z/(z+1)=U(v,Z\cup\{v\})$が成り立つ．よって，このような$v$は$Z$に属する頂点からなる提携に移動することにより効用が上がるので，$\C^*$は安定ではない．そこで，$K\setminus Z$に属する頂点が持つペンダント点の数に注目して，安定提携構造を考えていく．はじめに，$0<p_v<z$となる$v\in K\setminus Z$が存在し，$z\le p_v\le 2z-1$を満たす$v\in K\setminus Z$が存在する場合，$\PoS$が3以下となることを示す．
In this part, we consider the case where there exists $v\in K\setminus Z$ such that $0<p_v<z$. 
In this case, the utility of $v$ in $\C^*$ is $U(v,C_v)=p_v/(p_v+1)< z/(z+1)=U(v,Z\cup\{v\})$. 
Hence, $\C^*$ is not stable because the utility of such $v$ is increased by deviating to the coalition consisting of vertices belonging to $Z$. Therefore, we consider the stable coalition by focusing on the number of pendant vertices that each vertex belonging to $K\setminus Z$ has. 
First, we show that $\PoS \le3$ when there exists a vertex $v\in K\setminus Z$ such that $0<p_v<z$ and another vertex $u\in K\setminus Z$ satisfying $z\le p_u\le 2z-1$.


\begin{lemma}\label{lem:PoS:y=1}
%$0<p_v<z$を満たす$v\in K\setminus Z$が存在し，$z\le p_v\le 2z-1$を満たす$v \in K\setminus Z$が存在するとき，$\PoS \le3$．
When there exists a vertex $v\in K\setminus Z$ such that $0<p_v<z$ and another vertex $u\in K\setminus Z$ satisfying $z\le p_u\le 2z-1$, $\PoS \le3$.
\end{lemma}

\begin{proof}
%$z\le p_v\le 2z-1$を満たすような$v\in K\setminus Z$の1つを$u$として，$Y=\{u\}$とする．つまり，$C_Z=Z \cup \{u\} \cup (N(u)\cap I)$である．このとき$y=1$，定義より$p_u=x+z$であり，$z\le p_u\le 2z-1$である．すなわち，$0\le x\le z-1$と変形でき，$y-1\le x\le z+2y-3$が成り立っているので，補題\ref{lem:nash:suf}より，提携構造$\C$は安定である．ここで，$\sum_{v\in Y} 1/ (p_v+1)=1/(p_u+1)=1/(x+z+1)$なので式\eqref{align:PoS}より，
Let $u$ be one of $v\in K\setminus Z$ such that $z\le p_v\le 2z-1$, and $Y=\{u\}$. That is, $C_Z=Z \cup \{u\} \cup (N(u)\cap I)$. In this case, $y=1$, $p_u=x+z$, and $z\le p_u\le 2z-1$. That is, $0\le x\le z-1$ and $y-1\le x\le z+2y-3$ hold, and coalition structure $\C$ is stable by Lemma \ref{lem:nash:suf}. Since $\sum_{v\in Y} 1/ (p_v+1)=1/(p_u+1)=1/(x+z+1)$, by the formula \eqref{align:PoS},
\begin{align*}
f(x,z)=\frac{(2(1-1/(x+z+1))+z-1)(x+2z+1)}{2(x+z)+(z+1)z}
\end{align*}
%がPoSの上界を与える．ここで，$f(x,z)$を$x$で偏微分すると，
gives the upper bound of $\PoS$. The partial derivative with respect to the variable $x$ is
\begin{align*}
f_x(x,z)=\frac{x^2(z^3-3z+2)+2x(z^4+z^3-3z^2+3z+2)+z^5+2z^4+6z^2+5z+2}{(1+x+z)^2(2x+z(3+z))^2}.
\end{align*}
%$f_x(x,z)$について，$z\ge3$で$f_x(x,z)\ge0$が成り立つので，$f(x,z)$は$x$に関して単調増加する．よって，
For $f_x(x,z)$, $f(x,z)$ is monotonically increasing with respect to $x$ since $f_x(x,z)\ge0$ holds when $z\ge3$. Then, 
\begin{align*}
\PoS\le f(z-1,z)=\frac{3(z^2+z-1)}{z^2+5z-2}=3\left(1-\frac{4z-1}{z^2+5z-2}\right)\le3
\end{align*}
%であり，$0<p_v<z$を満たす$v\in K\setminus Z$が存在し，$z\le p_v\le 2z-1$を満たす$v \in K\setminus Z$が存在するとき，$\PoS \le3$が成り立つ．
and when there exists a vertex $v\in K\setminus Z$ such that $0<p_v<z$ and another vertex $u\in K\setminus Z$ satisfying $z\le p_u\le 2z-1$, $\PoS \le3$.
\end{proof}

%次に，$z\le p_v\le 2z-1$を満たす$v\in K\setminus Z$が存在しない場合について考え，PoSが3以下になることを示す．$v\in K\setminus Z$について$z\le p_v\le 2z-1$となる$v$が存在しないとき，任意の$v\in K\setminus Z$について$0<p_v<z$または$p_v\ge2z$である．仮定より$0<p_v<z$を満たす$v$が存在するので，そのいくつかを$Y$に加えていくことを考える．このとき，次の補題が成り立つ．
Next, we consider the case where there exists no $v\in K\setminus Z$ satisfying $z\le p_v\le 2z-1$, and show that $\PoS$ is at most 3. 
When there exists no $v\in K\setminus Z$ such that $z\le p_v\le 2z-1$, $0<p_v<z$ or $p_v\ge2z$ for any $v\in K\setminus Z$. Since there exists $v$ satisfying $0<p_v<z$ by assumption, we consider adding some of them to $Y$. %In this case, the following lemma holds.

\begin{lemma}\label{lem:PoS:y>1}
%$0<p_v<z$を満たす$v\in K\setminus Z$が存在し，$z\le p_v\le 2z-1$となる$v\in K\setminus Z$が存在しないとき，$\PoS \le3$．
When there exists a vertex $v\in K\setminus Z$ such that $0<p_v<z$ and there exists no $v\in K\setminus Z$ satisfying $z\le p_u\le 2z-1$, $\PoS \le3$.
\end{lemma}

\begin{proof}
%$0<p_v<z$を満たす$v$を$Y$に加えていくことを考える．はじめに，$0<p_v<z$を満たす$v$のいくつかを$Y$に加えていくと安定性の十分条件を満たす場合について考える．$0<p(v)<z$を満たす$v\in K\setminus Z$をペンダント点の数$|N(v)\cap I|$の降順に$v_1,v_2,\ldots$と並べて$Y$に加えていき，初めて$|N(Y)\cap I|\ge z+|Y|-1$を満たしたときの$Y$のサイズを$y$とする．すなわち，$Y=\{v_1,v_2,\ldots, v_y\}$，$y\ge2$である．このとき，仮定より安定性の十分条件を満たすので，補題\ref{lem:nash:suf}より，提携構造$\C$は安定である．$\PoS$の値を考える．
We consider adding $v$ satisfying $0<p_v<z$ to $Y$. 
First, we consider the case where the sufficient condition for stability is satisfied when some $v$ satisfying $0<p_v<z$ are added to $Y$.  
Let $v_1,v_2,\ldots$ be the number of pendant vertices $|N(v)\cap I|$ in descending order with $0<p(v)<z$ satisfying $v\in K\setminus Z$.
We add to $Y$ in order from $v_1$, and let the size of $Y$ when $|N(Y)\cap I|\ge z+|Y|-1$ is satisfied for the first time be $y$. 
That is, $Y=\{v_1,v_2,\ldots, v_y\}$ and $y\ge2$. Since the sufficient condition for stability is satisfied from the assumption, $\C$ is stable by Lemma \ref{lem:nash:suf}. Then we consider the value of $\PoS$.
%$p_i=|N(v_i)\cap I|$とすると$p_1\ge p_2\ge \cdots$であり，$|N(\{v_1,v_2,\ldots, v_{y-1}\})\cap I|=\sum_{i=1}^{y-1} p_i<z+(y-1)-1$かつ$|N(\{v_1,v_2,\ldots ,v_{y-1},v_y\})\cap I|=\sum_{i=1}^{y} p_i\ge z+y-1$を満たしている．ここで，$(y-1)p_{y-1}\le \sum_{i=1}^{y-1} p_i\le z+y-3$より，
We denote with $p_i=|N(v_i)\cap I|$ the number of pendant vertices of $v_i$. 
Then $p_1\ge p_2\ge \cdots$, $|N(\{v_1,v_2,\ldots, v_{y-1}\})\cap I|=\sum_{i=1}^{y-1} p_i<z+(y-1)-1$ and $|N(\{v_1,v_2,\ldots ,v_{y-1},v_y\})\cap I|=\sum_{i=1}^{y} p_i\ge z+y-1$. Since $(y-1)p_{y-1}\le \sum_{i=1}^{y-1} p_i\le z+y-3$, we obtain
\begin{align*}
p_y\le p_{y-1}\le 1+\frac{z-2}{y-1}.
\end{align*}
%である．さらに，$p_y=x+z-\sum_{i=1}^{y-1} p_i\ge x+z-(z+y-3)$より，$x\le p_y+y-3$なので，
Furthermore, since $p_y=x+z-\sum_{i=1}^{y-1} p_i\ge x+z-(z+y-3)$ and $x\le p_y+y-3$, 
\begin{align*}
    y-1\le x\le y+\frac{z-2}{y-1}-2
\end{align*}
%が成り立つ．
holds.

%ここで，式\eqref{align:PoS}の上界値を考える．
Then, we consider the upper bound of equation \eqref{align:PoS}.
%$a_i=\!\sqrt{p_i+1}$，$b_i=1/(\!\sqrt{p_i+1})$としてコーシー・シュワルツの不等式$\left(\sum_{i=1}^{y}a_i^2\right)\left(\sum_{i=1}^{y}b_i^2\right)\ge \left(\sum_{i=1}^{y}a_ib_i\right)^2$を用いると，$\sum_{i=1}^{y}p_i=x+z$より，
Denote $a_i=\!\sqrt{p_i+1}$, $b_i=1/(\!\sqrt{p_i+1})$ and apply to the Cauchy–Schwarz inequality $\left(\sum_{i=1}^{y}a_i^2\right)\left(\sum_{i=1}^{y}b_i^2\right)\ge \left(\sum_{i=1}^{y}a_ib_i\right)^2$, by $\sum_{i=1}^{y}p_i=x+z$, we can transform the inequality
\begin{align*}
&\left(\sum_{i=1}^{y}a_i^2\right)\left(\sum_{i=1}^{y}b_i^2\right)\ge \left(\sum_{i=1}^{y}a_ib_i\right)^2\\
&\Leftrightarrow\left(\sum_{i=1}^{y}\left(\sqrt{p_i+1}\right)^2\right)\left(\sum_{i=1}^{y}\left(\frac{1}{\sqrt{p_i+1}}\right)^2\right)\ge\left(\sum_{i=1}^{y}\left(\sqrt{p_i+1}\right)\frac{1}{\sqrt{p_i+1}}\right)^2\\
&\Leftrightarrow\left(x+y+z\right)\left(\sum_{i=1}^{y}\frac{1}{p_i+1}\right)\ge y^2
\end{align*}
%と変形できるので，$\sum_{i=1}^{y} 1/(p_i+1)$の最小値は$y^2/(x+y+z)$である．
and the minimum value of $\sum_{i=1}^{y} 1/(p_i+1)$ is $y^2/(x+y+z)$.
%よって，式\eqref{align:PoS}の上界値は，
Hence, the upper bound of equation \eqref{align:PoS} is
\begin{align*}
g(x,y,z)
&=\frac{(2(y-y^2/(x+y+z))+z-1)(x+y+2z)}{2(x+z)+(y+z)(y+z-1)}\\
&=\frac{(2y(x+z)+(z-1)(x+y+z))(x+y+2z)}{(x+y+z)(2(x+z)+(y+z)(y+z-1))}.
\end{align*}
%で与えられる．
%$g(x,y,z)$を$x$について偏微分すると，
The partial derivative of $g(x,y,z)$ with respect to the variable $x$ is
\begin{align*}
g_x(x,y,z)=\frac{h(x,y,z)}{(x+y+z)^2(2(x+z)+(y+z)(y+z-1))^2}
\end{align*}
%ただし，
where
\begin{align*}
h(x,y,z)
&=x^2(2y^3+(5z-3)y^2+(4z^2-11z+3)y+z(z-3)(z-1))\\
&+2x(2y^4+(7z-3)y^3+(9z^2-10z+3)y^2+(5z^2-15z+6)yz\\
&+(z^2-4z+3)z^2)+2y^5-3y^4+3y^3+11y^4z-15y^3z+9y^2z\\
&+20y^3z^2-23y^2z^2+9yz^2+16y^2z^3-19yz^3+3z^3+6yz^4-4z^4+z^5.
\end{align*}
%である．
%ここで$h(x,y,z)$の$x^2$の係数は，$y\ge1,\ z\ge3$では常に正である．また，$h(x,y,z)$を$x$の2次式とみなしたときの判別式は，
The coefficient of $x^2$ in $h(x,y,z)$ is always positive when $y\ge1,\ z\ge3$. Also, when $h(x,y,z)$ is regarded as a quadratic equation of $x$, the discriminant is
\begin{align*}
D/4&=-2y^2z(2y^5+9y^4(z-1)+2y^3(8z^2-17z+6)+y^2(14z^3-46z^2+37z-9)\\
&+2yz(3z^3-13z^2+16z-6)+(z-3)(z-1)^2z^2)
\end{align*}
%となり，$y\ge1,\ z\ge3$では$D/4\le0$となる．よって，$h(x,y,z)\ge0$である．ゆえに，$y\ge 1,\ z\ge3$のとき$g_x(x,y,z)\ge0$となるので，$g(x,y,z)$は$x$に関して単調増加である．
and $D/4\le0$ when $y\ge1,\ z\ge3$. Thus, $h(x,y,z)\ge0$. 
Hence, $g(x,y,z)$ is monotonically increasing with respect to $x$ since $g_x(x,y,z)\ge0$ when $y\ge 1,\ z\ge3$.
%よって，$x=y+(z-2)/(y-1)-2$を代入して，
Thus, by substituting $x=y+(z-2)/(y-1)-2$, we obtain
\begin{align*}
\PoS&\le g(y+\frac{z-2}{y-1}-2,y,z)\\
&=\frac{\left(2y(y+\frac{z-2}{y-1}-2+z)+(z-1)(y+\frac{z-2}{y-1}-2+y+z)\right)\left(y+\frac{z-2}{y-1}-2+y+2z\right)}{\left(y+\frac{z-2}{y-1}-2+y+z\right)\left(2(y+\frac{z-2}{y-1}-2+z)+(y+z)(y+z-1)\right)}\\
&=\frac{(2y^2+2y(z-2)-z)(2y^2+4y(z-2)+z^2-5z+4)}{(2y+z-4)(y^3+2y^2z-z(z-1)+y(z^2-z-5))}.
\end{align*}
%となる．
%ここで，この値が$y\ge2,\ z\ge3$において3以下となることを示す．これは，$y\ge2,\ z\ge3$において，
Next, we show that this value is at most 3 when $y\ge2,\ z\ge3$. This is equivalent to %the fact that
\begin{align*}
\phi(y,z)&=3(2y+z-4)(y^3+2y^2z-z(z-1)+y(z^2-z-5))\\
&-(2y^2+2y(z-2)-z)(2y^2+4y(z-2)+z^2-5z+4)\\
&=(y-2)z^3+(2y^2-3y+10)z^2+(3y^3+14y^2-33y-8)z\\
&+2y(y-2)(y^2+8y-19)\\
&\ge0
\end{align*}
%が成り立つことと同値である．$\phi(y,z)$の各次の$z$の係数に着目すると，$y\ge2$においてはそれぞれ0以上になるので，$ \phi(y,z)\ge0$が成り立つ．ゆえに，$0<p_v<z$を満たす$v$のいくつかを$Y$に加えていくと安定性の十分条件を満たす場合，$\PoS\le3$である．
holds in $y\ge2,\ z\ge3$.
By focusing on the coefficients of $z$ of each order of $\phi(y,z)$, $ \phi(y,z)\ge0$ holds since each of them is at least 0 in $y\ge2$. 
Thus, if the sufficient condition for stability is satisfied when some $v$ satisfying $0<p_v<z$ are added to $Y$, $\PoS\le3$.

%次に，$0<p_v<z$を満たす$v$をすべて$Y$に加えても安定性の十分条件を満たさない場合について考える．$0<p_v<z$を満たす頂点$v$の集合を$Y$とする．ここで，$0<p_v<z$を満たす頂点$v$をすべて$Y$に加えても安定性の十分条件を満たさないので，$x=\sum_{v\in Y} p_v-z<y-1\le y+(z-2)/(y-1)-2$であることに注意すると，提携構造$\C$が安定であれば式\eqref{align:PoS}の単調増加性から，この場合の$\PoS$は3以下となる．そのため，以下では$\C$が安定であることを示す．
Next, we consider the case where the sufficient condition for stability is not satisfied even if all $v$ satisfying $0<p_v<z$ are added to $Y$. 
Let $Y$ be the set of vertex $v$ satisfying $0<p_v<z$. Note that $x=\sum_{v\in Y} p_v-z<y-1\le y+(z-2)/(y-1)-2$ since adding all vertices $v$ satisfying $0<p_v<z$ does not satisfy the sufficient condition for stability. Then in this case, if the coalition structure $\C$ is stable, $\PoS \le3$ due to the monotonic increase in equation \eqref{align:PoS}.

%$p_v\ge2z$となる$v\in K\setminus Z$が存在しない場合，提携構造$\C$は全体提携からなっているので，$\C=\{K\cup I\}$であり安定である．$p_v\ge2z$となる$v\in K\setminus Z$が存在する場合について考える．はじめに，提携$C_v\ (v\in K\setminus (Y\cup Z))$について考える．各ペンダント点については，明らかに提携を移ることはない．$v\in K\setminus (Y\cup Z)$に注目すると$p_v\ge2z$が成り立つので，$v\in K\setminus (Y\cup Z)$の効用は，$U(v,C_v)=p_v/(p_v+1)\ge2z/(2z+1)$である．提携$C_Z$に移ると効用は，$U(v,C_Z\cup\{v\})=(y+z)/(y+z+(x+z)+1)=(y+z)/(x+y+2z+1)$となる．その差を求めると，
When there exists no $v\in K\setminus Z$ such that $p_v\ge2z$, the coalition structure $\C$ is stable since $\C=\{K\cup I\}$ and it contains all vertices. So we consider the case where there exists $v\in K\setminus Z$ such that $p_v\ge2z$. 
First, consider the coalition $C_v\ (v\in K\setminus (Y\cup Z))$. For each pendant vertex, there is obviously no deviating to another coalition. Since $p_v\ge2z$ holds, the utility of vertex $v\in K\setminus (Y\cup Z)$ is $U(v,C_v)=p_v/(p_v+1)\ge2z/(2z+1)$. 
If $v$ deviates to $C_Z$, the utility becomes $U(v,C_Z\cup\{v\})=(y+z)/(y+z+(x+z)+1)=(y+z)/(x+y+2z+1)$. The difference of the utility is
\begin{align*}
U(v,C_v)-U(v,C_Z\cup\{v\})&\ge
\frac{2z}{2z+1}-\frac{y+z}{x+y+2z+1}\\
&=\frac{2xz+2z^2+z-y}{(x+y+2z+1)(2z+1)}\\
&=\frac{2(x+z)z+z-y}{(x+y+2z+1)(2z+1)}\\
&\ge\frac{y(2z-1)+z}{(x+y+2z+1)(2z+1)}\\
&\ge0.
\end{align*}
%である．2つ目の不等号は$Y$の各頂点がペンダント点を1つ以上持つことから$x+z\ge y$が成り立つのでいえる．また，$K\setminus (Y\cup Z)$に属する別の頂点を中心としたスターへの移動を考えると，提携を移った後の$v$の効用は最大でも$1/(2z+2)<2z/(2z+1)\le U(v,C_v)$となる．よって，このような移動は起こらない．したがって，提携$C_v$側からの頂点の移動は起こらない．
The second inequality can be held because each vertex in $Y$ has at least one pendant vertex and $x+z\ge y$ holds. 
Also, by considering a deviation to a star whose center is another vertex belonging to $K\setminus (Y\cup Z)$, the utility of $v$ after deviating is at most $1/(2z+2)<2z/(2z+1)\le U(v,C_v)$. Thus, such a deviation cannot occur. Therefore, no vertex in each $C_v$ for $v\in K\setminus (Y\cup Z)$ deviate from the coalition.
%続いて，提携$C_Z$について考える．$x<y-1$に注意すると$v'\in Z$の効用について，
Then we consider the coalition $C_Z$. Note that $x<y-1$, the utility of $v'\in Z$ is
\begin{align*}
 U(v',C_Z)=\frac{y+z-1}{x+y+2z}>\frac{y+z-1}{(y-1)+y+2z}=\frac{y+z-1}{2y+2z-1}. 
\end{align*}
%が成り立つ．$v'$が提携$C_v$に移ると，
If $v'$ deviates to $C_v$, its utility becomes
\begin{align*}
U(v',C_v\cup\{v'\})=\frac{1}{p_v+2}\le\frac{1}{2z+2}.
\end{align*}
%となる．その差を求めると，
The difference of the utility is
\begin{align*}
U(v',C_Z)-U(v',C_v\cup\{v'\})>\frac{y+z-1}{2y+2z-1}-\frac{1}{2z+2}=\frac{2z(y+z-1)-1}{(2y+2z-1)(2z+2)}>0.
\end{align*}
%よって，$v'\in Z$が提携$C_v$に移ることはない．$v^{\prime\prime}\in Y$の効用は，
Hence, there is no deviation of $v'\in Z$ to the coalition $C_v$. The utility of $v^{\prime\prime}\in Y$ is
\begin{align*}
U(v^{\prime\prime},C_Z)=\frac{y+z-1+p_{v^{\prime\prime}}}{x+y+2z}>\frac{y+z-1}{x+y+2z}=U(v',C_Z)
\end{align*}
%となり$v'\in Z$の効用より大きいので，$v^\prime\prime\in Y$が提携$C_v$に移動することはない．ペンダント点は明らかに提携を移動しない．ゆえに，提携$C_Z$側からの頂点の移動も起こらない．以上より，別の提携に移ることによって効用が上がる頂点が存在しないので，提携構造$\C$は安定である．よって，$0<p_v<z$を満たす$v$をすべて$Y$に加えても安定性の十分条件を満たさない場合についても$\PoS\le3$である．
and it is grater than the utility of $v'\in Z$, then $v^{\prime\prime}\in Y$ does not deviates to $C_v$. 
Each pendant vertex obviously does not deviate the coalition it belongs to. 
Thus, no vertex deviates from the coalition $C_Z$. 
Hence, the coalition structure $\C$ is stable because there are no vertices whose utility is increased by deviating to another coalition. 
Therefore, when the sufficient condition for stability is not satisfied even if all $v$ satisfying $0<p_v<z$ are added to $Y$, $\PoS\le3$. 
%ゆえに，$0<p_v<z$を満たす$v\in K\setminus Z$が存在し，$z\le p_v\le 2z-1$となる$v\in K\setminus Z$が存在しないとき，$\PoS \le3$．
Therefore, when there exists a vertex $v\in K\setminus Z$ such that $0<p_v<z$ and there exists no $v\in K\setminus Z$ satisfying $z\le p_u\le 2z-1$, $\PoS \le3$.
\end{proof}

%以上より，補題\ref{lem:y=emptyset}，補題\ref{lem:PoS:y=1}，補題\ref{lem:PoS:y>1}が成り立つので，次の定理が成り立つ．
By Lemmas \ref{lem:y=emptyset}, \ref{lem:PoS:y=1} and \ref{lem:PoS:y>1}, Theorem \ref{thm:blocksplit:upper} holds. 

\begin{theorem}\label{thm:blocksplit:upper}
%クリーク内の頂点のうち$z\ (\ge3)$個がペンダント点を持たず，その他はペンダント点を1つ以上持つようなブロックスプリットグラフ$G=(K\cup I, E)$について，$\PoS \le3$．
For any block split graph $G=(K\cup I, E)$ such that $z\ (\ge3)$ vertices in $K$ have no pendant vertices and other vertices in $K$ have at least one pendant vertex, $\PoS \le3$.
\end{theorem}




==> chapter03_general.tex <==
\chapter{General graphs}\label{sec:gemeral}
%この章では，一般グラフにおける分数型ヘドニックゲームの$\PoS$にはこれまで知られていたものよりも小さい上界が存在することを示す．
In this section, we give an upper bound of $\PoS$ on general graphs that is smaller than the one already known.
%まず，グラフ$G$が非連結であるとき，$G$の$\PoS$は$G$の連結成分$C$が誘導する部分グラフ$G[C]$の$\PoS$の最大値によって抑えられることを示す．これを利用すると，任意のグラフに対して$\PoS\le \min\{n/2, \vc(G) n/(n-1)\}$を示すことができる．
To show that $\PoS\le \min\{n/2, \vc(G) n/(n-1)\}$ for any graphs, we first show that $\PoS$ of $G$ is at most the maximum value of $\PoS$ of the subgraph $G[C]$ induced by the connected component $C$ of $G$ when a graph $G$ is deconnected.

\begin{lemma}
%グラフ$G=(V,E)$が非連結であるとする．$G$の連結成分$C_1, C_2, \ldots, C_k$について，$G[C_i]$における分数型ヘドニックゲームの$\PoS$が$\alpha_i$以下ならば，$G$の$\PoS$は$\max_i\alpha_i$以下である．
Suppose that the graph $G=(V,E)$ is disconnected. 
Then, for connected components $C_1, C_2, \ldots, C_k$ of $G$, if $\PoS$ of fractional hedonic game in $G[C_i]$ is at most $\alpha_i$, $\PoS$ of $G$ is at most $\max_i\alpha_i$.
\end{lemma}

\begin{proof}
%グラフ$G$の各連結成分からなる部分グラフ$G[C_i]$において社会効用が最大となる安定提携構造を$\C_i$とする．%%%このとき，$\bigcup_i \C_i$は明らかに$G$の最大安定提携構造となる．
Let $\C_i$ be the stable coalition structure that maximizes the social welfare in the subgraph $G[C_i]$ consisting of each connected component of the graph $G$.
%このとき，$\bigcup_i \C_i$に含まれる各提携は，それぞれ同じ連結成分に属する頂点のみからなっている．ここで，複数の異なる部分グラフに属する頂点を含むような提携$C'_j\ (j=1,2,\ldots)$を含む別の安定提携構造$\C'$が存在すると仮定する．このとき，提携$C'_j$は同じ連結成分に属する頂点ごとに提携を分割すると，分割された提携のサイズはそれぞれ$C'_j$より小さくなるので，全体の社会効用は大きくなる．このようにしてできた提携構造を$\C^{\prime\prime}$とすると，$\C^{\prime\prime}$も安定提携構造である．また，$\C^{\prime\prime}$に属する提携はそれぞれ同じ連結成分に属する頂点のみからなっている．ここで，$\C_i$は$G[C_i]$において社会効用が最大となる安定提携構造なので，同じ連結成分に属する頂点だけを含む提携からなる提携構造で，$\bigcup_i \C_i$より社会効用が大きくなる安定提携構造は存在しない．よって，$\C=\bigcup_i \C_i$とすると，$\sw(\C)=\sw\left(\bigcup_i \C_i\right)\ge \sw(\C^{\prime\prime}) >\sw(\C')$である．ゆえに，$\bigcup_i \C_i$は$G$における社会効用が最大となる安定提携構造である．
Note that each coalition in $\bigcup_i \C_i$ consists of only vertices that belong to the same connected component. Assume that there exists another stable coalition structure $\C'$ that contains a coalition $C'_j\ (j=1,2,\ldots)$ such that the vertices in $C'_j$ belong to several different connected component. By dividing $C'_j$ into coalitions at each vertex belonging to the same connected component, the size of each divided coalition is smaller than $C'_j$, so the total utility is larger. 
Let $\C^{\prime\prime}$ be the coalition structure created in this way, $\C^{\prime\prime}$ is also a stable coalition structure. 
Moreover, each coalirion in $\C^{\prime\prime}$ consists of only vertices that belong to the same connected component. Since $\C_i$ is a stable coalition structure that maximizes social welfare in $G[C_i]$, there is no stable coalition structure whose social welfare is larger than $\bigcup_i \C_i$ among the coalition structures which consists of coalitions that include only vertices belonging to the same connected component. Therefore, let $\C=\bigcup_i \C_i$, $\sw(\C)=\sw\left(\bigcup_i \C_i\right)\ge \sw(\C^{\prime\prime}) >\sw(\C')$. Therefore, $\bigcup_i \C_i$ is a stable coalition structure that maximizes social welfare in $G$.
%%%%%%%ここで，複数の異なる部分グラフ$G[C_i],G[C_j],\ldots,$に属する頂点からなる提携$C'$を含む別の安定提携構造$\C'$が存在すると仮定する．このとき，提携$C'$は同じ連結成分に属する頂点ごとに提携を分割すると，分割された提携のサイズはそれぞれ$C'$より小さくなるので，全体の社会効用は大きくなる．このようにしてできた提携構造を$\C''$とすると，$\C''$も安定提携構造である．また，$\C''$に属する提携はそれぞれ同じ連結成分に属する頂点のみからなっている．ここで，$\C_i$は$G[C_i]$における最大安定提携構造なので，同じ連結成分に属する頂点だけを含む提携からなる提携構造で，$\bigcup_i \C_i$より社会効用が大きくなる安定提携構造は存在しない．よって，$\sw\left(\bigcup_i \C_i\right)\ge \sw(\C'') >\sw(\C')$である．ゆえに，$\bigcup_i \C_i$は$G$の最大安定提携構造となる．

%一方，$G[C_i]$における社会効用最大提携構造を$\C^*_i$とすると，$\bigcup_i \C^*_i$は$G$の社会効用最大提携構造となる．
On the other hand, let $\C^*_i$ be the social optimum in $G[C_i]$, $\bigcup_i \C^*_i$ is the social optimum in $G$.

%ここで，任意の$i$に対して$G[C_i]$における$\PoS$が$\alpha_i$以下であることから，$\sw(\C^*_i)\le \alpha_i \sw(\C_i)$が成り立つので，
Since $\PoS$ in $G[C_i]$ is at most $\alpha_i$ for any $i$, $\sw(\C^*_i)\le \alpha_i \sw(\C_i)$. Then, we obtain
\begin{align*}
    \PoS=\frac{\sw(\C^*)}{\sw(\C)}=\frac{\sum_i \sw(\C^*_i)}{\sum_i \sw(\C_i)}\le \frac{\sum_i \alpha_i\sw(\C_i)}{\sum_i \sw(\C_i)}
    \le \max_i \alpha_i.
\end{align*}
%である．ゆえに，グラフ$G=(V,E)$が非連結であるとき，$G$の連結成分$C_1, C_2, \ldots, C_k$について，$G[C_i]$における分数型ヘドニックゲームの$\PoS$が$\alpha_i$以下ならば，$G$の$\PoS$は$\max_i\alpha_i$以下である．
Therefore, when $G=(V,E)$ is disconnected, for connected components $C_1, C_2, \ldots, C_k$ of $G$, if $\PoS$ of fractional hedonic game in $G[C_i]$ is at most $\alpha_i$, $\PoS$ of $G$ is at most $\max_i\alpha_i$.
\end{proof}

%よって，以下ではグラフが連結であると仮定する．
Hence, in the following, we assume that the graph is connected.


\begin{theorem}\label{thm:pos:general}
%任意のグラフに対して，$\PoS\le \min\{n/2, \vc(G) n/(n-1)\}$．
For any graphs, $\PoS\le \min\{n/2, \vc(G) n/(n-1)\}$.
\end{theorem}

\begin{proof}
%任意の連結グラフを$G=(V,E)$とする．補題\ref{lem:Bilo:2018:vc}より，$\sw(\C^*)\le \min\{n-1,2\vc(G)\}$．
Let $G=(V,E)$ be an arbitrary connected graph. By Lemma \ref{lem:Bilo:2018:vc}, $\sw(\C^*)\le \min\{n-1,2\vc(G)\}$.
%一方，$G$は連結であるので，$|E|\ge|V|-1$が成り立つ．ここで，全体提携$\C=\{V\}$は安定であり，その社会効用は，$\sw(\C)=2|E|/|V|\ge2(|V|-1)/|V|=2-2/|V|$．
On the other hand, since $G$ is a connected graph, $|E|\ge|V|-1$. Moreover, grand coalition $\C=\{V\}$ is stable and the social welfare of $\C$ is $\sw(\C)=2|E|/|V|\ge2(|V|-1)/|V|=2-2/|V|$.
%よって，$\PoS$について，
Then we obtain
\begin{align*}
    \PoS\le\frac{\min\{n-1,2\vc(G)\}}{2-2/n}=\min\left\{\frac{n}{2},\frac{\vc(G)n}{n-1}\right\}.
\end{align*}
%が成り立つ．
\end{proof}

==> chapter03_split.tex <==
\chapter{Split graphs}\label{sec:split}
%%%%スプリットグラフは1つのクリーク$K$と1つの独立点集合$I$からなるグラフであり，$G=(K\cup I,E)$で表される．独立点集合$I$の各頂点はクリーク内の頂点と複数隣接してよい．
%この章では，安定提携構造として$G$の全体提携をとり，補題\ref{lem:Bilo:2018:vc}を用いることで，頂点数$n$のスプリットグラフにおけるPoSが$0.70711\sqrt{n}+1.2519$以下となることを示す．
In this section, we consider the upper bound of $\PoS$ on split graphs. We show that $\PoS$ on a split graph with $n$ vertices is at most $0.70711\sqrt{n}+1.2519$.

\begin{theorem}\label{thm:split:upper}
%任意のスプリットグラフ$G=(K\cup I, E)$について，$\PoS \le 0.70711\sqrt{n}+1.2519$．ただし，$n=|K\cup I|$．
For any split graph $G=(K\cup I, E)$, $\PoS \le 0.70711\sqrt{n}+1.2519$ where $n=|K\cup I|$.
\end{theorem}
\begin{proof}
Let $x=|K|$, $y=|I|$, $V=K\cup I$, and $|V|=n=x+y$.
%$G$の全体提携を$\C=\{K\cup I\}$とすると$\C$は安定である．また，$\C$の社会効用は，
The grand coalition $\C=\{K\cup I\}$ is stable and the social welfare of $\C$ is
\begin{align*}
    \sw(\C)=\frac{2|E|}{|V|}\ge \frac{2\left(\binom{x}{2}+y\right)}{x+y}=\frac{x(x-1)+2y}{x+y}.
\end{align*}

%$\C^*$を社会効用最大提携構造とする．補題\ref{lem:Bilo:2018:vc}と$\vc(G)=|K|=x$より，$\sw(\C^*)\le2\vc(G)=2x$．よって，$n\ge 7$に対して，
Let $\C^*$ be a social optimum. By Lemma \ref{lem:Bilo:2018:vc} and $\vc(G)=|K|=x$, $\sw(\C^*)\le2\vc(G)=2x$. Therefore, for $n\ge 7$,
\begin{align*}
    \PoS &\le \frac{\sw(\C^*)}{\sw(\C)} \le \frac{2x}{\frac{x(x-1)+2y}{x+y}}=\frac{2nx}{x(x-1)+2(n-x)}\\
    &=\frac{2nx}{x^2-3x+2n}\le \frac{2n\sqrt{2n}}{4n-3\sqrt{2n}}=\frac{2\sqrt{2}n}{4n-3\sqrt{2n}}\sqrt{n}\\
    &\le \frac{\sqrt{2}}{2}\sqrt{n}+\frac{3\sqrt{7}}{4\sqrt{7}-3\sqrt{2}}\le \frac{\sqrt{2}}{2}\sqrt{n}+1.2519\\
    &\le 0.70711\sqrt{n}+1.2519.
\end{align*}
%ここで，$1\le n\le 3$のとき，任意のグラフに対して$\PoS=1$である．また，$4\le n\le 5$のとき，$0.70711\sqrt{n}+1.2519\ge 2.667$を満たす．よって，$\PoS\le n/2\le2.5< 2.667\le 0.70711\sqrt{n}+1.2519$である．最後に，$n=6$のとき，$|E|\ge6$ならば，$\PoS\le |V|(|V|-1)/2|E|\le (6\cdot 5)/ (2\cdot 6) = 2.5\le 0.70711\sqrt{6}+1.2519\le  2.984$となる．一方，$G$は連結より，$|E|\ge |V|-1=5$であるから，$|E|=5$のときのグラフの$\PoS$を考える．グラフが連結かつ$|E|=|V|-1=5$であることから，このときのグラフは木である．よって，定理\ref{thm:pos:tree}より，$\PoS=1$である．ゆえに，任意の$n$に関して，$\PoS\le 0.70711\sqrt{n}+1.2519$である．
Here, when $1\le n\le 3$, $\PoS=1$ for any graphs. 
When $4\le n\le 5$, since $0.70711\sqrt{n}+1.2519\ge 2.667$ holds, $\PoS\le n/2\le2.5< 2.667\le 0.70711\sqrt{n}+1.2519$. 
When $n=6$, if $|E|\ge6$, $\PoS\le |V|(|V|-1)/2|E|\le (6\cdot 5)/ (2\cdot 6) = 2.5\le 0.70711\sqrt{6}+1.2519\le  2.984$. 
On the other hand, since $G$ is a connected graph and $|E|\ge |V|-1=5$, we conseider $\PoS$ of $G$ when $|E|=5$. 
Since $G$ is a connected graph and $|E|=|V|-1=5$, $G$ is a tree. Then, by Theorem \ref{thm:pos:tree}, $\PoS=1$. Therefore, for any $n$, $\PoS\le 0.70711\sqrt{n}+1.2519$ holds.
\end{proof}

==> chapter04.tex <==
\section{Maximizing utilitarian welfare on block graphs}\label{chap:block}
In this section, we show that a maximum utilitarian welfare coalition structure on block graphs can be computed in polynomial time. 
To show this, we first characterize an optimal coalition structure on block graphs, and then, we design a dynamic programming algorithm using the characterization.


\subsection{Characterizing an optimal coalition structure}
%はじめに，ブロックスプリットグラフの社会効用最大提携構造について，次のことが知られている．
In this subsection, we characterize an optimal coalition structure on block graphs.
\begin{theorem}\label{thm:block:opt}
%各提携がクリーク，スターのいずれかになる社会効用最大提携構造が存在する．
%There exists a maximum utilitarian welfare partition on the block graph in which each coalition induces a clique of size at least 2 or a star. 
There exists a maximum utilitarian welfare coalition structure on the block graph in which each coalition induces a clique or a star. 
\end{theorem}
To show this, we show the following two lemmas below.
% First, for the maximum utilitarian welfare coalition structure on block split graphs, which are more restricted graphs than block graphs,  the following lemma holds.
% \begin{lemma}[\cite{seniorthesis_2022}]\label{lem:blocksplit:opt}
% %任意のブロックスプリットグラフ$G=(K\cup I, E)$において，各提携がクリークまたはスターのいずれかになるような社会効用最大提携構造が存在する．
% For any block split graph $G=(K\cup I, E)$, there is a maximum utilitarian welfare coalition structure in which each coalition induces a clique of size at least 2 or a star.
% \end{lemma}

% \begin{lem}\label{lem:induce:block}
% ブロックグラフ$G=(V,E)$の社会効用最大提携構造の各提携はブロックグラフまたは孤立点からなる．
% \end{lem}
% \begin{proof}
% ブロックグラフ$G=(V,E)$の頂点部分集合$C\subseteq V$が誘導する部分グラフ$G[C]$はブロックグラフ，ブロックグラフと孤立点集合，孤立点集合のいずれかとなる．$G[C]$が複数の連結成分からなるとき，それらを連結成分ごとに分割して提携を形成した方が全体の効用は高くなるので，社会効用を下げることなく1つの連結成分からなる提携に分割することができる．よって，ブロックグラフ$G=(V,E)$の社会効用最大提携構造の各提携はブロックグラフまたは孤立点からなる．
% \end{proof}
%補題\ref{lem:induce:block}を用いて社会効用最大提携構造の各提携の直径について考えると，次の補題が成り立つ．
%次に，ブロックグラフにおける社会効用最大提携構造の各提携に着目すると，頂点部分集合が誘導する部分グラフがブロックグラフまたは孤立点集合のみを含むことより，社会効用最大提携構造の各提携がブロックグラフまたは孤立点からなることがわかる．そして，各提携の直径に着目することで，各提携がクリーク，スターのいずれかからなる社会効用最大提携構造が存在することを示す．
% Next, we focus on each coalition of optimal coalition structure on block graphs. We see that each coalition consists of a block graph or an isolated vertex, since all of the subgraphs induced by the subset of vertices are only block graph or independent set. We show that there exists a optimal coalition structure on the block graph in which each coalition induces a clique or a star by focusing the diameter of each coalition.

% Next, we show that a coalition with diameter 2 can be partitioned into cliques and stars without decreasing utilitarian welfare.
\begin{lemma}\label{lem:opt:diam2}
%直径2のブロックグラフからなる提携を$C$とする．このとき，社会効用を減らすことなく提携$C$をクリークまたはスターに分割することができる．
Let $C$ be a coalition such that the diameter of $G[C]$ is 2. Then  $C$ can be partitioned into cliques or stars without decreasing utilitarian welfare.
\end{lemma}

\begin{proof}
%グラフ$G=(v,E)$をブロックグラフ，$\C^*$を$G$のある社会効用最大提携構造とする．直径2の$C^*_i \in \C^*$が存在すると仮定する．ここで，$G$がブロックグラフであることから，$G[C^*_i]$はブロックグラフであり，関節点を1点のみ含む．この
%直径2の提携$C$が誘導する部分グラフ$G[C]$は関節点$v$をちょうど1つ含む．$G[C]$に含まれる各クリークは$v$を共有する．このとき，$G[C]$に含まれる最大クリークを$C_x$，そのサイズを$x$とする．$x=2$のとき，$C_x$が最大クリークであることより，$G[C]$はスターであるので，以降では$x\ge 3$の場合について考える．提携$C'$を$C'=C_x\setminus\{v\}$，提携$C^{\prime\prime}$を$C^{\prime\prime}=C\setminus C'$とする．このとき，$(\sw(C')+\sw(C^{\prime\prime})) \ge \sw(C)$となることを示す．
We first show that a coalition $C$ that induces a block graph having diameter 2 can be partitioned into cliques or stars without decreasing utilitarian welfare.
The subgraph $G[C]$ induced by a coalition $C$ having diameter 2 contains exactly one cut vertex $v$ and each maximal clique in $G[C]$ contains $v$.
Let $C_x$ be the largest clique in $G[C]$ and its size $x$. When $x=2$, $G[C]$ is a star. Thus, we consider the case $x\ge 3$ in the following. 
Let $C'=C_x\setminus\{v\}$ and $C^{\prime\prime}=C\setminus C'$. We show that $\uw(C')+\uw(C^{\prime\prime}) \ge \uw(C)$.

%提携$C^{\prime\prime}$に含まれる頂点数を$y$，辺数を$z$とする．$\sw(C)=2((x(x-1)/2)+z)/(x+y-1)=(x(x-1)+2z)/(x+y-1)$である．一方，$\sw(C')=(x-1)-1=x-2$であり，$\sw(C^{\prime\prime})=2z/y$である．よって，$C$を$C'$と$C^{\prime\prime}$に分割することによる社会効用の変化量は，
Let $y$ be the number of vertices and $z$ be the number of edges in  $G[C^{\prime\prime}]$. Then the utilitarian welfare of $C$ is $\uw(C)=2((x(x-1)/2)+z)/(x+y-1)=(x(x-1)+2z)/(x+y-1)$. On the other hand, $\uw(C')=(x-1)-1=x-2$ and $\uw(C^{\prime\prime})=2z/y$. Thus,  \begin{align}\label{align:opt:diam2}(\uw(C')+\uw(C^{\prime\prime}))-\uw(C) = (y^2(x-2)+2(x-1)(z-y))/y(x+y-1).\end{align}
% \begin{align}\label{align:opt:diam2}
%     &(\sw(C')+\sw(C^{\prime\prime}))-\sw(C)\notag\\
%     &= \left(x-2+\frac{2z}{y}\right) -\frac{x(x-1)+2z}{x+y-1}\notag\\
%     &= \frac{y^2(x-2)+2(x-1)(z-y)}{y(x+y-1)}. 
% \end{align}
If $G[C^{\prime\prime}]$ contains a clique of size at least 3, then $z-y\ge 0$. Since $x\ge 3$, we have $(\uw(C')+\uw(C^{\prime\prime}))\ge \uw(C)$. 
Otherwise, $G[C^{\prime\prime}]$ is a star. By Property \ref{property:star}, $\uw(C^{\prime\prime}) = 2(y-1)/y$.
Thus, $(\sw(C')+\sw(C^{\prime\prime}))-\sw(C) = x-2 +  2(y-1)/y - 2((x(x-1)/2)+y-1)/(x+y-1)
=x^2-2x +xy-2y -2x +2 +2(x+y-1) - 2(x+y-1)/y -x(x-1) + 2y -2 =  -x +xy  + 2y- 2(x-1)/y -4 \ge 1$ if $x\ge 3$ and $y\ge 2$.
For both cases, we can partition $C$ into two coalitions without decreasing utilitarian welfare. By repeating the partitioning procedure, we can partition $C$ into stars and cliques.\qed
\begin{comment}
%ここで，$x\ge 3$より，$y^2(x-2)\ge 0$，$y(x+y-1)\ge 0$である．また，$2(x-1)(z-y)$の正負について考えると，提携$C^{\prime\prime}$にサイズ3以上のクリークが1つ以上あるとき$z-y\ge 0$となるので，式\eqref{align:opt:diam2}より$(\sw(C')+\sw(C^{\prime\prime}))-\sw(C)\ge 0$となる．よって，提携$C^{\prime\prime}$にサイズ3以上のクリークが1つ以上あるとき，社会効用を下げることなく提携$C$を$C'$と$C^{\prime\prime}$に分割することができる．
Since $x\ge 3$, $y^2(x-2)\ge 0$，$y(x+y-1)\ge 0$.
Also, considering the sign of $2(x-1)(z-y)$, since $z-y\ge 0$ when there is one or more cliques whose size are at least 3 in the coalition $C^{\prime\prime}$, we get $(\sw(C')+\sw(C^{\prime})-\sw(C)\sw(C)\ge 0$ from the equation~\eqref{align:opt:diam2}. 
Thus, when there is more than one clique whose size are at least 3 in the coalition $C^{\prime\prime}$, we can split the coalition $C$ into $C'$ and $C^{\prime\prime}$ without decreasing the utilitarian welfare.
%ゆえに，この操作を繰り返すことにより，社会効用を下げることなく$C^*_i$をスターとクリークに分割することができる．
%一方，提携$C^{\prime\prime}$がサイズ2のクリークのみからなるとき，$z-y=-1$となる．しかし，このとき$G[C]$はブロックスプリットグラフであり，補題\ref{lem:blocksplit:opt}より，社会効用を下げずに提携$C$をクリークとスターに分割することができる．
On the other hand, when the coalition $C^{\prime\prime}$ contains only cliques whose size are 2, then $z-y=-1$. However, in this case $G[C]$ is a block split graph, and from Lemma~\ref{lem:blocksplit:opt}, we can split $C$ into cliques and stars without decreasing the utilitarian welfare.

%よって，この操作を高々$C$の2連結成分数回だけ行うことにより，社会効用を下げることなく提携$C$をクリークまたはスターに分割することができる．ゆえに，直径2のブロックグラフからなる提携$C$は，社会効用を減らすことなくクリークまたはスターに分割することができる．
By performing this operation at most a few times on the 2-connected components of $C$, the coalition $C$ can be split into cliques or stars without decreasing the utilitarian welfare.
Hence, a coalition $C$ which induces a block graph having diameter 2 can be split into cliques or stars without decreasing the utilitarian welfare.
%ある社会効用最大提携構造$\C^*$に直径2の提携$C^*_i \in \C^*$が存在するとき，社会効用を減らすことなくクリーク部分とスター部分に分割することができる．
\end{comment}
\end{proof}


% \begin{corollary}\label{cor:blocksplit:opt}
% There exists an optimal coalition structure such that each coalition of diameter 2 forms either a clique or a star on block graphs.
% \end{corollary}

%また，直径3以上の提携$C$についても，橋$e=\{u,v\}$（ただし，$e$を削除して得られる連結成分からなる2つの提携$C_u$，$C_v$の頂点数はともに2以上）が存在するか否かに着目して補題\ref{lem:opt:diam2}と同様に考えると，次の補題が成り立つ．

Then we prove that a coalition $C$ with diameter at least 3 can be partitioned into stars and cliques as in Lemma~\ref{lem:opt:diam2}. This implies the existence of an optimal coalition structure consisting of stars and cliques.
%We focus on whether or not there exists a bridge $e=\{u,v\}$ (however, two coalitions $C_u$ and $C_v$ obtained by deleting $e$ contain at least 2 vertices).
% \begin{lemma}\label{lem:opt:diam3}
% %直径3以上のブロックグラフからなる提携を$C$とする．このとき，社会効用を減らすことなく提携$C$を孤立点，クリーク，直径2のブロックグラフに分割することができる．
% Let $C$ be a coalition with induces a block graph having diameter 3 or more. We can split $C$ into isolated vertices, cliques, and a block graph whose diameter is 2 without decreasing the utilitarian welfare.
% \end{lemma}
\begin{lemma}\label{lem:opt:diam3}
Let $C$ be a coalition such that the diameter of $G[C]$ is at least 3. Then  $C$ can be partitioned into coalitions of diameter at most 2 without decreasing utilitarian welfare.
\end{lemma}

\begin{proof}
%はじめに，$C$に橋$e=\{u,v\}$（ただし，$e$を削除して得られる連結成分からなる提携$C_u$，$C_v$の頂点数はともに2以上）が存在するとき，$C$を$C_u$と$C_v$に社会効用を下げることなく分割できることを示す．


We first consider the case that $G[C]$ has a bridge $e=\{u,v\}$ and it connects two connected components of size at least 2. Let $C_u$ and $C_v$ be the connected components of $G[C]-e$ that contains $u$ and $v$, respectively. Then we can partition $C$ into two coalitions $C_u$ and $C_v$ without decreasing the utilitarian welfare.
%提携$C_u$に含まれる頂点数を$y_u$，辺数を$z_u$，提携$C_v$に含まれる頂点数を$y_v$，辺数を$z_v$とする．$\sw(C)=2(z_u+z_v+1)/(y_u+y_v)$である．一方，$\sw(C_u)=2z_u/y_u$であり，$\sw(C_v)=2z_v/y_v$である．よって，分割することによる社会効用の変化量は，
Let $y_u$ and $z_u$ be the number of vertices and the number of edges in $C_u$ and let $y_v, z_v$ be the number of vertices and  the number of edges in $G[C_v]$. 
Then the utilitarian welfare of $C$ is $\uw(C)=2(z_u+z_v+1)/(y_u+y_v)$.
On the other hand, the utilitarian welfare of $C_u$ is $\uw(C_u)=2z_u/y_u$  and the one of $C_v$ is $\uw(C_v)=2z_v/y_v$. Then, we have $(\uw(C_u)+\uw(C_v))-\uw(C)= {2z_u}/{y_u}+{2z_v}/{y_v}-{2(z_u+z_v+1)}/{(y_u+y_v)}
    = {(2y_u(y_u z_v-y_v)+2y_v^2 z_u)}/{y_u y_v(y_u+y_v)}\ge 0$.
% \begin{align*}
%     &(\uw(C_u)+\uw(C_v))-\uw(C)\\
%     &= \frac{2z_u}{y_u}+\frac{2z_v}{y_v}-\frac{2(z_u+z_v+1)}{y_u+y_v}\\
%     &= \frac{2y_u(y_u z_v-y_v)+2y_v^2 z_u}{y_u y_v(y_u+y_v)}\ge 0.
% \end{align*}
%ここで，最後の不等号は，$y_u,y_v\ge 2, z_v\ge y_v-1$であることより，$y_u z_v-y_v\ge y_u(y_v-1)-y_v=y_u y_v-(y_u+y_v)\ge0$であることから従う．よって，$C$に橋$e=\{u,v\}$があるとき，$C$を$C_u$と$C_v$に社会効用を下げることなく分割することができる．
The last inequality follows from $y_u,y_v\ge 2$ and  $z_v\ge y_v-1$. %since $y_u z_v-y_v\ge y_u(y_v-1)-y_v=y_u y_v-(y_u+y_v)\ge0$.
%Thus, when $C$ has a bridge $e=\{u,v\}$, we can split $C$ into $C_u$ and $C_v$ without decreasing the utilitarian welfare.
Thus, $C$ can be partitioned into two coalitions without decreasing the utilitarian welfare. 

%次に，$C$に橋がない場合について考える．
Next, we consider the case that there is no bridge that connects two connected components of size at least 2 in $C$.
%$G$がブロックグラフであることから，$G[C^*_i]$はブロックグラフである．$G[C]$において関節点を1つのみ持つクリークのうち最大であるものを$C_x$，そのサイズを$x$とする．また，$C_x$に属する頂点のうち$G[C]$において関節点となっている頂点を$v$とする．提携$C'$を$C'=C_x\setminus\{v\}$，提携$C^{\prime\prime}$を$C^{\prime\prime}=C\setminus C_x\cup\{v\}$とする．このとき，$(\sw(C')+\sw(C^{\prime\prime})) \ge \sw(C)$となることを示す．
Since $G$ is a block graph, $G[C]$ is also a block graph. Let $C_x$ be the largest clique of size $x(\ge 2)$ with only one cut vertex $v$ in $G[C]$. Such $v$ always exists unless $G[C]$ is not a clique. In other words, $C_x$ is a maximum-size leaf on the block-cut tree\footnote{The definition of a block-cut tree appears in Section~\ref{subsubsec:block-cut}} of $G[C]$. 
Let $C^{\prime}=C_x\setminus\{v\}$ and $C^{\prime\prime}=C\setminus C_x\cup\{v\}$. Then we show that $\uw(C^{\prime})+\uw(C^{\prime\prime})\ge\uw(C)$.

%提携$C^{\prime\prime}$に含まれる頂点数を$y$，辺数を$z$とする．このとき，補題\ref{lem:opt:diam2}と同様の議論により，提携$C$を提携$C'$と提携$C^{\prime\prime}$に分割することによる社会効用の変化量として，式\eqref{align:opt:diam2}と同じ式が得られる．$(y^2(x-2)+2(z-y)(x-1))/y(x+y-1)$の正負を考える．$x\ge2$より，$x-2\ge0,x-1>0,(x+y-1)>0$なので，$(y^2(x-2)+2(z-y)(x-1))/y(x+y-1)$の正負は$z-y$の正負による．ここで，$C$に橋がない場合について考えているので，$C_x$に隣接するクリークにはサイズ3以上のものが必ず存在する．よって，$z-y\ge0$は常に成り立つ．ここで，$C$に橋がない場合について考えているので，提携$C^{\prime\prime}$に含まれるクリークで$G[C]$において$C_x$に隣接するもののサイズは3以上である．よって，$z-y\ge0$は常に成り立つ．
Let $y$ be the number of vertices and $z$ be the number of edges in $G[C^{\prime\prime}]$. 
Figure~\ref{fig:nobridge} shows the value of $x,y$ and $z$ with respect to the examples of $C^{\prime}$ and $C^{\prime\prime}$.
\begin{figure}[htb]
\centering
\includegraphics[width=0.5\textwidth]{nobridge.pdf}
\caption{The value of $x,y$ and $z$ with respect to the examples of $C^{\prime}$ and $C^{\prime\prime}$.} \label{fig:nobridge}
\end{figure}
By the same argument as in Lemma~\ref{lem:opt:diam2}, we obtain Equation~\eqref{align:opt:diam2}. Since $x\ge 2$ and $y\ge 2$, the sign of $(y^2(x-2)+2(z-y)(x-1))/y(x+y-1)$ depends on the sign of $z-y$.
Since the diameter of $G[C]$ is at least 3, $C_x$ forms a clique, and there is no bridge that connects two connected components of size at least 2 in $C$, $G[C^{\prime\prime}]$ contains a cycle. Thus, we have $z-y\ge 0$. Therefore, we obtain $\uw(C^{\prime})+\uw(C^{\prime\prime})\ge\uw(C)$.


%これらの操作を高々$C$の2連結成分数回だけ行うこと行うことで$C$を孤立点，クリーク，直径2の提携に分割することができる．ゆえに社会効用を下げることなく提携$C$を孤立点，クリーク，直径2の提携に分割することができる．ゆえに，これらの操作を繰り返すことにより，社会効用を下げることなく$C^*_i$を孤立点，クリーク，直径2の提携に分割することができる．

By performing these operations unless the diameter of  $G[C]$ is at most 2, we can partition $C$ into coalitions whose diameter is 2 without decreasing utilitarian welfare. 
\qed
\end{proof}

%一方，補題\ref{lem:opt:diam2}，補題\ref{lem:opt:diam3}を用いると，社会効用最大提携構造について，孤立点のみからなる提携を含まないものが存在することが示せる．
By combining Lemmas~\ref{lem:opt:diam2} and \ref{lem:opt:diam3}, we can obtain a coalition structure whose coalitions form stars or cliques from any coalition structure. This implies Theorem~\ref{thm:block:opt}.

\begin{comment}
\begin{lemma}\label{lem:opt:isol}
%ブロックグラフ$G=(V,E)$において，孤立点のみからなる提携を含まない社会効用最大提携構造が存在する．
In a block graph $G=(V,E)$, there exists a maximum utilitarian welfare partition that does not contain a coalition which induces only isolated vertex.
\end{lemma}

\begin{proof}
%ブロックグラフ$G=(V,E)$の社会効用最大提携構造を考える．補題\ref{lem:induce:block}，補題\ref{lem:opt:diam2}，補題\ref{lem:opt:diam3}より，各提携が孤立点，クリーク，スターのいずれかからなる社会効用最大提携構造が存在する．このとき，孤立点のみからなる提携が存在しない，つまり，クリークとスターのみからなる社会効用最大提携構造が存在することを示す．
From Lemmas~\ref{lem:opt:diam2} and \ref{lem:opt:diam3}, there exists a maximum utilitarian welfare partition where each coalition induces either an isolated vertex, a clique, or a star.
We show that there is no coalition which induces an isolated vertex; i.e., there is a maximum utilitarian welfare partition where each coalition induces a clique or a star.
%孤立点のみからなる提携$C^*_i \in \C^*$が存在すると仮定する．このとき，$C^*_i$に隣接する提携を$C^*_j$とすると，$C^*_j$は孤立点，クリーク，スターのいずれかである．
Assume that there exists a coalition $C^*_i \in \C^*$ induces an isolated vertex. Let $C^*_j$ be the coalition adjacent to $C^*_i$, $C^*_j$ is either an isolated vertex, a clique, or a star.

%$C^*_j$が孤立点であるとき，$\sw(C^*_i)+\sw(C^*_j)=0$であり，$C'=C^*_i\cup C^*_j$とすると，$\sw(C')=1$より，提携$C^*_i$と$C^*_j$を併合してサイズ2のクリークにすることで社会効用が大きくなるので，$\C^*$が社会効用最大提携構造であることに矛盾する．このとき，提携$C'$はサイズ2のクリークとなっている．
%この場合の例を図\ref{}に示す．
When $C^*_j$ induces a isolated vertex, $\uw(C^*_i)+\uw(C^*_j)=0$.
Denote with $C'=C^*_i\cup C^*_j$, we can increase the utilitarian welfare to merge $C^*_i$ and $C^*_j$ because $C'$ induces a clique whose size is two and $\uw(C')=1$.
This contradicts the assumption that $\C^*$ is a maximum utilitarian welfare partition.

%$C^*_j$がクリークであるとき，そのサイズを$x$とすると，$\sw(C^*_i)+\sw(C^*_j)=0+x-1=x-1$である．グラフ$G$がブロックグラフであることより，$G[C^*_i\cup C^*_j]$はブロックスプリットグラフであり，補題\ref{lem:blocksplit:opt}より，社会効用を下げることなくスターまたはクリークからなる提携に分割することができる．
When $C^*_j$ induces a clique, let $x$ be its size, then $\uw(C^*_i)+\uw(C^*_j)=0+x-1=x-1$.
Since $G$ is a block graph, $G[C^*_i\cup C^*_j]$ is a block split graph. From Lemma~\ref{lem:blocksplit:opt}, we can split $C^*_i\cup C^*_j$ into a star or a clique without decreasing the utilitarian welfare.
%この場合の例を図\ref{}に示す．

%$C^*_j$がスターであるとき，$v\in C^*_i$が隣接しているのは，$C^*_j$の葉である1頂点のみ，葉である1頂点と中心点，中心点のみいずれかである．$C^*_j$の葉の数を$l$とすると，$\sw(C^*_i)+\sw(C^*_j)=0+2l/(l+1)=2l/(l+1)$である．
When $C^*_j$ induces a star, $v\in C^*_i$ is adjacent to either only one vertex that is a leaf of $C^*_j$, one of the leaf and the center of $C^*_j$, or only the center of $C^*_j$. Let $l$ be the number of leaves in $C^*_j$, then $\uw(C^*_i)+\uw(C^*_j)=0+2l/(l+1)=2l/(l+1)$.
%$v$が$C^*_j$の葉である1頂点のみと隣接しているとき，$v\in C^*_i$が隣接する$C^*_j$内の頂点を$u\in C^*_j$，提携$C_{\alpha}$を$C_{\alpha}=\{v\}\cup\{u\}$とする．このとき，提携$C_{\beta}$を$C_{\beta}=C^*_j\setminus \{u\}$とすると，$C_{\alpha}$はサイズ2のクリークであり，$C_{\beta}$は葉の数が$l-1$のスターである．よって，$\sw(C_{\alpha})+\sw(C_{\beta})=1+2(l-1)/l$である．
When $v$ is adjacent to only one vertex that is a leaf of $C^*_j$, let $u\in C^*_j$ be the vertex which $v\in C^*_i$ is adjacent to. Let $C_{\alpha}=\{v\}\cup\{u\}$ and $C_{\beta}=C^*_j\setminus \{u\}$, then $C_{\alpha}$ is a clique whose size is 2 and $C_{\beta}$ is a star with $l-1$ leaves. Therefore, $\uw(C_{\alpha})+\uw(C_{\beta})=1+2(l-1)/l$.
%したがって，$\sw(C_{\alpha})+\sw(C_{\beta})-(\sw(C^*_i)+\sw(C^*_j))=1+2(l-1)/l-2l/(l+1)=(l+2)(l-1)/l(l+1)>0$となるので，提携$C^*_i$と$C^*_j$を提携$C_{\alpha}$と$C_{\beta}$に分割し直すことで社会効用が大きくなる．これは$\C^*$が社会効用最大提携構造であることに矛盾する．%この場合の例を図\ref{}に示す．
Thus, since $\uw(C_{\alpha})+\uw(C_{\beta})-(\uw(C^*_i)+\uw(C^*_j))=1+2(l-1)/l-2l/(l+1)=(l+2)(l-1)/l(l+1)>0$, we can increase the utilitarian welfare by splitting $C^*_i$ and $C^*_j$ into $C_{\alpha}$ and $C_{\beta}$.
This contradicts the assumption that $\C^*$ is a maximum utilitarian welfare partition.
%$v$が，$C^*_j$の葉である1頂点，及び中心点と隣接しているとき，$G[\{v\}\cup C^*_j]$はブロックスプリットグラフであり，補題\ref{lem:blocksplit:opt}より，$C^*_i$を$C_{\alpha}=\{v\}\cup\{u\}$と$C_{\beta}=C^*_j\setminus \{u\}$に社会効用を下げることなく分割し直すことができる．$v$が，$C^*_j$の葉である1頂点のみと隣接しているときと同様の式から，$C^*_i$を$C_{\alpha}=\{v\}\cup\{u\}$と$C_{\beta}=C^*_j\setminus \{u\}$に社会効用を下げることなく分割し直すことができる．
When $v$ is adjacent to one of the leaf and the center of $C^*_j$, $G[\{v\}\cup C^*_j]$ is a block split graph. Thus from Lemma~\ref{lem:blocksplit:opt}, we can split $C^*_i$ into $C_{\alpha}=\{v\}\cup\{u\}$ and $C_{\beta}=C^*_j\setminus \{u\}$ without decreasing the utilitarian welfare.
%$v$が，$C^*_j$の中心点のみと隣接しているとき，提携$C'$を$C'=C^*_i\cup C^*_j$とすると$C'$もスターであり，社会効用は$\sw(C')=2(l+1)/(l+2)$である．$\sw(C')-(\sw(C^*_i)+\sw(C^*_j))=2(l+1)/(l+2)-2l/(l+1)=2/(l+1)(l+2)$なので，提携$C^*_i$と$C^*_j$を併合して，葉の数が$l+1$のスターにすることで，社会効用を大きくすることができる．これは$\C^*$が社会効用最大提携構造であることに矛盾する．
%この場合の例を図\ref{}に示す．
When $v$ is adjacent to only the center of $C^*_j$, let $C'=C^*_i\cup C^*_j$ then $C'$ is also a star and $\uw(C')=2(l+1)/(l+2)$. Since $\uw(C')-(\uw(C^*_i)+\uw(C^*_j))=2(l+1)/(l+2)-2l/(l+1)=2/(l+1)(l+2)$, we can increase the utilitarian welfare by merging $C^*_i$ and $C^*_j$ into a star with $l+1$ leaves.
%よって，孤立点のみからなる提携$C^*_i \in \C^*$が存在すると仮定すると，$C^*_j$がスターであるときについても，$\C^*$が社会効用最大提携構造であることに矛盾する．
Therefore, assuming that there exists a coalition $C^*_i\in\C^*$ which induces a isolated vertex, it contradicts that $\C^*$ is a maximum utilitarian welfare partition, even when $C^*_j$ induces a star.

%以上より，孤立点のみからなる提携を含まない社会効用最大提携構造が存在する．
In this way, we show that there exists a maximum utilitarian welfare partition that does not include coalitions which induces a isolated vertex.\qed
\end{proof}

%補題\ref{lem:induce:block}，
%補題\ref{lem:opt:diam2}，補題\ref{lem:opt:diam3}，補題\ref{lem:opt:isol}より，次の定理が成り立つ．
%From Lemmas~\ref{lem:opt:diam2}, \ref{lem:opt:diam3} and \ref{lem:opt:isol}, the following theorem holds.
\end{comment}

\subsection{Algorithm}
In this subsection, we give a polynomial-time algorithm based on dynamic programming using optimal coalition structures shown in Theorem~\ref{thm:block:opt}. To design a DP-based algorithm, we first define the block-cut tree of a graph.

\subsubsection{Block-cut tree}\label{subsubsec:block-cut}
%グラフ$G=(V,E)$をブロックグラフとする．$G$に含まれる極大クリークの集合を$\mathcal{B}=\{B_1,\ldots,B_\beta\}$とする．なお各クリーク$B$を点集合とみなすことにする．$G$における関節点の集合を$\cC=\{c_1,\ldots,c_{\gamma}\}$とする．これらに対し，$\mathcal{X}=\mathcal{B}\cup\mathcal{C}$をノード集合とした，ブロックグラフ$G$がなす木構造$\mathcal{T}(G)$を$\mathcal{T}=(\mathcal{X},\mathcal{E})$で定める．ただし，$\mathcal{E}=\left\{\{B,c\}\mid  B\in\mathcal{B},c\in\mathcal{C}: c \in B \right\}$である．対象とするグラフ$G$が明らかな場合，$\mathcal{T}(G)$を単に$\mathcal{T}$と書くことにする．ここで，$\mathcal{T}$において各$B\in \mathcal{B}$をブロックノード，各$c\in\mathcal{C}$を関節ノードと呼ぶ．便宜上，$\cT$を適当なブロックノード$B_r$を根とした根付き木とみなすことにする．すなわち，$\mathcal{T}$によって，$\mathcal{X}$の頂点の親子関係や子孫・祖先関係が定められる．$\cT$上で頂点$x\in \cX$とその子孫からなる部分木を$\mathcal{T}_{x}(G)$で表す．また$C_{\cT}(x)$を$\cT$における$x\in \cX$の子ノードの集合とする．また$\cT_x$に対応する$G$の頂点集合を$V_x$で表すことにする．このとき$\cT_x$に対応する$G$の部分グラフを$G[V_x]$で表すことができる．
For a block graph $G=(V,E)$, let $\mathcal{B}=\{B_1,\ldots,B_\beta\}$ be the set of maximal cliques, called \emph{blocks}, in $G$ and $\cC=\{c_1,\ldots,c_{\gamma}\}$ be the set of cut vertices in $G$. Then the \emph{block-cut tree} $\mathcal{T}(G) = (\mathcal{X}, \mathcal{E})$ of $G$ is a tree such that $\mathcal{X}=\mathcal{B}\cup\mathcal{C}$ and each edge in $\mathcal{E}$ connects a block $B\in \mathcal{B}$ and a cut vertex $c\in \mathcal{C}\cap B$.
For simplicity, we sometimes write $\mathcal{T}$ instead of $\mathcal{T}(G)$. 
We call $B\in \mathcal{B}$ a block node and $c\in \mathcal{C}$ a cut node of $\mathcal{T}$. 
For convenience, we consider a block-cut tree rooted by a block node $B_r$. We denote by $\mathcal{T}_{x}(G)$ a subtree consisting of a node $x\in \cX$ and its descendants on $\cT$, by $p_{\cT}(x)$ the parent node of $x\in \cX\setminus \{B_r\}$, and by $C_{\cT}(x)$ the set of children nodes of $x\in \cX$ in $\cT$ (see Figures~\ref{fig:tree:decomposition1} and \ref{fig:tree:decomposition2}). We also denote by $V_x$ the set of vertices in $G$ corresponding to $\cT_x$ and by $G[V_x]$ the induced subgraph of $G$ corresponding to $\cT_x$. For each block node $B\in \mathcal{B}\setminus \{B_r\}$ and its parent node $p_{\cT}(B)\in \mathcal{C}$, $c_p$ denotes the cut vertex in $B\cap p_{\cT}(B)$.
%また，$P_{\cT}(x)$を$\cT$における$x\in \cX$の親ノードとする．極大クリーク（ブロック）$B$を関節点とそれ以外の点$S(B):=B\setminus \cC$に分けると，ブロックグラフでは$S(B)$内の点は$B$内の点としか隣接しない．ブロックグラフに対する木構造の例を図\ref{fig:tree:decomposition}に示す．
For $B\in \mathcal{B}$, we define $R(B):=B\setminus\cC$ as the set of non-cut vertices in $B$.
For a rooted block-cut tree, its leaves are block nodes.
% Dividing the maximal clique $B$ into cut vertices and other vertices $R(B):=B\setminus\cC$, vertices in $R(B)$ are only adjacent to vertices in $B$ in the block graph. An example of a tree structure for a block graph is shown in Figures ~\ref{fig:tree:decomposition1} and \ref{fig:tree:decomposition2}.
\begin{figure}[htb]
\begin{tabular}{cc}
\begin{minipage}{0.45\hsize}
\centering
\includegraphics[width=\textwidth]{treedecomposition1.pdf}
\caption{Example of a block graph.} \label{fig:tree:decomposition1}
\end{minipage}
\begin{minipage}{0.45\hsize}
\centering
\includegraphics[width=\textwidth]{treedecomposition2.pdf}
\caption{The corresponding tree structure of block graph in Figure \ref{fig:tree:decomposition1}.}\label{fig:tree:decomposition2}
\end{minipage}
\end{tabular}
\end{figure}


\subsubsection{Defining recurrence relations}
%Now, we construct the algorithm to compute a social optimum in which each coalition induces a clique or a star. First, we prove that for such optimal coalition structure, the following lemma holds. 
%この結果を利用して，以下では各提携がサイズ2以上のクリークまたはスターのいずれかになるような社会効用最大提携構造を求めることを考える．$\mathcal{T}(G)$におけるクリークノードと関節ノードに対する漸化式を定義し，葉から順に適用していくことで，もとのブロックグラフ$G$の社会効用最大提携構造の総効用を求める動的計画法を設計する．
By Theorem~\ref{thm:block:opt}, we design a dynamic programming algorithm on block-cut trees to find an optimal coalition structure such that each coalition is either a clique of size at least 2 or a star. 
%We design dynamic programming by defining recurrence relation for the clique nodes and cut nodes in $\mathcal{T}(G)$ and applying them in order starting from the leaf nodes.

%$\texttt{T}_B=\{\iso,\cl,\stc,\stl\}$とする．これは，各カット点$x\in B_x$が動的計画法の途中で提携内でどのような構造をとっているのかを表す．具体的には，$\iso$は$x$が属する提携が孤立点であること，$\cl$は$x$が属する提携がサイズ2以上のクリークであること，$\stc$は$x$が属する提携がスターであり，かつ$x$がその中心であること，$\stl$は$x$が属する提携がスターであり，かつ$x$がその葉であることを表す．図\ref{fig:T_B}に$\texttt{T}_B$のイメージを示す．
We define $\texttt{T}_B=\{\iso,\cl,\stc,\stl\}$ as the set of states of a cut vertex $x\in B_x\cap \mathcal{C}$ that represents the role of $x$ within the coalition containing $x$ in the intermediate steps of the algorithm for a block node. For a coalition structure $\PP_x$ of $G[V_x]$, $\iso$ means that $x$ is a singleton in $\PP_x$, $\cl$  means that $x$ belongs to a coalition that forms a clique of size at least 2 in $\PP_x$, $\stc$ means that  $x$ belongs to a coalition that forms a star (not a singleton) and $x$ is its center in $\PP_x$, and $\stl$ means that $x$ belongs to a coalition that forms a star (not a singleton) and $x$ is its leaf in $\PP_x$. Figure~\ref{fig:T_B} shows the role of $x\in B_x\cap \mathcal{C}$ with respect to $\texttt{T}_B$.
\begin{figure}[htb]
\centering
\includegraphics[width=\textwidth]{typeB.pdf}
\caption{The role of $x\in B_x\cap \mathcal{C}$ with respect to $\texttt{T}_B$.} \label{fig:T_B}
\end{figure}

%また，$\texttt{T}_c=\{\iso, \cl, \stc_l,\stcu_l,\stl\}$（ただし，$c\in\cC$，$1\le l\le|C_{\cT}(c)|$）とする．これは，各カット点$c\in B_x\setminus\{x\}$が動的計画法の途中で提携内でどのような構造をとっているのかを表す．具体的には，$\iso,\cl,\stl$は$\texttt{T}_B$における定義と同様であり，$\stc_l,\stcu_l$は共に$c$が属する提携が$c$を中心とするスターであり，$V_c$の中から葉として$l$個の頂点を取るものであることを表す．ただし，$\stc$は$c$が$P_{\cT}(c)$内の頂点から葉を取らないこと，$\stcu$は$c$が$P_{\cT}(c)$内の頂点から葉を取ることを表す．つまり，$\stc_l$であれば$c$が属する提携は$c$を中心とする葉数$l$のスターであり，$\stcu_l$であれば$c$が属する提携は$c$を中心とする葉数$l+1$のスターである．図\ref{fig:T_B}に$\texttt{T}_c$のイメージを示す．
We also define $\texttt{T}_c=\{\iso,\cl,\stc_1,\ldots, \stc_{|C_{\cT}(c)|},\stcu_1,\ldots, \stcu_{|C_{\cT}(c)|}, \stl\}$ as  the set of states of a cut vertex $c\in \mathcal{C}$  that represents the role of a cut vertex $c$ in the intermediate step of the algorithm for a cut node.
The states $\iso$, $\cl$, $\stl$ are the same meaning as the ones in $\texttt{T}_B$. The states $\stc_l$ and $\stcu_l$ denote that the cut vertex $c$ is the center vertex in the coalition that forms a star with $l$ leaves in $G[V_c]$. The difference  between them is that $\stc_l$ denotes that the coalition  to which $c\in \mathcal{C}$ belongs only contains vertices in $V_c$ whereas $\stcu_l$ denotes that the coalition  to which $c\in \mathcal{C}$ belongs \emph{will} contain one vertex in the parent node $p_{\mathcal{T}}(c)\in \mathcal{B}$ as a leaf. Note that since the coalition forms a star and $p_{\mathcal{T}}(c)$ forms a clique, it can contain at most one vertex in $p_{\mathcal{T}}(c)$. Furthermore, if $c$ takes the state $\stc_l$, then the final coalition containing $c$ forms a star with $l+1$ leaves whose center is $c$.
Figure~\ref{fig:T_c} shows the role of $x\in B_x\cap \mathcal{C}$ with respect to types in $\texttt{T}_c$.
\begin{figure}[htb]
\centering
\includegraphics[width=\textwidth]{typec.pdf}
\caption{The role of $x\in B_x\cap \mathcal{C}$ with respect to $\texttt{T}_c$.} \label{fig:T_c}
\end{figure}

%$f^*(B_x,\typeB,k)$は，$G[V_{B_x}]$における以下の条件を満たす提携構造の中での最大社会効用を表す: 
Now, we define the recurrence relations for block nodes and cut nodes. 
For block nodes, we define $f^*(B_x,\typeB,k)$ as the maximum utilitarian welfare among coalition structures in $G[V_{B_x}]$ that satisfies the following condition: 
\begin{itemize}
    %\item ブロックノード$B$のカット点$x$が属する提携内での役割が$\typeB\in \{\iso, \cl, \stc,\stl\}$. 
    \item $x$ is the cut node of $B$ and the role of the $x$ within the coalition to which $x$ belongs is $\typeB\in \{\iso, \cl, \stc,\stl\}$.
    %\item $B$が子を持つならば，$C_{\cT}(B_x)$に属する関節点のうちちょうど$k$個が各部分木内の頂点とは提携を形成しない，かつその他の$C_{\cT}(B_x)$に属する関節点はいずれも\underline{各部分木内の頂点を含み}提携を形成する．
    %\item  If $B$ has children, then exactly $k$ cut nodes belonging to $C_{\cT}(B_x)$ do not form coalitions with vertices in each subtree, and all other cut nodes belonging to $C_{\cT}(B_x)$ form coalitions with vertices in each subtree.
     %\item $C_{\cT}(B_x)\neq\emptyset$ならば，
    %\begin{itemize}
    %    \item $V_c\setminus \{c\}$の頂点と提携を形成しない頂点が$C_{\cT}(B_x)$にちょうど$k$個存在，
    %    \item それ以外の$C_{\cT}(B_x)$内の頂点が属する提携はそれぞれ$V_c\setminus \{c\}$の頂点を\underline{少なくとも一つ含む}．
    %\end{itemize}
    \item if $C_{\cT}(B_x)\neq\emptyset$, for $c\in C_{\cT}(B_x)$
    \begin{itemize}
    \item There are exactly $k$ vertices in $C_{\cT}(B_x)$ that do not form a coalition with a vertex in $V_c\setminus \{c\}$.
    \item Each coalition to which other vertices in $C_{\cT}(B_x)$ belongs includes at least one vertex in $V_c\setminus \{c\}$.
    \end{itemize}
\end{itemize}


%$g^*(c,\typec)$は，$\typec\in\{\iso,\cl,\stc_l,\stl\}$のとき$G[V_c]$における，$\typec=\stcu_l$のとき$G[V_c\cup\{v\}]$（ただし$v$は$P_{\cT}(c)$内の頂点で$c$を中心点とするスターの葉となる頂点とする）における以下の条件を満たす提携構造の中での最大社会効用を表す：
%$g^*(c,\typec)$ denotes the maximum social welfare in the coalition structures in $G[V_c]$ when $\typec\in\{\iso,\cl,\stc_l,\stl\}$, and in $G[V_c\cup\{v\}]$ when $\typec=\stcu_l$ (note that $v$ is the vertex in $P_{\cT}(c)$ that is the leaf of a star centered at $c$) that satisfies the following condition: 
%\begin{itemize}
    %\item 関節ノード$c$が属する提携内での役割が$\typec\in \{\iso, \cl, \stc_1,\ldots,\stc_{|C_{\cT}(c)|},\stcu_1,\ldots,\stcu_{|C_{\cT}(c)|},\stl\}$.
 %   \item The role within the coalition to which the cut node $c$ belongs is $\typec\in \{\iso, \cl, \stc_1,\ldots,\stc_{|C_{\cT}(c)|},\stcu_1,\ldots,\stcu_{|C_{\cT}(c)|},\stl\}$.
%\end{itemize}

%カット点$c\in C$と$\typec\in\{\iso,\cl,\stc_1,\ldots,\stc_{|C_{\cT}(c)|},\stl\}$に対して，$g^*(c,\typec)$を$c$の役割が$\typec$であるような$G[V_c]$の提携構造の最大社会効用とする．
For the cut node $c\in C$ and $\typec\in\{\iso,\cl,\stc_1,\ldots,\stc_{|C_{\cT}(c)|},\stl\}$, let $g^*(c,\typec)$ be the maximum utilitarian welfare in the coalition structures in $G[V_c]$ in which the role of $c$ is $\typec$.

%また，$g^*(c,\stcu_l)$は，カット点$c\in C$が$P_{\cT}(c)$内の頂点から葉$v_l$を取りスターとなるときの$G[V_{c_{\textrm{center}}}\cup\{v_l\}]$部分の社会効用を表し，
Also, $g^*(c,\stcu_l)$ denotes the maximum utilitarian welfare in the $G[V_{c}\cup\{v_l\}]$ when the cut node $c\in C$ becomes the center of a star with $l$ leaves $v_1,\ldots, v_{l-1}\in V_c$ and $v_l\in P_{\cT}(c)$.
Then we can compute $g^*(c,\stcu_l)$ from $g^*(c,\stc_l)$ as follows:
\begin{align*}
g^*(c,\stcu_l)=g^*(c,\stc_l)-\frac{2l}{l+1}+\frac{2l+1}{l+2}=g^*(c,\stc_l)+\frac{2}{(l+1)(l+2)}.
\end{align*}
Note that $\frac{2l}{l+1}$ and $\frac{2l+1}{l+2}$ are the utilitarian welfare of a star with $l$ leaves and a star with $l+1$ leaves, respectively. Thus, $\frac{2l+1}{l+2}-\frac{2l}{l+1}$ denotes the increase of the utilitarian welfare when a leaf is added to a coalition that forms a star with $l$ leaves.

%$g^*(c,\fin)=\max_{\typec\in\{\cl,\stc_1,\ldots,\stc_|C_{\cT}(c)|,\stl\}}g^*(c,\typec)$とする．条件を満たす提携構造が存在しない場合は，$f^*(B,\typeB,k)=-\infty$，$g^*(c,\typec)=-\infty$とする．以下では，$f^*(B,\typeB,k)$，$g^*(c,\typec)$を$\mathcal{T}$上における動的計画法で計算する．
Let $g^*(c,\fin)=\max_{\typec\in\{\cl,\stc_1,\ldots,\stc_|C_{\cT}(c)|,\stl\}}g^*(c,\typec)$. If there is no coalition structure that satisfies the condition, let $f^*(B,\typeB,k)=-\infty$, \\$g^*(c,\typec)=-\infty$. In the following, we compute $f^*(B,\typeB,k)$ and $g^*(c,\typec)$ by dynamic programming on $\mathcal{T}$.




\subsubsection{Recurrence relation in the block nodes}
First, we prove that for such an optimal coalition structure, the following lemma holds. 
%$\mathcal{T}$において，カットノード$c\in \mathcal{C}$の親ノードを$B\in \mathcal{B}$とする．このとき以下の補題が成立する．
In $\mathcal{T}$, let $B\in \mathcal{B}$ be the parent node of the cut node $c\in \mathcal{C}$. Then, the following lemma holds.

\begin{lemma}\label{scu:num}
% 最適提携構造において，任意の$B$について，$C_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つである．
In the optimal coalition structure, for any $B$, there is at most one cut vertex belonging to $C_{\cT}(B)$ that is the center of the star that has both vertices in $V_{C_{\cT}(B)}$ and in $B$ as leaves. 
\end{lemma}

\begin{proof}
%背理法で示す．スターの中心点で$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするような$C_{\cT}(B)$に属する頂点が$t(\ge2)$個存在したとする．これらのスターを$P_1,\ldots,P_t$，それぞれの中心点を$c_1,\ldots,c_t$，葉の数を$l_1+1,\ldots,l_t+1$とする．今，$P_1,\ldots,P_t$が葉とする$B$内の頂点がそれぞれ$P_1,\ldots,P_t$から逸脱して1つのクリークになることを考える．このとき，$P_1,\ldots,P_t$は葉の数が1つずつ少ないスターになり，それぞれを$P'_1,\ldots,P'_t$とすると，$l_1,\ldots,l_t\ge1$より，逸脱前後の社会効用の差は，
%By way of contradiction, let us assume 
For a contradiction, suppose that there are $t(\ge2)$ vertices belonging to $C_{\cT}(B)$ that is the center of the star which has both vertices in $V_{C_{\cT}(B)}$ and in $B$ as leaves. Let $S_1,\ldots,S_t$ be these stars, $c_1,\ldots,c_t$ be the center of $S_1,\ldots,S_t$, and be $l_1+1,\ldots,l_t+1$ be the number of leaves of $S_1,\ldots,S_t$. Now we consider that each vertex in $B$ which is the leaves of $S_1,\ldots,S_t$ deviates from $S_1,\ldots,S_t$ and form a single clique together. Then, $S_1,\ldots,S_t$ becomes a star with one less leaf each, and denote with $S'_1,\ldots,S'_t$. Since $l_1,\ldots,l_t\ge1$, the difference in social welfare before and after deviation is
\begin{align*}
 &\uw(S_1)+\cdots+\uw(S_t)-(\uw(S'_1)+\cdots+\uw(S'_t)+t-1)\\
= &\uw(S'_1)+\cdots+\uw(S'_t)+\frac{2}{(l_1+1)(l_1+2)}+\cdots+\frac{2}{(l_t+1)(l_t+2)}\\
 &-(\sw(S'_1)+\cdots+\uw(S'_t)+t-1)\\
\le & -\frac{2}{3}t+1<0, 
\end{align*}
%となる．よって，最適性に矛盾する．
%We get a contradiction.
which contradicts the optimality. 
\qed
\end{proof}

%補題\ref{scu:num}より，$f^*(B_x,\typeB,k)$を実現する提携構造において$\stcu$である$C_{\cT}(B_x)$内の頂点は高々1つである．よって，提携構造に$\stcu$である$C_{\cT}(B_x)$内の頂点が存在しないときと1つ存在するときに場合分けをしてそれぞれの社会効用の最大値を考え，さらにそれらの最大値を求めることで，$f^*(B_x,\typeB,k)$の値を計算する．
From Lemma~\ref{scu:num}, there is at most one node whose role is $\stcu$ in the coalition structure that realizes $f^*(B_x,\typeB,k)$. Therefore, we divide the cases where there is no vertex in $C_{\cT}(B_x)$ whose role is $\stcu$ and where there is one to compute the value of $f^*(B_x,\typeB,k)$. Then, we consider the maximum value of each social welfare, and find their maximum values.
%はじめに，$\stcu$である$C_{\cT}(B_x)$内の頂点が存在しない場合について考える．まず，補助関数$f(B_x,\typeB,i,k)$を定義する．$x_1, x_2, \ldots, x_i \in C_{\cT}(B_x)$に対して，$f(B_x,\typeB,i,k)$は，$G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$の提携構造のうち以下の条件を満たすものの最大社会効用を表す：(i) $x$のタイプが$\typeB$, (ii) $B_x$に属する関節点$x_1, x_2, \ldots, x_i$のうち，ちょうど$k$個が各部分木内の頂点とは提携を形成しない，かつその他のちょうど$i-k$個の関節点は\underline{各部分木内の点のみと}提携を形成している，
%つまり$\stcu_l$である$C_{\cT}(B_x)$内の頂点が存在しない．なお$0\le k\le i \le |C_{\cT}(B_x)|$である．すると，$\stcu$である$C_{\cT}(B_x)$内の頂点が存在しない場合の社会効用の最大値は，$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$で表すことができる．図\ref{fig:f}に$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$のイメージを示す．
First, we consider the case where there is no node in $C_{\cT}(B_x)$ whose roll is $\stcu$. Define an auxiliary function $f(B_x,\typeB,i,k)$ as follows. 
For $x_1, x_2, \ldots, x_i \in C_{\cT}(B_x)$, $f(B_x,\typeB,i,k)$ represents the maximum utilitarian welfare in the coalition structure in $G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$ that satisfies the following conditions : 
\begin{itemize}
 \item The role of $x$ is $\typeB$. 
 %\item $x_1, x_2, \ldots, x_i\in C_{\cT}(B_x)$のうち，$V_{x_i}\setminus\{x_i\}$の頂点と提携を形成しない頂点がちょうど$k$個，それ以外の$i-k$個はそれぞれ$V_{x_i}\setminus \{x_i\}$の頂点\underline{のみと}提携を形成している．
 \item Exactly $k$ cut nodes in $x_1, x_2, \ldots, x_i$ do not form coalitions with vertices in $V_{x_j}\setminus\{x_j\}$, and exactly $i-k$ other cut nodes in $x_1, x_2, \ldots, x_i$ form coalitions only with vertices in $V_{x_j}\setminus \{x_j\}$. 
\end{itemize}
%なお$0\le k\le i \le |C_{\cT}(B_x)|$である．すると，$\stcu$である$C_{\cT}(B_x)$内の頂点が存在しない場合の社会効用の最大値は，$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$で表すことができる．
Note that $0\le k\le i \le |C_{\cT}(B_x)|$. Then, the maximum utilitarian welfare when there is no nodes in $C_{\cT}(B_x)$ whose role is $\stcu$ can be expressed by $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$. 
%Figure\ref{fig:f} shows an image of $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f.jpg}
%\caption{The image of $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$} \label{fig:f}
%\end{figure}

%次に，$\stcu$である$C_{\cT}(B_x)$内の頂点が1つ存在する場合について考える．まず，$\stcu$である$C_{\cT}(B_x)$内の頂点とその葉となる$B_x$内の頂点を決め打つ．ここで，$\stcu$である$C_{\cT}(B_x)$内の頂点は，葉として$B_x$内からは1頂点のみをとる．よって，$\stcu$である$C_{\cT}(B_x)$内の頂点とその葉となる$B_x$内の頂点の組は高々$\Delta^2$通りである．$\stcu$である$C_{\cT}(B_x)$内の頂点を$c_{\textrm{center}}$，$c_{\textrm{center}}$の葉となる$B_x$内の頂点を$v_l$として，補助関数$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$を定義する．$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$は，$c_{\textrm{center}}$と$v_l$を決め打ちしたとき，$G[V(B_x)]$の提携構造のうち以下の条件を満たすものの最大社会効用を表す：
Next, we consider the case where there is one vertex in $C_{\cT}(B_x)$ whose role is $\stcu$. First, fix the vertex in $C_{\cT}(B_x)$ whose role is $\stcu$ and the vertex in $B_x$ that is its leaf. Note that, there are at most $\Delta^2$ pairs of vertices in $C_{\cT}(B_x)$ in which the role of one node is $\stcu$ and the other node becomes its leaves since the node in $C_{\cT}(B_x)$ whose role is $\stcu$ takes only one vertex from $B_x$ as a leaf. 
Let $c_{\textrm{center}}$ be a node in $C_{\cT}(B_x)$ whose role is $\stcu$ and $v_l$ be a vertex in $B_x$ that is a leaf of the star centered $c_{\textrm{center}}$. We define an auxiliary function $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$. The $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$ represents the maximum social welfare in the coalition structures in $G[V(B_x)]$ that satisfies the following conditions when $c_{\textrm{center}}$ and $v_l$ are fixed:
%(i) $x$のタイプが$\typeB$,
%(ii) $c_{\textrm{center}}$のタイプが$\stcu$，かつ$c_{\textrm{center}}$は$v_l$を葉にもつ,
%(iii) $x_1, x_2, \ldots, x_{|C_{\cT}(B_x)|}\in C_{\cT}(B_x)$について，$c_{\textrm{center}}=x'_1$とし，残りの頂点を$v_l\in S(B_x)\cup\{x\}$であればラベルの昇順に$x'_2,\ldots, x'_{|C_{\cT}(B_x)|}$，$v_l\in C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$であれば$v_l=x'_2$としたのち残りの頂点をラベルの昇順に$x'_3,\ldots, x'_{|C_{\cT}(B_x)|}$としたとき，$x'_1,x'_2,\ldots, x'_i \in C_{\cT}(B_x)$のうちちょうど$k$個が各部分木内の頂点とは提携を形成しない，かつその他のちょうど$i-k$個の関節点は\underline{各部分木内の点を含み}提携を形成している．
\begin{itemize}
    \item The role of $x$ is $\typeB$. 
    \item The role of $c_{\textrm{center}}$ is $\stcu$ and $v_l$ belongs to the same coalition as $c_{\textrm{center}}$ as a leaf. 
    \item For $x_1, x_2, \ldots, x_{|C_{\cT}(B_x)|}\in C_{\cT}(B_x)$, let $c_{\textrm{center}}=x'_1$, and if $v_l\in R(B_x)\cup\{x\}$, let the remaining nodes be $x'_2,\ldots, x'_{|C_{\cT}(B_x)|}$ in ascending order of label, and if $v_l\in C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$, let $v_l=x'_2$ and the remaining nodes be $x'_3,\ldots, x'_{|C_{\cT}(B_x)|}$ in ascending order of label. Then exactly $k$ vertices in $x'_1,x'_2,\ldots, x'_i \in C_{\cT}(B_x)$ do not form coalitions with vertices in $V_{x_j}\setminus\{x_j\}$, and exactly other $i-k$ cut nodes form coalitions with vertices in $V_{x_j}\setminus\{x_j\}$.
\end{itemize}
%図\ref{fig:f_center}に$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$のイメージを示す．
%Figure\ref{fig:f_center} shows the image of $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_center.jpg}
%\caption{The image of $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$} \label{fig:f_center}
%\end{figure}


%ただし，$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$については，$v_l\in S(B_x)$であれば，最初に$c_{\textrm{center}}$と$v_l$をセットして，その後$G[V_{B_x}\setminus V_{c_{\textrm{center}}}\setminus\{v_l\}]$について$C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$の頂点のうち$k$個が$C_{\cT}(x'_j)$内の頂点と提携を形成しないときの社会効用の最大値を$f(B_x,\typeB,i,k)$の計算と同様の方針で計算する．また，$v_l\in C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$であれば，方針は同様であるが$v_l$のタイプが$\iso$となるので，$C_{\cT}(B_x)\setminus\{c_{\textrm{center}},v_l\}$の頂点のうち$k-1$個が$C_{\cT}(x'_j)$内の頂点と提携を形成しないときの社会効用の最大値を計算することに注意する．以下では，$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$を動的計画法で計算する．
%However, for $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$, if $v_l\in S(B_x)$, we first set $c_{\textrm{center}}$ and $v_l$, and then compute the maximum social welfare in $G[V_{B_x}\setminus V_{c_{\textrm{center}}}\setminus\{v_l\}]$ when $k$ nodes in $C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$ do not form coalitions with the vertices in $C_{\cT}(x'_j)$. This computation can be done in same way as computing $f(B_x,\typeB,i,k)$. If $v_l\in C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$, the policy is the same, but since the type of $v_l$ is $\iso$, note that we compute the maximum social welfare when $k-1$ nodes in $C_{\cT}(x'_j)$ do not form coalitions with vertices in $C_{\cT}(x'_j)$.In the following, we  compute $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$ by dynamic programming.

%$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$は$f(B_x,\typeB,i,k)$と同様の方針で再帰的に計算できる．$x'_1=c_{\textrm{center}}$を$B_x$内の頂点を葉に持つスターの中心点，$v_l$を$c_{\textrm{center}}$が持つ$B_x$内の葉であると決め打ちしているので，$G[V_{c_{\textrm{center}}}\cup\{v_l\}]$部分の社会効用として，
%\begin{align*}
%g^*(c_{\textrm{center}},\stcu)&=\max_l\{g^*(c_{\textrm{center}},\stcu_l)\}\\
%&=\max_l\left\{g^*(c_{\textrm{center}},\stc_l)+\frac{2}{(l+1)(l+2)}\right\}
%\end{align*}
%を計算する．
Function $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$ can be calculated recursively in the same way as $f(B_x,\typeB,i,k)$. Since we fix $x'_1=c_{\textrm{center}}$ as the center of the star whose leaves have vertices in $B_x$ and $v_l\in B_x$ as the leaf that $c_{\textrm{center}}$ has, the utilitarian welfare in $G[V_{c_{\textrm{center}}}\cup\{v_l\}]$ is
\begin{align*}
g^*(c_{\textrm{center}},\stcu)&=\max_l\{g^*(c_{\textrm{center}},\stcu_l)\}\\
&=\max_l\left\{g^*(c_{\textrm{center}},\stc_l)+\frac{2}{(l+1)(l+2)}\right\}.
\end{align*}
%そして，漸化式においては，$v_l\in R(B_x)\cup\{x\}$であれば，初期化として$x'_1=c_{\textrm{center}}$は$B_x$内の頂点を葉に持つスターの中心点であると決め打ちして，その後$x'_2,\ldots, x'_i \in C_{\cT}(B_x)$うち$V_{x_j}\setminus\{x_j\}$の頂点とは提携を形成しない頂点が$k$個のときの社会効用の最大値を再帰的に計算する．一方，$v_l\in C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$であれば，初期化として$x'_1=c_{\textrm{center}}$の役割を$\stcu$，$x'_2=v_l$の役割を$\iso$と決め打つので，その後の動的計画法では$x'_3,\ldots, x'_i \in C_{\cT}(B_x)$の頂点のうち$k-1$個が$\mathcal{T}_{x'_j}$のノードに対応する頂点とは提携を形成しないときの社会効用の最大値を計算することに注意する．図\ref{fig:f_center}に$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$のイメージを示す．
Then, in the recurrence relation, if $v_l\in R(B_x)\cup\{x\}$, we assume as initialization that $x'_1=c_{\textrm{center}}$ is the center of the star which contains a vertex in $B_x$ as a leaf, and then we recursively compute the maximum utilitarian welfare when exact $k$ vertices in $x'_2,\ldots, x'_i \in C_{\cT}(B_x)$ do not form a coalition with a vertex in $V_{x_j}\setminus\{x_j\}$. 
On the other hand, if $v_l\in C_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$, the role of $x'_1=c_{\textrm{center}}$ is determined as $\stcu$ and the role of $x'_2=v_l$ as $\iso$ as initialization, then in dynamic programming we compute the maximum utilitarian welfare when $k-1$ vertices in $x'_3,\ldots,x'_i \in C_{\cT}(B_x)$ do not form a coalition with a vertex in $V_{x_j}\setminus\{x_j\}$. %Figure\ref{fig:f_center} shows the image of $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$.
%また，$f(B_x,\typeB,i,k)$の計算と同様に，$x$の役割である$\typeB$によって$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$を求める漸化式も異なる．特に，$\typeB\in\{\iso,\cl,\stl\}$のときは$v_l=x$であれば$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)=-\infty$となる．
As with the computation of $f(B_x,\typeB,i,k)$, the recurrence relations computing $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$ also differ depending on $\typeB$. In particular, when $\typeB\in\{\iso,\cl,\stl\}$, $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)=-\infty$ if $v_l=x$.

%さらに，$f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)\}$とすると，各$c_{\textrm{center}}$に対する社会効用の最大値は，$f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$で表すことができる．
Furthermore, if $f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)\\=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)\}$, the maximum utilitarian welfare for each $c_{\textrm{center}}$ can be expressed by $f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$.

%よって，$f^*(B_x,\typeB,k)$は，
Therefore, we have 
\begin{align*}
&f^*(B_x,\typeB,k)\\
&=\max\{f(B_x,\typeB,|C_{\cT}(B_x)|,k),f_{x_1}(B_x,\typeB,|C_{\cT}(B_x)|,k),\\
&\ldots,f_{x_{|C_{\cT}(B_x)|}}(B_x,\typeB,|C_{\cT}(B_x)|,k)\}. 
\end{align*}
%で表される．
%$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$の計算方針は$f(B_x,\typeB,i,k)$の計算方針とほぼ同様なので，以降では，$f(B_x,\typeB,i,k)$を再帰的に計算する方法を示す．
Since $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$ can compute in almost same way as $f(B_x,\typeB,i,k)$, we show only how to compute $f(B_x,\typeB,i,k)$ recursively in the following.



%まずベースケースとして，$i=0$のときを考える．このとき対象となるグラフは$G[\{x\}\cup S(B_x)]$であり，これがクリークをなしていることに注意すると
First, we consider the case when $i=0$ as a base case. In this case, the target graph is $G[\{x\}\cup R(B_x)]$, which is a clique. Then we can obtain 
\begin{align*}
 f(B_x,\typeB,0,0) &= \begin{cases}
0 & \text{if $R(B_x)=\emptyset$}\\ 
|R(B_x)|-1 & \text{if $R(B_x)\neq\emptyset$ \& $\typeB= \iso$}\\ 
|R(B_x)| & \text{if $R(B_x)\neq\emptyset$ \& $\typeB= \cl$}\\
\max\{1,|R(B_x)|-1\} & \text{otherwise}. %\typeB\in\{\stc,\stl\}
\end{cases}
\end{align*}
%が得られる．それぞれ確認する：$S(B_x)=\emptyset$のときは，$G[\{x\}\cup S(B_x)]$は1点のみからなるため，$f=0$となる．$S(B_x)\neq \emptyset$のときは，$\typeB=\iso$のときは$S(B_x)$だけでクリークを構成するのでその効用は$|S(B_x)|-1$となる，$\typeB=\cl$のときは$x$と$S(B_x)$がクリークの形で提携をとり効用は$|S(B_x)|$となる．$\typeB=\stc,\stl$の場合は，$S(B_x)$のうち1点と$x$がスターを形成するかたちをとるため，$|S(B_x)|=1$のときは$1$, $|S(B_x)|>1$のときは$|S(B_x)|-1$の値をとる．
The reason why the above equation holds is as follows: 
When $R(B_x)=\emptyset$, $G[\{x\}\cup R(B_x)]$ consists of only one node, so $f=0$. Considering the case where $R(B_x)\neq \emptyset$. When $\typeB=\iso$, the utilitarian welfare becomes $|R(B_x)|-1$ because $R(B_x)$ forms a clique. When $\typeB=\cl$, $x$ and $R(B_x)$ form a coalition together in a clique and the utilitarian welfare is $|R(B_x)|$. In the case of $\typeB=\stc,\stl$, one node in $R(B_x)$ and $x$ form a star, so the utilitarian welfare is $1$ when $|R(B_x)|=1$ and $|R(B_x)|-1$ when $|R(B_x)|>1$.


%次に$i>0$の場合を考える．
Next, we consider the case when $i>0$. 
%\paragraph{When $\typeB=\iso$}\
\paragraph{Case $\typeB=\iso$:}\ 

We obtain
\begin{align*}
&f(B_x,\iso,i,k)\\
&=
\begin{cases}
f(B_x,\iso,i-1,0)+g^*(x_i,\fin)%c_iはisoでない
& \text{if k = 0}\\
\max\left\{
\begin{array}{c}
f(B_x,\iso,i-1,0)+g^*(x_i,\iso),\\%c_iはiso
f(B_x,\iso,i-1,1)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{if $k=1$ \& $R(B_x)= \emptyset$}\\
\max\left\{
\begin{array}{c}
f(B_x,\iso,i-1,k-1)+g^*(x_i,\iso)+1,\\%c_iはiso
f(B_x,\iso,i-1,k)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise}
\end{cases}
\end{align*}
%となる．
%このようになる理由は次の通りである：$G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i-1} V_{x_j}]$の提携構造の差分を考える．まず$k=0$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．$k>0$に対しては，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．この際，$x_i$が$B_x$内の頂点と同じ提携に入り$k>1$または$S(B)\neq\emptyset$であるならば，$x_i$は他の関節点あるいは$S(B)$の点とクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．$k=1$かつ$S(B)=\emptyset$ならば，関節点$x_i$は他に提携する頂点が存在しないため1頂点からなる提携をなし，社会効用を$1$増やす形はとらない．図\ref{fig:f_iso}に$k=1$かつ$S(B)\neq\emptyset$，または$k>2$(otherwise)のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
Consider the difference in the coalition structure in $G[\{x\}\cup R(B_x)\bigcup_{j=1}^{i} V_{x_j}]$ and $G[\{x\}\cup R(B_x)\bigcup_{j=1}^{i-1} V_{x_j}]$. 
First, when $k=0$, the cut node $x_i$ in $G[V_{x_i}]$ is not in the same coalition with any vertex in $B_x$. 

When $k>0$, the cut node $x_i$ in $G[V_{x_i}]$ can either be in the same coalition with a vertex in $B_x$ ($g^*(x_i,\iso)$) or not ($g^*(x_i,\fin)$), so the one with not smaller utilitarian welfare is adopted. In this case, if $x_i$ is in the same coalition with some vertices in $B_x$ and $k>1$ or $R(B)\neq\emptyset$, $x_i$ will form a clique with other cut nodes or vertices in $R(B)$, so the utilitarian welfare will increase by $1$. If $k=1$ and $R(B)=\emptyset$, there is no other vertices with which $x_i$ form a coalition, so $x_i$ forms a coalition consisting of one vertex and the utilitarian welfare of the relevant part is not increased by $1$. 
%Figure\ref{fig:f_iso} shows the transition when $k=1$ and $R(B)\neq\emptyset$ or $k>2$(otherwise).
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_iso.jpg}
%\caption{The transition when $\typeB=\iso$ ($k=1$ \& $S(B)\neq\emptyset$, or When $k>2$).} \label{fig:f_iso}
%\end{figure}


%\paragraph{When $\typeB=\cl$}\
\paragraph{Case $\typeB=\cl$}\

We obtain
\begin{align*}
f(B_x,\cl,i,k)=&
\begin{cases}
f(B_x,cl,i-1,0)+g^*(x_i,\fin)
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B_x,\cl,i-1,k-1)+g^*(x_i,\iso)+1,\\%c_iはiso
f(B_x,\cl,i-1,k)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise}
\end{cases}
\end{align*}
%$G[\{x\}\cup R\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup R\cup \bigcup_{j=1}^{i-1} V_{x_j}]$の提携構造の差分を考える．まず$k=0$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．ただし，$f(B_x,\cl,|C_{\cT}(B_x)|,k)$は，$k=0$かつ$R=\emptyset$のとき，$x$がサイズ2以上のクリークになり得ないので，$R=\emptyset$であれば$f(B_x,\cl,|C_{\cT}(B_x)|,0)=-\infty$とする．
%$k>0$に対しては，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．この際，$x_i$が$B_x$内の頂点と同じ提携に入るならば$x$及び他の関節点あるいは$R$の点とクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．

The reason why the above equation holds is as follows: 
We consider the difference between the coalition structures in $G[\{x\}\cup R(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$ and $G[\{x\}\cup R(B_x)\cup \bigcup_{j=1}^{i-1} V_{x_j}]$. 
First, when $k=0$, the cut node $x_i$ in $G[V_{x_i}]$ is not in the same coalition with any vertex in $B_x$. 
However, $f(B_x,\cl,|C_{\cT}(B_x)|,k)=-\infty$ when $k=0$ and $R(B_x)=\emptyset$, since $x$ cannot be a clique of size at least 2. 

When $k>0$, since the cut node $x_i$ in $G[V_{x_i}]$ can either be in the same coalition as a vertex in $B_x$ ($g^*(x_i,\iso)$) or not ($g^*(x_i,\fin)$), the one with not smaller utilitarian welfare will be adopted. In this case, if $x_i$ is in the same coalition with some vertices in $B_x$, it will form a clique with $x$ and other cut nodes or vertices in $R(B_x)$, and the utilitarian welfare of the relevant part is increased by $1$. %Figure\ref{fig:f_cl} shows the transition when $k\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_cl.jpg}
%\caption{The transition when $\typeB=\cl$($k\neq0$(otherwise))} \label{fig:f_cl}
%\end{figure}


\paragraph{Case $\typeB=\stc$}\

We obtain
\begin{align*}
&f(B_x,\stc,i,k)\\
&=
\begin{cases}
f(B_x,\stc,i-1,0)+g^*(x_i,\fin)%c_iはisoでない
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B_x,\stc,i-1,1)+g^*(x_i,\iso),\\%c_iはiso
f(B_x,\iso,i-1,2)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
%& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
& \text{if $k\neq 0$ \& $k+|R(B_x)|=2$}\\
\max\left\{
\begin{array}{c}
f(B_x,\stc,i-1,k-1)+g^*(x_i,\iso)+1,\\%c_iはiso
f(B_x,\stc,i-1,k)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise}
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：
%$G[\{x\}\cup R\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup R\cup \bigcup_{j=1}^{i-1}V_{x_j}]$の提携構造の差分を考える．$k=0$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．ただし，$f(B_x,\stc,|C_{\cT}(B_x)|,k)$は，$k=0$かつ$R=\emptyset$のとき$x$がスターの中心点になり得ないので，$R=\emptyset$であれば$f(B_x,\stc,|C_{\cT}(B_x)|,0)=-\infty$とする．
The reason why the above equation holds is as follows: 
We consider the difference between the coalition structures in $G[\{x\}\cup R(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$ and $G[\{x\}\cup R(B_x)\cup \bigcup_{j=1}^{i-1}V_{x_j}]$. 
First, when $k=0$, the cut node $x_i$ in $G[V_{x_i}]$ is not in the same coalition with any vertex in $B_x$. 
However, $f(B_x,\stc,|C_{\cT}(B_x)|,k)=-\infty$ when $k=0$ and $R(B_x)=\emptyset$, since $x$ cannot be the center of a star.

%$k>0$に対しては，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$でないとき，$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$）を考える．$f(B_x,\stc,i,k)$を実現する提携構造で$x$を中心点とするスターの葉となっている頂点を$s_i$とすると，$s_i=x_i$の場合と$s_i=s_{i-1}$の場合が考えられるが，いずれの場合も$x$は$x_i$もしくは$s_{i-1}$を中心点とするサイズ2のスターを形成し，$s_i$以外の関節点及び$R$の点はクリークをなす形で提携するため，社会効用は等しくなる．また，$s_i$以外の関節点及び$R$の点はクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$ならば役割が$\iso$である$C_{\cT}(B_x)$に属する2頂点のうち1点が$x$とスターを形成し，もう1点は1頂点からなる提携を形成するので，社会効用を$1$増やす形はとらない．図\ref{fig:f_stc}に$k>0$で$k=2$かつ$R=\emptyset$以外(otherwise)のときの遷移の様子を示す．
When $k>0$, $x_i$ is either in the same coalition with vertices in $B_x$ ($g^*(x_i,\iso)$) or not ($g^*(x_i,\fin)$), so the one with not smaller utilitarian welfare is adopted.
Consider the case where $x_i$ enters into the same coalition as a vertex in $B_x$ ($g^*(x_i,\iso)$) when $k\neq1$ or $|R(B_x)|\neq1$, or $k\neq2$ or $R(B_x)\neq\emptyset$. Let $s_i$ be the vertex that is the leaf of the star with $x$ as its center in the coalition structure realizing $f(B_x,\stc,i,k)$, then there are two possible cases: $s_i=x_i$ and $s_i=s_{i-1}$. 
In both cases, $x$ forms a star of size 2 with $x_i$ or $s_{i-1}$ as the center point, and the cut nodes except $s_i$ and the vertices in $R(B_x)$ form a clique, so the utilitarian welfare are equal. In addition, since the cut nodes except $s_i$ and the vertices in $R(B_x)$ form a clique, the utilitarian welfare of the relevant part is increased by $1$. 
If $k=1$ and $|R(B_x)|=1$ or $k=2$ and $R(B_x)=\emptyset$, one of the two vertices belonging to $C_{\cT}(B_x)$ whose role is $\iso$ forms a star with $x$ and the other vertex forms a coalition consisting of one vertex, so the utilitarian welfare of the relevant part is not increased by $1$. 
%Figure\ref{fig:f_stc} shows the transition when $k>0$, $k\neq1$ or $|R(B_x)|\neq1$, or $k\neq2$ or $R(B_x)\neq\emptyset$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_stc.jpg}
%\caption{The transition when $\typeB=\stc$(without $k>0$ \& $k\neq1$ or $|R|\neq1$, or $k\neq2$ or $R\neq\emptyset$))} \label{fig:f_stc}
%\end{figure}


%\paragraph{When $\typeB=\stl$}\
\paragraph{Case $\typeB=\stl$}\

We obtain
\begin{align*}
&f(B_x,\stl,i,k)\\
&=
\begin{cases}
f(B_x,\stl,i-1,0)+g^*(x_i,\fin)
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B_x,\stl,i-1,1)+g^*(x_i,\iso),\\%c_iはiso
f(B_x,\iso,i-1,2)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
%& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
& \text{if $k\neq 0$ \& $k+|R(B_x)|=2$}\\
\max\left\{
\begin{array}{c}
f(B_x,\stl,i-1,k-1)+g^*(x_i,\iso)+1,\\%c_iはiso
f(B_x,\stl,i-1,k)+g^*(x_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise.}
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$G[\{x\}\cup R\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup R\cup \bigcup_{j=1}^{i-1}V_{x_j}]$の提携構造の差分を考える．$k=0$かつ $R\neq \emptyset$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．ただし，$f(B_x,\stl,|C_{\cT}(B_x)|,k)$は，$k=0$かつ$R=\emptyset$のとき，$x$がスターの葉になり得ないので，$f(B_x,\stl,|C_{\cT}(B_x)|,0)=-\infty$とする．
The reason why the above equation holds is as follows: 
We consider the difference between the coalition structures in $G[\{x\}\cup R(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$ and $G[\{x\}\cup R(B_x)\cup \bigcup_{j=1}^{i-1}V_{x_j}]$. 
First, when $k=0$, the cut node $x_i$ in $G[V_{x_i}]$ is not in the same coalition with any vertex in $B_x$. 
However, $f(B_x,\stl,|C_{\cT}(B_x)|,k)=-\infty$ when $k=0$ and $R(B_x)=\emptyset$, since $x$ cannot be a leaf of a star. 

%$k>0$のとき，$f(B_x,\stl,i,k)$を実現する提携構造において，$x$は$C_{\cT}(B_x)$に属する頂点のうち役割が$\iso$である頂点あるいは$R$に属する頂点を中心点としたサイズ2のスターを形成している．$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．この際，$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$でなく，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），関節点$x_i$は$x$とスターを形成するあるいは他の関節点及び$R$の点とクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$ならば，関節点$x_i$は他に提携を組む頂点が存在しないため1頂点からなる提携をなし，社会効用を$1$増やす形はとらない．$\typeB=\stl$のときの遷移の様子は，図\ref{fig:f_stc}で示した$\typeB=\stc$のときの遷移の様子と同様である．
When $k\neq0$, in the coalition structure realizing $f(B_x,\stl,i,k)$, $x$ forms a star of size 2 with the vertex belonging to $C_{\cT}(B_x)$ whose role is $\iso$ or the vertex in $R(B_x)$ as center. 
Since the cut node $x_i$ in $G[V_{x_i}]$ can either be in the same coalition with vertices in $B_x$ ($G^*(x_i,\iso)$) or not ($G^*(x_i,\fin)$), the one with not smaller utilitarian welfare is adopted. 
In this case, if $k\neq1$ or $|R(B_x)|\neq1$, or $k\neq2$ or $R\neq\emptyset$, and cut node $x_i$ in $G[V_{x_i}]$ is not in the same coalition with vertices in $B_x$ ($g^*(x_i,\iso)$), $x_i$ forms a star with $x$ or a clique with another cut nodes and vertices in $R(B_x)$, and thus its utilitarian utility is increased by $1$.
If $k=1$ and $|R(B_x)|=1$ or $k=2$ and $R(B_x)=\emptyset$, there is no other vertices with which $x_i$ form a coalition, so $x_i$ forms a coalition consisting of one vertex and the utilitarian welfare of the relevant part is not increased by $1$. 
%The transition when $\typeB=\stl$ is similar to the transition when $\typeB=\stc$ shown in Figure\ref{fig:f_stc}.



\subsubsection{Recurrence relation in the cut nodes}
%$g^*(c,\typec)$を計算するにあたって，補助関数$g(c,\typec,i)$を定義する．$C_{\cT}(c)$に属する頂点を$B_c^1, B_c^2, \ldots, B_c^{|C_{\cT}(c)|}$とする．まず$B_c^1, B_c^2, \ldots, B_c^i \in C_{\cT}(c)$に対して，$g(c,\typec,i)$は，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$における提携構造のうち$c$のタイプが$\typec$であるものの最大効用を表す．また，$l\le i$とする．すると，定義より
To compute $g^*(c,\typec)$, we define an auxiliary function $g(c,\typec,i)$. Let $B_c^1, B_c^2, \ldots, B_c^{|C_{cT}(c)|}$ be the nodes belonging to $C_{\cT}(c)$. First, for $B_c^1, B_c^2, \ldots, B_c^i \in C_{\cT}(c)$, $g(c,\typec,i)$ is the maximum utilitarian welfare of coalition structures in $G[\bigcup_{j=1}^{i}V_{B_x^j}]$ in which the role of $c$ is $\typec$. Let $l\le i$. By definition, we obtain
\[
g^*(c,\typec) = g(c,\typec,|C_{\cT}(c)|).
\]
%となる．図\ref{fig:g}に$g(c,\typec,|C_{\cT}(c)|)$のイメージを示す．
%Figure\ref{fig:g} shows the image of $g(c,\typec,|C_{\cT}(c)|)$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g.jpg}
%\caption{The image of $g(c,\typec,|C_{\cT}(c)|)$} \label{fig:g}
%\end{figure}
%以下では，$g(c,\typec,|C_{\cT}(c)|)$を$i$に関する動的計画法で計算する．
In the following, we compute $g(c,\typec,|C_{\cT}(c)|)$ by dynamic programming. 


%\paragraph{When $\typec=\iso$}\
\paragraph{Case $\typec=\iso$}\

We obtain
\begin{align*}
g(c,\iso,i)=& \begin{cases}
0 & i = 0 \\
g(c,\iso,i-1)+\max_{k}f^*(B_c^i,\iso,k)
& i\neq 0.
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\iso,0)=0$とする．$i\neq0$のとき，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$と$G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$の提携構造の差分を考える．このとき，$c$は$B_c^1,\ldots,B_c^i$に対応するいずれのクリークからも同じ提携に入る頂点をとらないので，社会効用を$\max_{k}f^*(B_c^i,\iso,k)$だけ増やす形をとる．図\ref{fig:g_iso}に$i\neq0$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\iso,0)\\=0$. When $i\neq0$, consider the difference between the coalition structures in $G[\bigcup_{j=1}^{i}V_{B_x^j}]$ and $G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$. In this case, since $c$ does not take a vertex that forms a coalition together from any of the cliques corresponding to $B_c^1,\ldots,B_c^i$, the utilitarian welfare increases by $\max_{k}f^*(B_c^i,\iso,k)$. 
%Figure\ref{fig:g_iso} shows the transition when $i\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_iso.jpg}
%\caption{The transition when $\typec=\iso$ ($i\neq0$)} \label{fig:g_iso}
%\end{figure}


%\paragraph{When $\typec=\cl$}\
\paragraph{Case $\typec=\cl$}\

We obtain
\begin{align*}
g(c,\cl,i)=& \begin{cases}
0 & i = 0\\
\max_{k}f^*(B_c^1,\cl,k)& i = 1\\
\max\left\{
\begin{array}{c}
g(c,\cl,i-1)+\max_{k}f^*(B_c^i,\iso,k),\\
g(c,\iso,i-1)+\max_{k}f^*(B_c^i,\cl,k)
\end{array}
\right\}
& i>1.
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\cl,0)=0$とする．$i\neq0$のとき，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$と$G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$の提携構造の差分を考える．このとき，$c$はクリークを形成するので$B_c^1,\ldots,B_c^i$に対応するクリークのうち1つからのみ同じ提携に入る頂点をとり，他のクリークノードにおいて$c$の役割は$\iso$となる．よって，$c$がクリークを形成する頂点が$B_c^i$内の頂点である場合とそうでない場合の社会効用を比較し，小さくない方を採用する形となる．図\ref{fig:g_cl}に$i\neq0$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\cl,0)\\=0$. When $i\neq0$, consider the difference between the coalition structures in $G[\bigcup_{j=1}^{i}V_{B_x^j}]$ and $G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$. In this case, since $c$ forms a clique, it takes a vertex from only one of the cliques corresponding to $B_c^1,\ldots,B_c^i$ into the same coalition, and the role of $c$ in the other clique nodes is $\iso$. Therefore, we compare the utilitarian welfare of the case where $c$ forms a clique with a vertex in $B_c^i$ and the case where $c$ forms a clique with a vertex not in $B_c^i$, and adopt the one that is not smaller. %Figure\ref{fig:g_cl} shows the transition when $i\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_cl.jpg}
%\caption{The transition when $\typec=\cl$ ($i\neq0$)} \label{fig:g_cl}
%\end{figure}


%\paragraph{When $\typec=\stc_l$}\
\paragraph{Case $\typec=\stc_l$}\

We obtain
\begin{align*}
g(c,\stc_l,i)=& \begin{cases}
0 & i=0\\
\sum_{j=1}^{l}{\max_{k}f^*(B_c^j,\stc,k)}-\frac{(l-1)(l+2)}{l(l+1)} & i = l\\
\max\left\{
\begin{array}{c}
g(c,\stc_l,i-1)+\max_{k}f^*(B_c^i,\iso,k),\\
g(c,\stc_{l-1},i-1)+\max_{k}f^*(B_c^i,\stc,k)-\frac{(l-1)(l+2)}{l(l+1)}
\end{array}
\right\}
& i > l.
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\stc_l,i)=0$とする．$i=l$であれば，$c$は$B_c^1,\ldots,B_c^l$に対応するクリーク内からスターの葉となる頂点をそれぞれ1つずつとって提携を形成する．この際，サイズ2のスター$l$個の社会効用とサイズ$l+1$のスターの社会効用の差が$\frac{(l-1)(l+2)}{l(l+1)}$であることに注意する．$i>l$のとき，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$と$G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$の提携構造の差分を考える．スターの中心点$c$が$l$個の葉のうちの1点を$B_c^i$内の頂点からとらない場合ととる場合の社会効用を比較し小さくない方を採用する形となる．図\ref{fig:g_stc}に$i>l$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\stc_l,i)\\=0$. If $i=l$, $c$ forms a star by taking one vertex from each of the cliques corresponding to $B_c^1,\ldots,B_c^l$ as a star leaf. Note that the difference between the utilitarian welfare of the sum of $l$ stars of size 2 and a star of size $l+1$ is $\frac{(l-1)(l+2)}{l(l+1)}$. When $i>l$, consider the difference between the coalition structures in $G[\bigcup_{j=1}^{i}V_{B_x^j}]$ and $G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$. Then we compare with the utilitarian welfare of the case where $c$ takes a vertex from $B_c^i$ as one of its leaves and the case $c$ takes no vertex from $B_c^i$, and the not smaller of the two is adopted. 
%Figure\ref{fig:g_stc} shows the transition when $i>l$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_stc.jpg}
%\caption{the transition when $\typec=\stc_l$($i>l$)} \label{fig:g_stc}
%\end{figure}



%\paragraph{When $\typec=\stcu_l$}\

%We obtain
%\begin{align*}
%g(c,\stcu_l,i)=& \begin{cases}
%0 & i = 0\\
%g(c,\stc_l,i)+\frac{2}{(l+1)(l+2)}
%& i \neq0.
%\end{cases}
%\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\stcu_l,i)=0$とする．$i\neq0$のとき，$c$が$P_{\cT}(c)$内の頂点から葉をとることからその頂点$v$をとすると，$G[\bigcup_{j=1}^{i}V_{B_x^j}\cup\{v\}]$において$c$を中心点とするスターの葉の数は$l+1$である．$g(c,\stc_l,i)$を実現する提携構造における$c$を中心点とするスターの社会効用が$2l/(l+1)$，葉の数が$l+1$のスターの社会効用が$2(l+1)/(l+2)$であることに注意するとその差分は$2/(l+1)(l+2)$となる．
%The reason why the above equation holds is as follows: When $i=0$, let $g(c,\stcu_l,i)=0$. When $i\neq0$, since $c$ takes a vertex from $P_{\cT}(c)$ as a leaf, let the vertex,be $v$. Then in $G[\bigcup_{j=1}^{i}V_{B_x^j}\cup\{v\}]$, the number of leaves of the star whose center is $c$ is $l+1$. Note that the social welfare of the star whose center is $c$ in the coalition structure realizing $g(c,\stc_l,i)$ is $2l/(l+1)$ and the social welfare of the star with $l+1$ leaves is $2(l+1)/(l+2)$, the difference of which is $2/(l+1)(l+2)$.


%\paragraph{When $\typec=\stl$}\
\paragraph{Case $\typec=\stl$}\

We obtain
\begin{align*}
g(c,\stl,i)=& \begin{cases}
0 & i = 0\\
\max_{k}f^*(B_c^1,\stl,k) & i = 1\\ 
\max\left\{
\begin{array}{c}
g(c,\stl,i-1)+\max_{k}f^*(B_c^i,\iso,k),\\
g(c,\iso,i-1)+\max_{k}f^*(B_c^i,\stl,k)
\end{array}
\right\}
& i>1.
\end{cases}
\end{align*}
%となる．
%このようになる理由は次の通りである：$i=0$のとき$g(c,\stl,0)=0$とする．$i\neq0$のとき，$c$はスターの葉なので，その中心点として$B_c^1,\ldots,B_c^i$に対応するクリークのうち1つからのみ同じ提携に入る頂点をとり，他のクリークノードにおいて$c$の役割は$\iso$となる．よって，$c$が$B_c^i$内の頂点をスターの中心点としない場合とする場合の社会効用を比較し，小さくない方を採用する形となる．図\ref{fig:g_stl}に$i\neq0$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\stl,0)\\=0$. When $i\neq0$, since $c$ is a leaf of the star, it takes as its center a vertex that enters the same coalition only from one of the cliques corresponding to $B_c^1,\ldots,B_c^i$, and the role of $c$ at the other clique nodes is $\iso$. 
Therefore, we compare the utilitarian welfare of the case where $c$ does not take a vertex from $B_c^i$ as the center of the star and the case where it does, and adopt the one that is not smaller. 
%Figure\ref{fig:g_stl} shows the transition when $i\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_stl.jpg}
%\caption{When $\typec=\stl$ ($i\neq0$)} \label{fig:g_stl}
%\end{figure}



\subsubsection{Complexity}
%本アルゴリズムでは，ブロックノードと関節ノードで漸化式が異なるので，それぞれに必要な計算時間を考える．
Since the recurrence relations are different for block nodes and cut nodes in this algorithm, we consider the computation time required for each.

%はじめに，ブロックノードにおける計算時間について考える．ブロックノードでは，$f^*(B_x,\typeB,k)$の値を計算するために，$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$と各$f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$の値を子$i$に関する動的計画法で求める．まず，$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$の計算時間を考える．一つの$B_x,\typeB,i,k$の組に対して$f(B_x,\typeB,i,k)$を求めるのに必要な計算時間は，$O(\Delta)$時間である．よって，すべての$B_x\in\mathcal{B},\typeB\in\texttt{T}_B,k$について$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$を子$i$に関する動的計画法で求める際に必要な計算時間は，
First, we consider the computation time at the block nodes. In a block node, to compute the value of $f^*(B_x,\typeB,k)$, we compute the values of \\$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$ and each $f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$ by dynamic programming. We consider the computation time of $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$. Since the time required to compute the value of $f(B_x,\typeB,i,k)$ for a single set of $B_x$, $\typeB$, $i,k$ is $O(\Delta)$, the time required to compute $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$ for all $B_x\in\mathcal{B},\typeB\in\texttt{T}_B,k$ by dynamic programming is
\begin{align*}
O((\text{Number of candidates of}\  B_x)\cdot4\cdot\Delta^3)= O(n\Delta^3).
\end{align*}
%となり，$O(n\Delta^3)$時間である．
%次に，各$f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$の計算時間について考える．一つの$B_x,\typeB,i,k,c_{\textrm{center}},v_l$の組に対して$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$の計算時間は，$f(B_x,\typeB,i,k)$の計算と同様に$O(\Delta)$時間である．また，$c_{\textrm{center}}$と$v_l$の取り方は高々$\Delta^2$通りであるので，すべての$B_x\in\mathcal{B},\typeB\in\texttt{T}_B,c_{\textrm{center}}\in |C_{\cT}(B_x)|,v_l\in B_x\setminus\{c_{\textrm{center}}\},k$について$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$を子$i$に関する動的計画法で求める際に必要な計算時間は，
Next, consider the computation time for each $f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$. The time required to compute $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$ for a single set of $B_x$, $\typeB$, $i$, $k$, $c_{\textrm{center}}$, $v_l$ is $O(\Delta)$ as in the case of $f(B_x,\typeB,i,k)$. Also, since there are at most $\Delta^2$ ways to take $c_{\textrm{center}}$ and $v_l$, the time required to compute $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)$ for all $B_x\in\mathcal{B},\typeB\in\texttt{T}_B,c_{\textrm{center}}\in |C_{\cT}(B_x)|,v_l\in B_x\setminus\{c_{\textrm{center}}\},k$ by dynamic programming is
\begin{align*}
O((\text{Number of candidates of} \ B_x)\cdot4\cdot\Delta^3\cdot\Delta^2)= O(n\Delta^5).
\end{align*}
%となり，$O(n\Delta^5)$時間である．
%さらに，$f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)\}$であり，$f^*(B_x,\typeB,k)$を求めるには，$f(B_x,\typeB,|C_{\cT}(B_x)|,k)$と各$f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$の最大値をとればよい．よって，ブロックノードにおける全体の計算時間は，$O(n\Delta^7)$となる．
%Furthermore, since $f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|C_{\cT}(B_x)|,k)\}$, we consider the maximum value of $f(B_x,\typeB,|C_{\cT}(B_x)|,k)$ and each $f_{c_{\textrm{center}}}(B_x,\typeB,|C_{\cT}(B_x)|,k)$ to compute $f^*(B_x,\typeB,k)$.
Therefore, the total computation time at the block node is $O(n\Delta^5)$.

%次に，関節ノードにおける計算で必要な計算時間について考える．関節ノードにおける計算では，$g(c,\typec,|C_{\cT}(c)|)$を子$i$に関する動的計画法で求める．一つの$c,\typec,i$の組に対して$g(c,\typec,i)$のを求めるのに必要な計算時間は，$O(\Delta)$時間である．よって，すべての$c\in\mathcal{C},\typec\in\texttt{T}_c$について$g^*(c,\typec)=g(c,\typec,|C_{\cT}(c)|)$を子$i$に関する動的計画法で求める際に必要な計算時間は，
Next, we consider the computation time at the cut nodes. In the computation at a cut node, we compute the value of $g(c,\typec,|C_{\cT}(c)|)$ by dynamic programming. The time required to compute $g(c,\typec,i)$ for a single $c,\typec,i$ set is $O(\Delta)$. Hence, the time required to compute $g^*(c,\typec)=g(c,\typec,|C_{\cT}(c)|)$ for all $c\in\mathcal{C},\typec\in\texttt{T}_c$ by dynamic programming is
\begin{align*}
O((\text{Number of candidates of\ } c)\cdot(2\Delta+3)\cdot\Delta^2)= O(n\Delta^3).
\end{align*}
%となり，$O(n\Delta^3)$時間である．

%ゆえに，本アルゴリズムの計算時間は$O(n\Delta^5)$時間となる．
Therefore, this algorithm returns the maximum utilitarian welfare partition in time $O(n\Delta^5)$.

\begin{theorem}\label{thm:block:sw:opt}
For any unweighted block graph $G$, the utilitarian welfare maximization can be computed in polynomial time.
\end{theorem}

\begin{comment}
\subsection{Egalitarian welfare}
\subsubsection{Characterization of the optimal coalition}
%Next, we show that there is also an optimal coalition structure on egalitarian welfare in which each coalition induces a clique of size 2 or larger or a star.

%はじめに，$C$に橋$e=\{u,v\}$（ただし，$e$を削除して得られる連結成分からなる提携$C_u$，$C_v$の頂点数はともに2以上）が存在するとき，$C$を$C_u$と$C_v$に社会効用を下げることなく分割できることを示す．
%We first show that when there exists a bridge $e=\{u,v\}$ (however, two coalitions $C_u$ and $C_v$ obtained by deleting $e$ contain 2 or more vertices), we can split $C$ into $C_u$ and $C_v$ without decreasing the minimum utility.



\begin{lemma}\label{lem:egal:star}
$C$をブロックグラフからなる提携とする．$C$に$v$のみを関節点として持つサイズ2の極大クリークが存在するとき，それらを$v$を中心点とするスターとして分割しても最小効用が下がることはない．
\end{lemma}

\begin{proof}
$C$において，$v$のみを関節点として持つサイズ2の極大クリークが存在すると仮定する．
$C$における最小効用はサイズ2の極大クリークの$v$でない方の頂点の効用で，その大きさは$1/|C|$である．
唯一の関節点として$v$を持つサイズ2の極大クリーク集合を$v$を中心点とするスターとして分割することを考える．
$C'$を$v$を中心点とするスター，$C^{\prime\prime}_i$を$C\setminus C'$に含まれる各連結成分とする．

はじめに，$C'$内の頂点の効用の変化を考える．
$C'\setminus\{v\}$内の頂点については，分割により隣接頂点数は変化せず，提携サイズが小さくなるので，分割により効用は増加する．
$w\in C'\setminus \{v\}$とすると$v$の効用は，$u(v,C')\ge u(w,C')>u(w,C)=1/|C|$となるので，分割により$v$の効用が$1/|C|$より小さくなることはない．

次に，$C^{\prime\prime}_i$内の頂点の効用の変化を考える．
$C^{\prime\prime}_i$内の頂点のうち$C$において$v$に隣接していないものについては，分割により隣接頂点数は変化せず，提携サイズが小さくなるので，分割により効用は増加する．
$C$において$v$を関節点として含んでいた極大クリーク内の任意の頂点$u$に着目する．
$u(u,C^{\prime\prime}_i)\ge 1/C^{\prime\prime}_i>1/|C|$なので，$C$において$v$を関節点として含んでいた極大クリーク内の任意の頂点も分割により効用が$1/|C|$より小さくなることはない．

よって，$C$に$v$のみを関節点として持つサイズ2の極大クリークが存在するとき，それらを$v$を中心点とするスターとして分割しても最小効用が下がることはない．
\end{proof}

補題\ref{lem:egal:star}を繰り返すことにより，ブロックグラフからなる任意の提携を関節点を1つのみもつ極大クリークはサイズ3以上であるような提携に最小効用を下げることなく分割できるので，以降では，関節点を1つのみもつ極大クリークはサイズ3以上であるような提携を考える．




\begin{lemma}\label{lem:egal:scu:num}
任意の$B$について，$C_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つであるような最適提携構造が存在する．
\end{lemma}

\begin{proof}
最適提携構造において，スターの中心点で$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするような$C_{\cT}(B)$に属する頂点が$t(\ge2)$個存在したとする．これらのスターを$S_i (i=1, \ldots, t)$，それぞれの中心点を$c_i (i=1, \ldots, t)$，葉の数を$l_i (i=1, \ldots, t)$とする（$c_1,\ldots,c_t$の役割が$\stcu$であるので，$l_i\ge2$）．
このとき，各スター$S_1,\ldots,S_t$内の最小効用はそれぞれの葉の効用なので，
\begin{align*}
\frac{1}{l_1+1},\frac{1}{l_2+1},\cdots,\frac{1}{l_t+1}\le\frac{1}{3}
\end{align*}
である．
今，$S_1,\ldots,S_t$が葉とする$B$内の頂点がそれぞれ$S_1,\ldots,S_t$から逸脱して1つのクリークになることを考える．
このとき，$S_1,\ldots,S_t$は葉の数が1つずつ少ないスターになり，それぞれを$S'_i (i=1, \ldots, t)$とすると，$S'_1,\ldots,S'_t$内の最小効用は，
\begin{align*}
\frac{1}{l_1},\frac{1}{l_2},\cdots,\frac{1}{l_t}
\end{align*}
となる．よって，各スターにおける逸脱前後の最小効用の差は，任意の$i(=1,\ldots,t)$に対して，
\begin{align*}
\frac{1}{l_i}-\frac{1}{l_i+1}=\frac{1}{l_i(l_i+1)}>0
\end{align*}
で表せる．

一方，$S_1,\ldots,S_t$が葉とする$B$内の頂点がそれぞれ$S_1,\ldots,S_t$から逸脱して形成したクリーク内の最小効用は少なくとも$1/2>1/(l_i+1)$である．

また，もとの最適提携構造における他の提携については最小効用は変化しない．

よって，最適提携構造においてスターの中心点で$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするような$C_{\cT}(B)$に属する頂点が$t(\ge2)$個存在するとき，その最小効用を下げることなく，$C_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つであるような最適提携構造にすることができる．

ゆえに，任意の$B$について，$C_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{C_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つであるような最適提携構造が存在する．
\end{proof}
\end{comment}

==> chapter04_ver2.tex <==
\section{Maximizing utilitarian welfare on block graphs}\label{chap:block}
In this section, we show that a maximum utilitarian welfare coalition structure on block graphs can be computed in polynomial time. 
To show this, we first characterize an optimal coalition structure on block graphs, and then, we design a dynamic programming algorithm using the characterization.


\subsection{Characterizing an optimal coalition structure}
%はじめに，ブロックスプリットグラフの社会効用最大提携構造について，次のことが知られている．
In this subsection, we characterize an optimal coalition structure on block graphs.
\begin{theorem}\label{thm:block:opt}
%各提携がクリーク，スターのいずれかになる社会効用最大提携構造が存在する．
%There exists a maximum utilitarian welfare partition on the block graph in which each coalition induces a clique of size at least 2 or a star. 
There exists a maximum utilitarian welfare coalition structure on the block graph in which each coalition induces a clique or a star. 
\end{theorem}
To show this, we show the following two lemmas below.
% First, for the maximum utilitarian welfare coalition structure on block split graphs, which are more restricted graphs than block graphs,  the following lemma holds.
% \begin{lemma}[\cite{seniorthesis_2022}]\label{lem:blocksplit:opt}
% %任意のブロックスプリットグラフ$G=(K\cup I, E)$において，各提携がクリークまたはスターのいずれかになるような社会効用最大提携構造が存在する．
% For any block split graph $G=(K\cup I, E)$, there is a maximum utilitarian welfare coalition structure in which each coalition induces a clique of size at least 2 or a star.
% \end{lemma}

% \begin{lem}\label{lem:induce:block}
% ブロックグラフ$G=(V,E)$の社会効用最大提携構造の各提携はブロックグラフまたは孤立点からなる．
% \end{lem}
% \begin{proof}
% ブロックグラフ$G=(V,E)$の頂点部分集合$C\subseteq V$が誘導する部分グラフ$G[C]$はブロックグラフ，ブロックグラフと孤立点集合，孤立点集合のいずれかとなる．$G[C]$が複数の連結成分からなるとき，それらを連結成分ごとに分割して提携を形成した方が全体の効用は高くなるので，社会効用を下げることなく1つの連結成分からなる提携に分割することができる．よって，ブロックグラフ$G=(V,E)$の社会効用最大提携構造の各提携はブロックグラフまたは孤立点からなる．
% \end{proof}
%補題\ref{lem:induce:block}を用いて社会効用最大提携構造の各提携の直径について考えると，次の補題が成り立つ．
%次に，ブロックグラフにおける社会効用最大提携構造の各提携に着目すると，頂点部分集合が誘導する部分グラフがブロックグラフまたは孤立点集合のみを含むことより，社会効用最大提携構造の各提携がブロックグラフまたは孤立点からなることがわかる．そして，各提携の直径に着目することで，各提携がクリーク，スターのいずれかからなる社会効用最大提携構造が存在することを示す．
% Next, we focus on each coalition of optimal coalition structure on block graphs. We see that each coalition consists of a block graph or an isolated vertex, since all of the subgraphs induced by the subset of vertices are only block graph or independent set. We show that there exists a optimal coalition structure on the block graph in which each coalition induces a clique or a star by focusing the diameter of each coalition.

% Next, we show that a coalition with diameter 2 can be partitioned into cliques and stars without decreasing utilitarian welfare.
\begin{lemma}\label{lem:opt:diam2}
%直径2のブロックグラフからなる提携を$C$とする．このとき，社会効用を減らすことなく提携$C$をクリークまたはスターに分割することができる．
Let $C$ be a coalition such that the diameter of $G[C]$ is 2. Then  $C$ can be partitioned into cliques or stars without decreasing utilitarian welfare.
\end{lemma}

\begin{proof}
%グラフ$G=(v,E)$をブロックグラフ，$\C^*$を$G$のある社会効用最大提携構造とする．直径2の$C^*_i \in \C^*$が存在すると仮定する．ここで，$G$がブロックグラフであることから，$G[C^*_i]$はブロックグラフであり，関節点を1点のみ含む．この
%直径2の提携$C$が誘導する部分グラフ$G[C]$は関節点$v$をちょうど1つ含む．$G[C]$に含まれる各クリークは$v$を共有する．このとき，$G[C]$に含まれる最大クリークを$C_x$，そのサイズを$x$とする．$x=2$のとき，$C_x$が最大クリークであることより，$G[C]$はスターであるので，以降では$x\ge 3$の場合について考える．提携$C'$を$C'=C_x\setminus\{v\}$，提携$C^{\prime\prime}$を$C^{\prime\prime}=C\setminus C'$とする．このとき，$(\sw(C')+\sw(C^{\prime\prime})) \ge \sw(C)$となることを示す．
We first show that a coalition $C$ that induces a block graph having diameter 2 can be partitioned into cliques or stars without decreasing utilitarian welfare.
The subgraph $G[C]$ induced by a coalition $C$ having diameter 2 contains exactly one cut vertex $v$ and each maximal clique in $G[C]$ contains $v$.
Let $C_x$ be the largest clique in $G[C]$ and its size $x$. When $x=2$, $G[C]$ is a star. Thus, we consider the case $x\ge 3$ in the following. 
Let $C'=C_x\setminus\{v\}$ and $C^{\prime\prime}=C\setminus C'$. We show that $\uw(C')+\uw(C^{\prime\prime}) \ge \uw(C)$.

%提携$C^{\prime\prime}$に含まれる頂点数を$y$，辺数を$z$とする．$\sw(C)=2((x(x-1)/2)+z)/(x+y-1)=(x(x-1)+2z)/(x+y-1)$である．一方，$\sw(C')=(x-1)-1=x-2$であり，$\sw(C^{\prime\prime})=2z/y$である．よって，$C$を$C'$と$C^{\prime\prime}$に分割することによる社会効用の変化量は，
Let $y$ be the number of vertices and $z$ be the number of edges in  $G[C^{\prime\prime}]$. Then the utilitarian welfare of $C$ is $\uw(C)=2((x(x-1)/2)+z)/(x+y-1)=(x(x-1)+2z)/(x+y-1)$. On the other hand, $\uw(C')=(x-1)-1=x-2$ and $\uw(C^{\prime\prime})=2z/y$. Thus,  \begin{align}\label{align:opt:diam2}(\uw(C')+\uw(C^{\prime\prime}))-\uw(C) = (y^2(x-2)+2(x-1)(z-y))/y(x+y-1).\end{align}
% \begin{align}\label{align:opt:diam2}
%     &(\sw(C')+\sw(C^{\prime\prime}))-\sw(C)\notag\\
%     &= \left(x-2+\frac{2z}{y}\right) -\frac{x(x-1)+2z}{x+y-1}\notag\\
%     &= \frac{y^2(x-2)+2(x-1)(z-y)}{y(x+y-1)}. 
% \end{align}
If $G[C^{\prime\prime}]$ contains a clique of size at least 3, then $z-y\ge 0$. Since $x\ge 3$, we have $(\uw(C')+\uw(C^{\prime\prime}))\ge \uw(C)$. 
Otherwise, $G[C^{\prime\prime}]$ is a star. By Property \ref{property:star}, $\uw(C^{\prime\prime}) = 2(y-1)/y$.
Thus, $(\sw(C')+\sw(C^{\prime\prime}))-\sw(C) = x-2 +  2(y-1)/y - 2((x(x-1)/2)+y-1)/(x+y-1)
=x^2-2x +xy-2y -2x +2 +2(x+y-1) - 2(x+y-1)/y -x(x-1) + 2y -2 =  -x +xy  + 2y- 2(x-1)/y -4 \ge 1$ if $x\ge 3$ and $y\ge 2$.
For both cases, we can partition $C$ into two coalitions without decreasing utilitarian welfare. By repeating the partitioning procedure, we can partition $C$ into stars and cliques.\qed
\begin{comment}
%ここで，$x\ge 3$より，$y^2(x-2)\ge 0$，$y(x+y-1)\ge 0$である．また，$2(x-1)(z-y)$の正負について考えると，提携$C^{\prime\prime}$にサイズ3以上のクリークが1つ以上あるとき$z-y\ge 0$となるので，式\eqref{align:opt:diam2}より$(\sw(C')+\sw(C^{\prime\prime}))-\sw(C)\ge 0$となる．よって，提携$C^{\prime\prime}$にサイズ3以上のクリークが1つ以上あるとき，社会効用を下げることなく提携$C$を$C'$と$C^{\prime\prime}$に分割することができる．
Since $x\ge 3$, $y^2(x-2)\ge 0$，$y(x+y-1)\ge 0$.
Also, considering the sign of $2(x-1)(z-y)$, since $z-y\ge 0$ when there is one or more cliques whose size are at least 3 in the coalition $C^{\prime\prime}$, we get $(\sw(C')+\sw(C^{\prime})-\sw(C)\sw(C)\ge 0$ from the equation~\eqref{align:opt:diam2}. 
Thus, when there is more than one clique whose size are at least 3 in the coalition $C^{\prime\prime}$, we can split the coalition $C$ into $C'$ and $C^{\prime\prime}$ without decreasing the utilitarian welfare.
%ゆえに，この操作を繰り返すことにより，社会効用を下げることなく$C^*_i$をスターとクリークに分割することができる．
%一方，提携$C^{\prime\prime}$がサイズ2のクリークのみからなるとき，$z-y=-1$となる．しかし，このとき$G[C]$はブロックスプリットグラフであり，補題\ref{lem:blocksplit:opt}より，社会効用を下げずに提携$C$をクリークとスターに分割することができる．
On the other hand, when the coalition $C^{\prime\prime}$ contains only cliques whose size are 2, then $z-y=-1$. However, in this case $G[C]$ is a block split graph, and from Lemma~\ref{lem:blocksplit:opt}, we can split $C$ into cliques and stars without decreasing the utilitarian welfare.

%よって，この操作を高々$C$の2連結成分数回だけ行うことにより，社会効用を下げることなく提携$C$をクリークまたはスターに分割することができる．ゆえに，直径2のブロックグラフからなる提携$C$は，社会効用を減らすことなくクリークまたはスターに分割することができる．
By performing this operation at most a few times on the 2-connected components of $C$, the coalition $C$ can be split into cliques or stars without decreasing the utilitarian welfare.
Hence, a coalition $C$ which induces a block graph having diameter 2 can be split into cliques or stars without decreasing the utilitarian welfare.
%ある社会効用最大提携構造$\C^*$に直径2の提携$C^*_i \in \C^*$が存在するとき，社会効用を減らすことなくクリーク部分とスター部分に分割することができる．
\end{comment}
\end{proof}


% \begin{corollary}\label{cor:blocksplit:opt}
% There exists an optimal coalition structure such that each coalition of diameter 2 forms either a clique or a star on block graphs.
% \end{corollary}

%また，直径3以上の提携$C$についても，橋$e=\{u,v\}$（ただし，$e$を削除して得られる連結成分からなる2つの提携$C_u$，$C_v$の頂点数はともに2以上）が存在するか否かに着目して補題\ref{lem:opt:diam2}と同様に考えると，次の補題が成り立つ．

Then we prove that a coalition $C$ with diameter at least 3 can be partitioned into stars and cliques as in Lemma~\ref{lem:opt:diam2}. This implies the existence of an optimal coalition structure consisting of stars and cliques.
%We focus on whether or not there exists a bridge $e=\{u,v\}$ (however, two coalitions $C_u$ and $C_v$ obtained by deleting $e$ contain at least 2 vertices).
% \begin{lemma}\label{lem:opt:diam3}
% %直径3以上のブロックグラフからなる提携を$C$とする．このとき，社会効用を減らすことなく提携$C$を孤立点，クリーク，直径2のブロックグラフに分割することができる．
% Let $C$ be a coalition with induces a block graph having diameter 3 or more. We can split $C$ into isolated vertices, cliques, and a block graph whose diameter is 2 without decreasing the utilitarian welfare.
% \end{lemma}
\begin{lemma}\label{lem:opt:diam3}
Let $C$ be a coalition such that the diameter of $G[C]$ is at least 3. Then  $C$ can be partitioned into coalitions of diameter at most 2 without decreasing utilitarian welfare.
\end{lemma}

\begin{proof}
%はじめに，$C$に橋$e=\{u,v\}$（ただし，$e$を削除して得られる連結成分からなる提携$C_u$，$C_v$の頂点数はともに2以上）が存在するとき，$C$を$C_u$と$C_v$に社会効用を下げることなく分割できることを示す．


We first consider the case that $G[C]$ has a bridge $e=\{u,v\}$ and it connects two connected components of size at least 2. Let $C_u$ and $C_v$ be the connected components of $G[C]-e$ that contains $u$ and $v$, respectively. Then we can partition $C$ into two coalitions $C_u$ and $C_v$ without decreasing the utilitarian welfare.
%提携$C_u$に含まれる頂点数を$y_u$，辺数を$z_u$，提携$C_v$に含まれる頂点数を$y_v$，辺数を$z_v$とする．$\sw(C)=2(z_u+z_v+1)/(y_u+y_v)$である．一方，$\sw(C_u)=2z_u/y_u$であり，$\sw(C_v)=2z_v/y_v$である．よって，分割することによる社会効用の変化量は，
Let $y_u$ and $z_u$ be the number of vertices and the number of edges in $C_u$ and let $y_v, z_v$ be the number of vertices and  the number of edges in $G[C_v]$. 
Then the utilitarian welfare of $C$ is $\uw(C)=2(z_u+z_v+1)/(y_u+y_v)$.
On the other hand, the utilitarian welfare of $C_u$ is $\uw(C_u)=2z_u/y_u$  and the one of $C_v$ is $\uw(C_v)=2z_v/y_v$. Then, we have $(\uw(C_u)+\uw(C_v))-\uw(C)= {2z_u}/{y_u}+{2z_v}/{y_v}-{2(z_u+z_v+1)}/{(y_u+y_v)}
    = {(2y_u(y_u z_v-y_v)+2y_v^2 z_u)}/{y_u y_v(y_u+y_v)}\ge 0$.
% \begin{align*}
%     &(\uw(C_u)+\uw(C_v))-\uw(C)\\
%     &= \frac{2z_u}{y_u}+\frac{2z_v}{y_v}-\frac{2(z_u+z_v+1)}{y_u+y_v}\\
%     &= \frac{2y_u(y_u z_v-y_v)+2y_v^2 z_u}{y_u y_v(y_u+y_v)}\ge 0.
% \end{align*}
%ここで，最後の不等号は，$y_u,y_v\ge 2, z_v\ge y_v-1$であることより，$y_u z_v-y_v\ge y_u(y_v-1)-y_v=y_u y_v-(y_u+y_v)\ge0$であることから従う．よって，$C$に橋$e=\{u,v\}$があるとき，$C$を$C_u$と$C_v$に社会効用を下げることなく分割することができる．
The last inequality follows from $y_u,y_v\ge 2$ and  $z_v\ge y_v-1$. %since $y_u z_v-y_v\ge y_u(y_v-1)-y_v=y_u y_v-(y_u+y_v)\ge0$.
%Thus, when $C$ has a bridge $e=\{u,v\}$, we can split $C$ into $C_u$ and $C_v$ without decreasing the utilitarian welfare.
Thus, $C$ can be partitioned into two coalitions without decreasing the utilitarian welfare. 

%次に，$C$に橋がない場合について考える．
Next, we consider the case that there is no bridge that connects two connected components of size at least 2 in $C$.
%$G$がブロックグラフであることから，$G[C^*_i]$はブロックグラフである．$G[C]$において関節点を1つのみ持つクリークのうち最大であるものを$C_x$，そのサイズを$x$とする．また，$C_x$に属する頂点のうち$G[C]$において関節点となっている頂点を$v$とする．提携$C'$を$C'=C_x\setminus\{v\}$，提携$C^{\prime\prime}$を$C^{\prime\prime}=C\setminus C_x\cup\{v\}$とする．このとき，$(\sw(C')+\sw(C^{\prime\prime})) \ge \sw(C)$となることを示す．
Since $G$ is a block graph, $G[C]$ is also a block graph. Let $C_x$ be the largest clique of size $x(\ge 2)$ with only one cut vertex $v$ in $G[C]$. Such $v$ always exists unless $G[C]$ is not a clique. In other words, $C_x$ is a maximum-size leaf on the block-cut tree\footnote{The definition of a block-cut tree appears in Section~\ref{subsubsec:block-cut}} of $G[C]$. 
Let $C^{\prime}=C_x\setminus\{v\}$ and $C^{\prime\prime}=C\setminus C_x\cup\{v\}$. Then we show that $\uw(C^{\prime})+\uw(C^{\prime\prime})\ge\uw(C)$.

%提携$C^{\prime\prime}$に含まれる頂点数を$y$，辺数を$z$とする．このとき，補題\ref{lem:opt:diam2}と同様の議論により，提携$C$を提携$C'$と提携$C^{\prime\prime}$に分割することによる社会効用の変化量として，式\eqref{align:opt:diam2}と同じ式が得られる．$(y^2(x-2)+2(z-y)(x-1))/y(x+y-1)$の正負を考える．$x\ge2$より，$x-2\ge0,x-1>0,(x+y-1)>0$なので，$(y^2(x-2)+2(z-y)(x-1))/y(x+y-1)$の正負は$z-y$の正負による．ここで，$C$に橋がない場合について考えているので，$C_x$に隣接するクリークにはサイズ3以上のものが必ず存在する．よって，$z-y\ge0$は常に成り立つ．ここで，$C$に橋がない場合について考えているので，提携$C^{\prime\prime}$に含まれるクリークで$G[C]$において$C_x$に隣接するもののサイズは3以上である．よって，$z-y\ge0$は常に成り立つ．
Let $y$ be the number of vertices and $z$ be the number of edges in $G[C^{\prime\prime}]$. 
Figure~\ref{fig:nobridge} shows the value of $x,y$ and $z$ with respect to the examples of $C^{\prime}$ and $C^{\prime\prime}$.
\begin{figure}[htb]
\centering
\includegraphics[width=0.5\textwidth]{nobridge.pdf}
\caption{The value of $x,y$ and $z$ with respect to the examples of $C^{\prime}$ and $C^{\prime\prime}$.} \label{fig:nobridge}
\end{figure}
By the same argument as in Lemma~\ref{lem:opt:diam2}, we obtain Equation~\eqref{align:opt:diam2}. Since $x\ge 2$ and $y\ge 2$, the sign of $(y^2(x-2)+2(z-y)(x-1))/y(x+y-1)$ depends on the sign of $z-y$.
Since the diameter of $G[C]$ is at least 3, $C_x$ forms a clique, and there is no bridge that connects two connected components of size at least 2 in $C$, $G[C^{\prime\prime}]$ contains a cycle. Thus, we have $z-y\ge 0$. Therefore, we obtain $\uw(C^{\prime})+\uw(C^{\prime\prime})\ge\uw(C)$.


%これらの操作を高々$C$の2連結成分数回だけ行うこと行うことで$C$を孤立点，クリーク，直径2の提携に分割することができる．ゆえに社会効用を下げることなく提携$C$を孤立点，クリーク，直径2の提携に分割することができる．ゆえに，これらの操作を繰り返すことにより，社会効用を下げることなく$C^*_i$を孤立点，クリーク，直径2の提携に分割することができる．

By performing these operations unless the diameter of  $G[C]$ is at most 2, we can partition $C$ into coalitions whose diameter is 2 without decreasing utilitarian welfare. 
\qed
\end{proof}

%一方，補題\ref{lem:opt:diam2}，補題\ref{lem:opt:diam3}を用いると，社会効用最大提携構造について，孤立点のみからなる提携を含まないものが存在することが示せる．
By combining Lemmas~\ref{lem:opt:diam2} and \ref{lem:opt:diam3}, we can obtain a coalition structure whose coalitions form stars or cliques from any coalition structure. This implies Theorem~\ref{thm:block:opt}.

\begin{comment}
\begin{lemma}\label{lem:opt:isol}
%ブロックグラフ$G=(V,E)$において，孤立点のみからなる提携を含まない社会効用最大提携構造が存在する．
In a block graph $G=(V,E)$, there exists a maximum utilitarian welfare partition that does not contain a coalition which induces only isolated vertex.
\end{lemma}

\begin{proof}
%ブロックグラフ$G=(V,E)$の社会効用最大提携構造を考える．補題\ref{lem:induce:block}，補題\ref{lem:opt:diam2}，補題\ref{lem:opt:diam3}より，各提携が孤立点，クリーク，スターのいずれかからなる社会効用最大提携構造が存在する．このとき，孤立点のみからなる提携が存在しない，つまり，クリークとスターのみからなる社会効用最大提携構造が存在することを示す．
From Lemmas~\ref{lem:opt:diam2} and \ref{lem:opt:diam3}, there exists a maximum utilitarian welfare partition where each coalition induces either an isolated vertex, a clique, or a star.
We show that there is no coalition which induces an isolated vertex; i.e., there is a maximum utilitarian welfare partition where each coalition induces a clique or a star.
%孤立点のみからなる提携$C^*_i \in \C^*$が存在すると仮定する．このとき，$C^*_i$に隣接する提携を$C^*_j$とすると，$C^*_j$は孤立点，クリーク，スターのいずれかである．
Assume that there exists a coalition $C^*_i \in \C^*$ induces an isolated vertex. Let $C^*_j$ be the coalition adjacent to $C^*_i$, $C^*_j$ is either an isolated vertex, a clique, or a star.

%$C^*_j$が孤立点であるとき，$\sw(C^*_i)+\sw(C^*_j)=0$であり，$C'=C^*_i\cup C^*_j$とすると，$\sw(C')=1$より，提携$C^*_i$と$C^*_j$を併合してサイズ2のクリークにすることで社会効用が大きくなるので，$\C^*$が社会効用最大提携構造であることに矛盾する．このとき，提携$C'$はサイズ2のクリークとなっている．
%この場合の例を図\ref{}に示す．
When $C^*_j$ induces a isolated vertex, $\uw(C^*_i)+\uw(C^*_j)=0$.
Denote with $C'=C^*_i\cup C^*_j$, we can increase the utilitarian welfare to merge $C^*_i$ and $C^*_j$ because $C'$ induces a clique whose size is two and $\uw(C')=1$.
This contradicts the assumption that $\C^*$ is a maximum utilitarian welfare partition.

%$C^*_j$がクリークであるとき，そのサイズを$x$とすると，$\sw(C^*_i)+\sw(C^*_j)=0+x-1=x-1$である．グラフ$G$がブロックグラフであることより，$G[C^*_i\cup C^*_j]$はブロックスプリットグラフであり，補題\ref{lem:blocksplit:opt}より，社会効用を下げることなくスターまたはクリークからなる提携に分割することができる．
When $C^*_j$ induces a clique, let $x$ be its size, then $\uw(C^*_i)+\uw(C^*_j)=0+x-1=x-1$.
Since $G$ is a block graph, $G[C^*_i\cup C^*_j]$ is a block split graph. From Lemma~\ref{lem:blocksplit:opt}, we can split $C^*_i\cup C^*_j$ into a star or a clique without decreasing the utilitarian welfare.
%この場合の例を図\ref{}に示す．

%$C^*_j$がスターであるとき，$v\in C^*_i$が隣接しているのは，$C^*_j$の葉である1頂点のみ，葉である1頂点と中心点，中心点のみいずれかである．$C^*_j$の葉の数を$l$とすると，$\sw(C^*_i)+\sw(C^*_j)=0+2l/(l+1)=2l/(l+1)$である．
When $C^*_j$ induces a star, $v\in C^*_i$ is adjacent to either only one vertex that is a leaf of $C^*_j$, one of the leaf and the center of $C^*_j$, or only the center of $C^*_j$. Let $l$ be the number of leaves in $C^*_j$, then $\uw(C^*_i)+\uw(C^*_j)=0+2l/(l+1)=2l/(l+1)$.
%$v$が$C^*_j$の葉である1頂点のみと隣接しているとき，$v\in C^*_i$が隣接する$C^*_j$内の頂点を$u\in C^*_j$，提携$C_{\alpha}$を$C_{\alpha}=\{v\}\cup\{u\}$とする．このとき，提携$C_{\beta}$を$C_{\beta}=C^*_j\setminus \{u\}$とすると，$C_{\alpha}$はサイズ2のクリークであり，$C_{\beta}$は葉の数が$l-1$のスターである．よって，$\sw(C_{\alpha})+\sw(C_{\beta})=1+2(l-1)/l$である．
When $v$ is adjacent to only one vertex that is a leaf of $C^*_j$, let $u\in C^*_j$ be the vertex which $v\in C^*_i$ is adjacent to. Let $C_{\alpha}=\{v\}\cup\{u\}$ and $C_{\beta}=C^*_j\setminus \{u\}$, then $C_{\alpha}$ is a clique whose size is 2 and $C_{\beta}$ is a star with $l-1$ leaves. Therefore, $\uw(C_{\alpha})+\uw(C_{\beta})=1+2(l-1)/l$.
%したがって，$\sw(C_{\alpha})+\sw(C_{\beta})-(\sw(C^*_i)+\sw(C^*_j))=1+2(l-1)/l-2l/(l+1)=(l+2)(l-1)/l(l+1)>0$となるので，提携$C^*_i$と$C^*_j$を提携$C_{\alpha}$と$C_{\beta}$に分割し直すことで社会効用が大きくなる．これは$\C^*$が社会効用最大提携構造であることに矛盾する．%この場合の例を図\ref{}に示す．
Thus, since $\uw(C_{\alpha})+\uw(C_{\beta})-(\uw(C^*_i)+\uw(C^*_j))=1+2(l-1)/l-2l/(l+1)=(l+2)(l-1)/l(l+1)>0$, we can increase the utilitarian welfare by splitting $C^*_i$ and $C^*_j$ into $C_{\alpha}$ and $C_{\beta}$.
This contradicts the assumption that $\C^*$ is a maximum utilitarian welfare partition.
%$v$が，$C^*_j$の葉である1頂点，及び中心点と隣接しているとき，$G[\{v\}\cup C^*_j]$はブロックスプリットグラフであり，補題\ref{lem:blocksplit:opt}より，$C^*_i$を$C_{\alpha}=\{v\}\cup\{u\}$と$C_{\beta}=C^*_j\setminus \{u\}$に社会効用を下げることなく分割し直すことができる．$v$が，$C^*_j$の葉である1頂点のみと隣接しているときと同様の式から，$C^*_i$を$C_{\alpha}=\{v\}\cup\{u\}$と$C_{\beta}=C^*_j\setminus \{u\}$に社会効用を下げることなく分割し直すことができる．
When $v$ is adjacent to one of the leaf and the center of $C^*_j$, $G[\{v\}\cup C^*_j]$ is a block split graph. Thus from Lemma~\ref{lem:blocksplit:opt}, we can split $C^*_i$ into $C_{\alpha}=\{v\}\cup\{u\}$ and $C_{\beta}=C^*_j\setminus \{u\}$ without decreasing the utilitarian welfare.
%$v$が，$C^*_j$の中心点のみと隣接しているとき，提携$C'$を$C'=C^*_i\cup C^*_j$とすると$C'$もスターであり，社会効用は$\sw(C')=2(l+1)/(l+2)$である．$\sw(C')-(\sw(C^*_i)+\sw(C^*_j))=2(l+1)/(l+2)-2l/(l+1)=2/(l+1)(l+2)$なので，提携$C^*_i$と$C^*_j$を併合して，葉の数が$l+1$のスターにすることで，社会効用を大きくすることができる．これは$\C^*$が社会効用最大提携構造であることに矛盾する．
%この場合の例を図\ref{}に示す．
When $v$ is adjacent to only the center of $C^*_j$, let $C'=C^*_i\cup C^*_j$ then $C'$ is also a star and $\uw(C')=2(l+1)/(l+2)$. Since $\uw(C')-(\uw(C^*_i)+\uw(C^*_j))=2(l+1)/(l+2)-2l/(l+1)=2/(l+1)(l+2)$, we can increase the utilitarian welfare by merging $C^*_i$ and $C^*_j$ into a star with $l+1$ leaves.
%よって，孤立点のみからなる提携$C^*_i \in \C^*$が存在すると仮定すると，$C^*_j$がスターであるときについても，$\C^*$が社会効用最大提携構造であることに矛盾する．
Therefore, assuming that there exists a coalition $C^*_i\in\C^*$ which induces a isolated vertex, it contradicts that $\C^*$ is a maximum utilitarian welfare partition, even when $C^*_j$ induces a star.

%以上より，孤立点のみからなる提携を含まない社会効用最大提携構造が存在する．
In this way, we show that there exists a maximum utilitarian welfare partition that does not include coalitions which induces a isolated vertex.\qed
\end{proof}

%補題\ref{lem:induce:block}，
%補題\ref{lem:opt:diam2}，補題\ref{lem:opt:diam3}，補題\ref{lem:opt:isol}より，次の定理が成り立つ．
%From Lemmas~\ref{lem:opt:diam2}, \ref{lem:opt:diam3} and \ref{lem:opt:isol}, the following theorem holds.
\end{comment}

\subsection{Algorithm}
In this subsection, we give a polynomial-time algorithm based on dynamic programming using optimal coalition structures shown in Theorem~\ref{thm:block:opt}. 

\begin{theorem}\label{thm:block:sw:opt}
\textsc{Utilitarian Welfare Maximization} on unweighted block graphs can be computed in time $O(n\Delta^5)$.
\end{theorem}

To design a DP-based algorithm, we first define the block-cut tree of a graph.

%\begin{theorem}\label{thm:block:sw:opt}
%\textsc{Utilitarian Welfare Maximization} on unweighted block graphs can be computed in time $O(n\Delta^5)$.
%\end{theorem}

\subsubsection{Block-cut tree}\label{subsubsec:block-cut}
%グラフ$G=(V,E)$をブロックグラフとする．$G$に含まれる極大クリークの集合を$\mathcal{B}=\{B_1,\ldots,B_\beta\}$とする．なお各クリーク$B$を点集合とみなすことにする．$G$における関節点の集合を$\cC=\{c_1,\ldots,c_{\gamma}\}$とする．これらに対し，$\mathcal{X}=\mathcal{B}\cup\mathcal{C}$をノード集合とした，ブロックグラフ$G$がなす木構造$\mathcal{T}(G)$を$\mathcal{T}=(\mathcal{X},\mathcal{E})$で定める．ただし，$\mathcal{E}=\left\{\{B,c\}\mid  B\in\mathcal{B},c\in\mathcal{C}: c \in B \right\}$である．対象とするグラフ$G$が明らかな場合，$\mathcal{T}(G)$を単に$\mathcal{T}$と書くことにする．ここで，$\mathcal{T}$において各$B\in \mathcal{B}$をブロックノード，各$c\in\mathcal{C}$を関節ノードと呼ぶ．便宜上，$\cT$を適当なブロックノード$B_r$を根とした根付き木とみなすことにする．すなわち，$\mathcal{T}$によって，$\mathcal{X}$の頂点の親子関係や子孫・祖先関係が定められる．$\cT$上で頂点$x\in \cX$とその子孫からなる部分木を$\mathcal{T}_{x}(G)$で表す．また$\textrm{Child}_{\cT}(x)$を$\cT$における$x\in \cX$の子ノードの集合とする．また$\cT_x$に対応する$G$の頂点集合を$V_x$で表すことにする．このとき$\cT_x$に対応する$G$の部分グラフを$G[V_x]$で表すことができる．
For a block graph $G=(V,E)$, let $\mathcal{B}=\{B_1,\ldots,B_\beta\}$ be the set of maximal cliques, called \emph{blocks}, in $G$ and $\cC=\{c_1,\ldots,c_{\gamma}\}$ be the set of cut vertices in $G$. Then the \emph{block-cut tree} $\mathcal{T}(G) = (\mathcal{X}, \mathcal{E})$ of $G$ is a tree such that $\mathcal{X}=\mathcal{B}\cup\mathcal{C}$ and each edge in $\mathcal{E}$ connects a block $B\in \mathcal{B}$ and a cut vertex $c\in \mathcal{C}\cap B$.
For simplicity, we sometimes write $\mathcal{T}$ instead of $\mathcal{T}(G)$. 
We call $B\in \mathcal{B}$ a block node and $c\in \mathcal{C}$ a cut node of $\mathcal{T}$. 
For convenience, we consider a block-cut tree rooted by a block node $B_r$. We denote by $\mathcal{T}_{x}(G)$ a subtree consisting of a node $x\in \cX$ and its descendants on $\cT$, by $p_{\cT}(x)$ the parent node of $x\in \cX\setminus \{B_r\}$, and by $\textrm{Child}_{\cT}(x)$ the set of children nodes of $x\in \cX$ in $\cT$ (see Figures~\ref{fig:tree:decomposition1} and \ref{fig:tree:decomposition2}). We also denote by $V_x$ the set of vertices in $G$ corresponding to $\cT_x$ and by $G[V_x]$ the induced subgraph of $G$ corresponding to $\cT_x$. For each block node $B\in \mathcal{B}\setminus \{B_r\}$ and its parent node $p_{\cT}(B)\in \mathcal{C}$, $c_p$ denotes the cut vertex in $B\cap p_{\cT}(B)$.
%また，$P_{\cT}(x)$を$\cT$における$x\in \cX$の親ノードとする．極大クリーク（ブロック）$B$を関節点とそれ以外の点$S(B):=B\setminus \cC$に分けると，ブロックグラフでは$S(B)$内の点は$B$内の点としか隣接しない．ブロックグラフに対する木構造の例を図\ref{fig:tree:decomposition}に示す．
For $B\in \mathcal{B}$, we define $R(B):=B\setminus\cC$ as the set of non-cut vertices in $B$.
For a rooted block-cut tree, its leaves are block nodes.
% Dividing the maximal clique $B$ into cut vertices and other vertices $R(B):=B\setminus\cC$, vertices in $R(B)$ are only adjacent to vertices in $B$ in the block graph. An example of a tree structure for a block graph is shown in Figures ~\ref{fig:tree:decomposition1} and \ref{fig:tree:decomposition2}.
\begin{figure}[htb]
\begin{tabular}{cc}
\begin{minipage}{0.45\hsize}
\centering
\includegraphics[width=\textwidth]{treedecomposition1.pdf}
\caption{Example of a block graph.} \label{fig:tree:decomposition1}
\end{minipage}
\begin{minipage}{0.45\hsize}
\centering
\includegraphics[width=\textwidth]{treedecomposition2.pdf}
\caption{The corresponding tree structure of block graph in Figure \ref{fig:tree:decomposition1}.}\label{fig:tree:decomposition2}
\end{minipage}
\end{tabular}
\end{figure}


\subsubsection{Defining recurrence relations}
%Now, we construct the algorithm to compute a social optimum in which each coalition induces a clique or a star. First, we prove that for such optimal coalition structure, the following lemma holds. 
%この結果を利用して，以下では各提携がサイズ2以上のクリークまたはスターのいずれかになるような社会効用最大提携構造を求めることを考える．$\mathcal{T}(G)$におけるクリークノードと関節ノードに対する漸化式を定義し，葉から順に適用していくことで，もとのブロックグラフ$G$の社会効用最大提携構造の総効用を求める動的計画法を設計する．
By Theorem~\ref{thm:block:opt}, we design a dynamic programming algorithm on block-cut trees to find an optimal coalition structure such that each coalition is either a clique of size at least 2 or a star. 
%We design dynamic programming by defining recurrence relation for the clique nodes and cut nodes in $\mathcal{T}(G)$ and applying them in order starting from the leaf nodes.

%$\texttt{T}_B=\{\iso,\cl,\stc,\stl\}$とする．これは，各カット点$x\in B_x$が動的計画法の途中で提携内でどのような構造をとっているのかを表す．具体的には，$\iso$は$x$が属する提携が孤立点であること，$\cl$は$x$が属する提携がサイズ2以上のクリークであること，$\stc$は$x$が属する提携がスターであり，かつ$x$がその中心であること，$\stl$は$x$が属する提携がスターであり，かつ$x$がその葉であることを表す．図\ref{fig:T_B}に$\texttt{T}_B$のイメージを示す．
For a block node $B\in \mathcal{B}$, we define $\texttt{T}_B=\{\iso,\cl,\stc,\stl\}$ as the set of states of the cut vertex $c_p\in B\cap p_{\cT}(B)$ that represents the role of $c_p$ within the coalition containing $c_p$ in the intermediate steps of the algorithm for a block node. For a coalition structure $\PP_{B}$ of $G[V_B]$, $\iso$ means that $c_p$ is a singleton in $\PP_B$, $\cl$  means that $c_p$ belongs to a coalition that forms a clique of size at least 2 in $\PP_B$, $\stc$ means that  $c_p$ belongs to a coalition that forms a star (not a singleton) and $c_p$ is its center in $\PP_B$, and $\stl$ means that $c_p$ belongs to a coalition that forms a star (not a singleton) and $c_p$ is its leaf in $\PP_B$. Figure~\ref{fig:T_B} shows the role of $c_p\in B\cap p_{\cT}(B)$ with respect to $\texttt{T}_B$.
\begin{figure}[htb]
\centering
\includegraphics[width=\textwidth]{typeB.pdf}
\caption{The role of $c_p\in B\cap p_{\cT}(B)$ in $B$ with respect to $\texttt{T}_B$.} \label{fig:T_B}
\end{figure}


%また，$\texttt{T}_c=\{\iso, \cl, \stc_l,\stcu_l,\stl\}$（ただし，$c\in\cC$，$1\le l\le|\textrm{Child}_{\cT}(c)|$）とする．これは，各カット点$c\in B_x\setminus\{x\}$が動的計画法の途中で提携内でどのような構造をとっているのかを表す．具体的には，$\iso,\cl,\stl$は$\texttt{T}_B$における定義と同様であり，$\stc_l,\stcu_l$は共に$c$が属する提携が$c$を中心とするスターであり，$V_c$の中から葉として$l$個の頂点を取るものであることを表す．ただし，$\stc$は$c$が$P_{\cT}(c)$内の頂点から葉を取らないこと，$\stcu$は$c$が$P_{\cT}(c)$内の頂点から葉を取ることを表す．つまり，$\stc_l$であれば$c$が属する提携は$c$を中心とする葉数$l$のスターであり，$\stcu_l$であれば$c$が属する提携は$c$を中心とする葉数$l+1$のスターである．図\ref{fig:T_B}に$\texttt{T}_c$のイメージを示す．
We also define $\texttt{T}_c=\{\iso,\cl,\stc_1,\ldots, \stc_{|\textrm{Child}_{\cT}(c)|},\stcu_1,\ldots, \stcu_{|\textrm{Child}_{\cT}(c)|}, \stl\}$ for a cut node $c\in \mathcal{C}$ as  the set of states of cut vertex $c$  that represents the role of  $c$ in the intermediate step of the algorithm.
Intuitively, in a cut node, the results of its children's block nodes  are integrated.
The states $\iso$, $\cl$, $\stl$ are the same meaning as the ones in $\texttt{T}_B$. The states $\stc_\ell$ and $\stcu_\ell$ denote that the cut vertex $c$ is the center vertex in the coalition that forms a star with $\ell$ leaves in $G[V_c]$. The difference  between them is that $\stc_\ell$ denotes that the coalition  to which $c\in \mathcal{C}$ belongs only contains vertices in $V_c$ whereas $\stcu_\ell$ denotes that the coalition  to which $c\in \mathcal{C}$ belongs \emph{will} contain one vertex in the parent node $p_{\mathcal{T}}(c)\in \mathcal{B}$ as a leaf. Note that since the coalition forms a star and $p_{\mathcal{T}}(c)$ forms a clique, it can contain at most one vertex in $p_{\mathcal{T}}(c)$. Furthermore, if $c$ takes the state $\stcu_\ell$, then the final coalition containing $c$ forms a star with $\ell+1$ leaves whose center is $c$.
Figure~\ref{fig:T_c} shows the role of $c\in \mathcal{C}$ with respect to types in $\texttt{T}_c$.
\begin{figure}[htb]
\centering
\includegraphics[width=\textwidth]{typec.pdf}
\caption{The role of $c\in \mathcal{C}$ in its cut node with respect to $\texttt{T}_c$.} \label{fig:T_c}
\end{figure}

%$f^*(B_x,\typeB,k)$は，$G[V_{B_x}]$における以下の条件を満たす提携構造の中での最大社会効用を表す: 
Now, we define the recurrence relations for block nodes and cut nodes. 
For block nodes, we define $f^*(B,\typeB,k)$ as the maximum utilitarian welfare among coalition structures in $G[V_{B}]$ that satisfies the following condition: 
\begin{itemize}
    %\item ブロックノード$B$のカット点$x$が属する提携内での役割が$\typeB\in \{\iso, \cl, \stc,\stl\}$. 
    \item $c_p$ is the parent cut node of $B$ and the role of the $c_p$ within the coalition to which $c_p$ belongs is $\typeB\in \{\iso, \cl, \stc,\stl\}$.
    %\item $B$が子を持つならば，$\textrm{Child}_{\cT}(B_x)$に属する関節点のうちちょうど$k$個が各部分木内の頂点とは提携を形成しない，かつその他の$\textrm{Child}_{\cT}(B_x)$に属する関節点はいずれも\underline{各部分木内の頂点を含み}提携を形成する．
    %\item  If $B$ has children, then exactly $k$ cut nodes belonging to $\textrm{Child}_{\cT}(B_x)$ do not form coalitions with vertices in each subtree, and all other cut nodes belonging to $\textrm{Child}_{\cT}(B_x)$ form coalitions with vertices in each subtree.
     %\item $\textrm{Child}_{\cT}(B_x)\neq\emptyset$ならば，
    %\begin{itemize}
    %    \item $V_c\setminus \{c\}$の頂点と提携を形成しない頂点が$\textrm{Child}_{\cT}(B_x)$にちょうど$k$個存在，
    %    \item それ以外の$\textrm{Child}_{\cT}(B_x)$内の頂点が属する提携はそれぞれ$V_c\setminus \{c\}$の頂点を\underline{少なくとも一つ含む}．
    %\end{itemize}
    \item if $\textrm{Child}_{\cT}(B)\neq\emptyset$, there are exactly $k$ cut vertices $c_1,\ldots c_k\in \textrm{Child}_{\cT}(B)$ such that the coalition that $c_i$ belongs to contain no vertex in $V_{c_i}\setminus \{c_{i}\}$ for $1\le i\le k$.
    % \begin{itemize}
    % \item There are exactly $k$ cut vertices $c_1,\ldots c_k\in \textrm{Child}_{\cT}(B)$ whose coalitions contain no vertex in $V_{c_i}\setminus \{c_{i}\}$ for $1\le i\le k$.
    % %that do not form a coalition with vertices in $V_c\setminus \{c\}$.
    % \item Coalitions to which other $|\textrm{Child}_{\cT}(B)|-k$ vertices $c_{k+1},\ldots c_{|\textrm{Child}_{\cT}(B)|}\in \textrm{Child}_{\cT}(B)$ belong contain at least one vertex in $V_{c_i}\setminus \{c_i\}$ for $k+1\le i\le |\textrm{Child}_{\cT}(B)|$.
    % \end{itemize}
\end{itemize}


%$g^*(c,\typec)$は，$\typec\in\{\iso,\cl,\stc_l,\stl\}$のとき$G[V_c]$における，$\typec=\stcu_l$のとき$G[V_c\cup\{v\}]$（ただし$v$は$P_{\cT}(c)$内の頂点で$c$を中心点とするスターの葉となる頂点とする）における以下の条件を満たす提携構造の中での最大社会効用を表す：
%$g^*(c,\typec)$ denotes the maximum social welfare in the coalition structures in $G[V_c]$ when $\typec\in\{\iso,\cl,\stc_l,\stl\}$, and in $G[V_c\cup\{v\}]$ when $\typec=\stcu_l$ (note that $v$ is the vertex in $P_{\cT}(c)$ that is the leaf of a star centered at $c$) that satisfies the following condition: 
%\begin{itemize}
    %\item 関節ノード$c$が属する提携内での役割が$\typec\in \{\iso, \cl, \stc_1,\ldots,\stc_{|\textrm{Child}_{\cT}(c)|},\stcu_1,\ldots,\stcu_{|\textrm{Child}_{\cT}(c)|},\stl\}$.
 %   \item The role within the coalition to which the cut node $c$ belongs is $\typec\in \{\iso, \cl, \stc_1,\ldots,\stc_{|\textrm{Child}_{\cT}(c)|},\stcu_1,\ldots,\stcu_{|\textrm{Child}_{\cT}(c)|},\stl\}$.
%\end{itemize}

%カット点$c\in C$と$\typec\in\{\iso,\cl,\stc_1,\ldots,\stc_{|\textrm{Child}_{\cT}(c)|},\stl\}$に対して，$g^*(c,\typec)$を$c$の役割が$\typec$であるような$G[V_c]$の提携構造の最大社会効用とする．
For a cut node $c\in C$ and $\typec\in\{\iso,\cl,\stc_1,\ldots,\stc_{|\textrm{Child}_{\cT}(c)|},\stl\}$, let $g^*(c,\typec)$ be the maximum utilitarian welfare in the coalition structures in $G[V_c]$ in which the role of $c$ is $\typec$.

%また，$g^*(c,\stcu_l)$は，カット点$c\in C$が$P_{\cT}(c)$内の頂点から葉$v_l$を取りスターとなるときの$G[V_{c_{\textrm{center}}}\cup\{v_l\}]$部分の社会効用を表し，
Also, $g^*(c,\stcu_\ell)$ denotes the maximum utilitarian welfare in the $G[V_{c}\cup\{v_{\ell+1}\}]$ when the cut node $c\in C$ becomes the center of a star with $\ell+1$ leaves $v_1,\ldots, v_{\ell}\in V_c$ and $v_{\ell+1}\in p_{\cT}(c)$.
Then we can compute $g^*(c,\stcu_\ell)$ from $g^*(c,\stc_\ell)$ as follows:
\begin{align*}
g^*(c,\stcu_\ell)=g^*(c,\stc_\ell)-\frac{2\ell}{\ell+1}+\frac{2(\ell+1)}{\ell+2}=g^*(c,\stc_\ell)+\frac{2}{(\ell+1)(\ell+2)}.
\end{align*}
Note that $\frac{2\ell}{\ell+1}$ and $\frac{2(\ell+1)}{\ell+2}$ are the utilitarian welfare of a star with $\ell$ leaves and a star with $\ell+1$ leaves, respectively. Thus, $\frac{2(\ell+1)}{\ell+2}-\frac{2\ell}{\ell+1}$ denotes the increase of the utilitarian welfare when a leaf is added to a coalition that forms a star with $\ell$ leaves.

%$g^*(c,\fin)=\max_{\typec\in\{\cl,\stc_1,\ldots,\stc_|\textrm{Child}_{\cT}(c)|,\stl\}}g^*(c,\typec)$とする．条件を満たす提携構造が存在しない場合は，$f^*(B,\typeB,k)=-\infty$，$g^*(c,\typec)=-\infty$とする．以下では，$f^*(B,\typeB,k)$，$g^*(c,\typec)$を$\mathcal{T}$上における動的計画法で計算する．
Let $g^*(c,\fin)=\max_{\typec\in\{\cl,\stc_1,\ldots,\stc_|\textrm{Child}_{\cT}(c)|,\stl\}}g^*(c,\typec)$ be the maximum utilitarian welfare in $G[V_c]$. If there is no coalition structure that satisfies the conditions, we set $f^*(B,\typeB,k)=-\infty$ and $g^*(c,\typec)=-\infty$ as invalid cases. 
In the following, we define the recurrence relations of the dynamic programming algorithm to compute $f^*(B,\typeB,k)$ and $g^*(c,\typec)$ recursively.




\subsubsection{Recurrence relations in the block nodes}
First, we prove that for such an optimal coalition structure, the following lemma holds. 
%$\mathcal{T}$において，カットノード$c\in \mathcal{C}$の親ノードを$B\in \mathcal{B}$とする．このとき以下の補題が成立する．
In $\mathcal{T}$, let $B\in \mathcal{B}$ be the parent node of the cut node $c\in \mathcal{C}$. Then, the following lemma holds.

\begin{lemma}\label{scu:num}
% 最適提携構造において，任意の$B$について，$\textrm{Child}_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つである．
Let $B\in \mathcal{B}$ be a block node in a rooted block-cut tree.
Then there exists an optimal coalition structure such that at most one cut vertex $c$ in $\textrm{Child}_{\cT}(B)$ that is the center of a star having both vertices in $V_B\setminus B$ and in $B$ as leaves. 
\end{lemma}

\begin{proof}
%背理法で示す．スターの中心点で$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするような$\textrm{Child}_{\cT}(B)$に属する頂点が$t(\ge2)$個存在したとする．これらのスターを$P_1,\ldots,P_t$，それぞれの中心点を$c_1,\ldots,c_t$，葉の数を$l_1+1,\ldots,l_t+1$とする．今，$P_1,\ldots,P_t$が葉とする$B$内の頂点がそれぞれ$P_1,\ldots,P_t$から逸脱して1つのクリークになることを考える．このとき，$P_1,\ldots,P_t$は葉の数が1つずつ少ないスターになり，それぞれを$P'_1,\ldots,P'_t$とすると，$l_1,\ldots,l_t\ge1$より，逸脱前後の社会効用の差は，
%By way of contradiction, let us assume 
For the sake of contradiction, suppose that there are $t(\ge 2)$ vertices $c_1,\ldots, c_t\in \textrm{Child}_{\cT}(B)$ that are the centers of $t$ stars having both vertices in $V_{\textrm{Child}_{\cT}(B)}$ and in $B$ as leaves in an optimal coalition structure $\PP^*$. Let $S_1,\ldots,S_t$ be $t$ stars whose centers are $c_1,\ldots, c_t$ 
and let $\ell_1+1,\ldots,\ell_t+1$ be the number of leaves of $S_1,\ldots,S_t$. 
Since $S_i$ is a star and $B$ forms a clique, each $S_i$ contains exactly one vertex in $B$ as a leaf.
We denote by $u_i$ the unique leaf in $B$ of $S_i$.

Now we reconstruct a coalition structure $\PP$ from $\PP^*$. 
Let $S'_i=S_i\setminus \{u_i\}$ for $1\le i\le t$ and $C_B = \{u_1,\ldots, u_t\}$.
Then $S'_i$ is a star with $\ell_i$ leaves and $C_B$ is a clique of size $t$.
Let $\PP = \PP^*\setminus \{S_1,\ldots,S_t\} \cup  \{S'_1,\ldots,S'_t,C_B\}$.

Considering $\ell_1,\ldots,\ell_t\ge 1$, the difference between $\PP$ and $\PP^*$ is as follows:
\begin{align*}
\uw(\PP^*) -\uw(\PP)
 &=\uw(S_1)+\cdots+\uw(S_t)-(\uw(S'_1)+\cdots+\uw(S'_t)+t-1)\\
 %&=\uw(S'_1)+\cdots+\uw(S'_t)+\frac{2}{(\ell_1+1)(\ell_1+2)}+\cdots+\frac{2}{(\ell_t+1)(\ell_t+2)}\\
 &=\frac{2}{(\ell_1+1)(\ell_1+2)}+\cdots+\frac{2}{(\ell_t+1)(\ell_t+2)}-t+1\\
&\le  -\frac{2}{3}t+1<0.
\end{align*}
%となる．よって，最適性に矛盾する．
%We get a contradiction.
This contradicts the optimality of $\PP^*$. 
\qed
\end{proof}

%補題\ref{scu:num}より，$f^*(B_x,\typeB,k)$を実現する提携構造において$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点は高々1つである．よって，提携構造に$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点が存在しないときと1つ存在するときに場合分けをしてそれぞれの社会効用の最大値を考え，さらにそれらの最大値を求めることで，$f^*(B_x,\typeB,k)$の値を計算する．
From Lemma~\ref{scu:num}, there is at most one cut vertex in $\textrm{Child}_{\cT}(B)$ whose role is $\stcu_{\ell}$ in the coalition structure that realizes $f^*(B,\typeB,k)$. Therefore, we consider two cases (1) no cut vertex in $\textrm{Child}_{\cT}(B)$ takes the role $\stcu_{\ell}$ and (2) exactly one cut vertex in $\textrm{Child}_{\cT}(B)$ takes the role $\stcu_{\ell}$. 
%one to compute the value of $f^*(B,\typeB,k)$. Then, we consider the maximum value of each social welfare, and find their maximum values.

\medskip
\noindent \textbf{[Case (1): No cut vertex in $\textrm{Child}_{\cT}(B)$ takes the role $\stcu_{\ell}$.]}

%はじめに，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点が存在しない場合について考える．まず，補助関数$f(B_x,\typeB,i,k)$を定義する．$x_1, x_2, \ldots, x_i \in \textrm{Child}_{\cT}(B_x)$に対して，$f(B_x,\typeB,i,k)$は，$G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$の提携構造のうち以下の条件を満たすものの最大社会効用を表す：(i) $x$のタイプが$\typeB$, (ii) $B_x$に属する関節点$x_1, x_2, \ldots, x_i$のうち，ちょうど$k$個が各部分木内の頂点とは提携を形成しない，かつその他のちょうど$i-k$個の関節点は\underline{各部分木内の点のみと}提携を形成している，
%つまり$\stcu_l$である$\textrm{Child}_{\cT}(B_x)$内の頂点が存在しない．なお$0\le k\le i \le |\textrm{Child}_{\cT}(B_x)|$である．すると，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点が存在しない場合の社会効用の最大値は，$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$で表すことができる．図\ref{fig:f}に$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$のイメージを示す．
First, we consider Case (1). 
%Define an auxiliary function $f(B,\typeB,i,k)$ as follows. 
For a block node $B$ and $c_1, c_2, \ldots, c_i \in \textrm{Child}_{\cT}(B)$ where $1\le i\le |\textrm{Child}_{\cT}(B)|$, we define  $f(B,\typeB,i,k)$ as the maximum utilitarian welfare  in $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i} V_{c_j}]$ that satisfies the following conditions: 
\begin{itemize}
 \item $c_p$ is the parent cut node of $B$ and the role of the $c_p$ within the coalition to which $c_p$ belongs is $\typeB\in \{\iso, \cl, \stc,\stl\}$.
 %The role of $x$ is $\typeB$. 
 %\item $x_1, x_2, \ldots, x_i\in \textrm{Child}_{\cT}(B_x)$のうち，$V_{x_i}\setminus\{x_i\}$の頂点と提携を形成しない頂点がちょうど$k$個，それ以外の$i-k$個はそれぞれ$V_{x_i}\setminus \{x_i\}$の頂点\underline{のみと}提携を形成している．
 \item There are exactly $k$ cut vertices among $c_1, c_2, \ldots, c_i$ such that each of $k$ such cut vertices does not form the coalition with vertices in its subtree, and each of exactly $i-k$ other cut vertices among $c_1, c_2, \ldots, c_i$ forms a coalition  with only vertices  in its subtree. 
\end{itemize}
%なお$0\le k\le i \le |\textrm{Child}_{\cT}(B_x)|$である．すると，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点が存在しない場合の社会効用の最大値は，$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$で表すことができる．
Note that $0\le k\le i \le |\textrm{Child}_{\cT}(B)|$. Then, the maximum utilitarian welfare in $G[V_B]$ in Case (1) can be expressed by $f(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$. 
We can compute $f(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$ as follows.
%Figure\ref{fig:f} shows an image of $f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f.jpg}
%\caption{The image of $f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$} \label{fig:f}
%\end{figure}

%まずベースケースとして，$i=0$のときを考える．このとき対象となるグラフは$G[\{x\}\cup S(B_x)]$であり，これがクリークをなしていることに注意すると
As the base case, we consider the maximum utilitarian welfare in  $G[\{c_p\}\cup R(B)]$. For convenience, we set this case as $i=0$. Considering $G[\{c_p\}\cup R(B)]$ is a clique, we can obtain 
\begin{align*}
 f(B,\typeB,0,0) &= \begin{cases}
0 & \text{if $R(B)=\emptyset$}\\ 
|R(B)|-1 & \text{if $R(B)\neq\emptyset$ \& $\typeB= \iso$}\\ 
|R(B)| & \text{if $R(B)\neq\emptyset$ \& $\typeB= \cl$}\\
\max\{1,|R(B)|-1\} & \text{otherwise}. %\typeB\in\{\stc,\stl\}
\end{cases}
\end{align*}
%が得られる．それぞれ確認する：$S(B_x)=\emptyset$のときは，$G[\{x\}\cup S(B_x)]$は1点のみからなるため，$f=0$となる．$S(B_x)\neq \emptyset$のときは，$\typeB=\iso$のときは$S(B_x)$だけでクリークを構成するのでその効用は$|S(B_x)|-1$となる，$\typeB=\cl$のときは$x$と$S(B_x)$がクリークの形で提携をとり効用は$|S(B_x)|$となる．$\typeB=\stc,\stl$の場合は，$S(B_x)$のうち1点と$x$がスターを形成するかたちをとるため，$|S(B_x)|=1$のときは$1$, $|S(B_x)|>1$のときは$|S(B_x)|-1$の値をとる．
The reason for the above equation is as follows.
In the first case, $G[\{c_p\}\cup R(B)]$ consists of only one vertex, and hence $f=0$. 
If $R(B)\neq \emptyset$,  $R(B)$ is contained in some coalition in any optimal coalition structure in $G[\{c_p\}\cup R(B)]$.
In the second case, $c_p$ is a singleton. Thus, the maximum utilitarian welfare, in this case, is  $|R(B)|-1$. Note that $R(B)$ forms a clique. In the third case, the optimal coalition structure with the maximum utilitarian welfare is clearly $\{c_p\}\cup R(B)$ and it forms a clique. Thus, the maximum utilitarian welfare is $|R(B)|$. 
In the remaining case, $c_p$ takes the state $\stc$ or $\stl$, which means that $c_p$'s coalition forms a star. In this case, if $|R(B)|=1$,  an optimal coalition structure forms a clique of size 2. Thus, the utilitarian welfare is $1$. 
On the other hand, if $|R(B)|>1$, an optimal coalition structure forms a singleton of $c_p$ and a clique of size $|R(B)|$. Thus, the utilitarian welfare is  $|R(B)|-1$.
%池山作成
%In the remaining case, $c_p$ takes the state $\stc$ or $\stl$, which means that $c_p$'s coalition forms a star. In this case, if $|R(B)|=1$,  an optimal coalition structure forms a star of size 2. Thus, the utilitarian welfare is $1$. On the other hand, if $|R(B)|>1$, an optimal coalition structure forms a star of $c_p$ and avertex in $R(B)$ and a clique of size $|R(B)|-1$. Thus, the utilitarian welfare is  $|R(B)|-1$.


%次に$i>0$の場合を考える．
Next, we consider the case when $i\ge 0$. 
%\paragraph{When $\typeB=\iso$}\
\paragraph{Case $\typeB=\iso$:}\ 

We define the recurrence relation for $\typeB=\iso$ as follows.
\begin{align*}
&f(B,\iso,i,k)\\
&=
\begin{cases}
f(B,\iso,i-1,0)+g^*(c_i,\fin)%c_iはisoでない
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B,\iso,i-1,0)+g^*(c_i,\iso),\\%c_iはiso
f(B,\iso,i-1,1)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{if $k=1$ \& $R(B)= \emptyset$}\\
\max\left\{
\begin{array}{c}
f(B,\iso,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
f(B,\iso,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise}
\end{cases}
\end{align*}
%となる．
%このようになる理由は次の通りである：$G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup S(B_x)\cup \bigcup_{j=1}^{i-1} V_{x_j}]$の提携構造の差分を考える．まず$k=0$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．$k>0$に対しては，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．この際，$x_i$が$B_x$内の頂点と同じ提携に入り$k>1$または$S(B)\neq\emptyset$であるならば，$x_i$は他の関節点あるいは$S(B)$の点とクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．$k=1$かつ$S(B)=\emptyset$ならば，関節点$x_i$は他に提携する頂点が存在しないため1頂点からなる提携をなし，社会効用を$1$増やす形はとらない．図\ref{fig:f_iso}に$k=1$かつ$S(B)\neq\emptyset$，または$k>2$(otherwise)のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
Consider the difference between the coalition structure in $G[\{c_p\}\cup R(B)\bigcup_{j=1}^{i} V_{c_j}]$ and 
the one in $G[\{c_p\}\cup R(B)\bigcup_{j=1}^{i-1} V_{c_j}]$. 
First, when $k=0$, the cut node $c_i$ in $G[V_{c_i}]$ is not in the same coalition with any vertex in $B$. 

When $k\ge 1$, the cut node $c_i$ in $G[V_{c_i}]$ belongs to either a coalition containing a vertex in $B$ ($g^*(c_i,\iso)$) or not ($g^*(c_i,\fin)$). Thus, we take the maximum one.
Suppose that $k=1$ and $R(B)=\emptyset$. We have two choices: $c_i$ is a singleton or $c_i$ belongs to a coalition containing only vertices in $V_{c_i}$.
On the other hand, consider the case when $k\ge 2$ or $R(B)\neq \emptyset$. Then if $c_i$ belongs to a coalition with vertices in $B$, its coalition forms a clique of size at least $2$. Thus the utilitarian welfare will increase by $1$. 
%Figure\ref{fig:f_iso} shows the transition when $k=1$ and $R(B)\neq\emptyset$ or $k>2$(otherwise).
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_iso.jpg}
%\caption{The transition when $\typeB=\iso$ ($k=1$ \& $S(B)\neq\emptyset$, or When $k>2$).} \label{fig:f_iso}
%\end{figure}


%\paragraph{When $\typeB=\cl$}\
\paragraph{Case $\typeB=\cl$}\

We define the recurrence relation for $\typeB=\cl$ as follows.
\begin{align*}
f(B,\cl,i,k)=&
\begin{cases}
f(B,\cl,i-1,0)+g^*(c_i,\fin)
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B,\cl,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
f(B,\cl,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise}
\end{cases}
\end{align*}
%$G[\{x\}\cup R\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup R\cup \bigcup_{j=1}^{i-1} V_{x_j}]$の提携構造の差分を考える．まず$k=0$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．ただし，$f(B_x,\cl,|\textrm{Child}_{\cT}(B_x)|,k)$は，$k=0$かつ$R=\emptyset$のとき，$x$がサイズ2以上のクリークになり得ないので，$R=\emptyset$であれば$f(B_x,\cl,|\textrm{Child}_{\cT}(B_x)|,0)=-\infty$とする．
%$k>0$に対しては，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．この際，$x_i$が$B_x$内の頂点と同じ提携に入るならば$x$及び他の関節点あるいは$R$の点とクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．
In a valid case, we define $f(B,\cl,|\textrm{Child}_{\cT}(B)|,0)=-\infty$ if  $R(B)=\emptyset$ since $c_p$ cannot be a clique of size at least 2. 

The reason why the above equation holds is as follows: 
We consider the difference between the coalition structures in $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i} V_{c_j}]$ and $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i-1} V_{c_j}]$. 
When $k=0$, the cut node $c_i$ in $G[V_{c_i}]$ is not in the same coalition with any vertex in $B$. 


When $k\ge 1$, the cut node $c_i$ in $G[V_{c_i}]$ belongs to either a coalition containing a vertex in $B$ ($g^*(c_i,\iso)$) or not ($g^*(c_i,\fin)$). In the former case, $c_i$ joins a coalition that forms a clique in $B$. Thus the utilitarian welfare will increase by $1$. 
The latter case is that $c_i$ belongs to a coalition containing only vertices in $V_{c_i}$.
Thus, the utilitarian welfare can be computed by adding the coalition structure in $G[V_{c_i}]$.


% When $k\ge 1$, since the cut node $c_i$ in $G[V_{c_i}]$ can either be in the same coalition as a vertex in $B$ ($g^*(c_i,\iso)$) or not ($g^*(c_i,\fin)$), the one with not smaller utilitarian welfare will be adopted. In this case, if $c_i$ is in the same coalition with some vertices in $B$, it will form a clique with $c_p$ and other cut nodes or vertices in $R(B)$, and the utilitarian welfare of the relevant part is increased by $1$. %Figure\ref{fig:f_cl} shows the transition when $k\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_cl.jpg}
%\caption{The transition when $\typeB=\cl$($k\neq0$(otherwise))} \label{fig:f_cl}
%\end{figure}


\paragraph{Case $\typeB=\stc$}\

We define the recurrence relation for $\typeB=\stc$ as follows.

%\begin{align*}
%&f(B,\stc,i,k)\\
%&=
%\begin{cases}
%f(B,\stc,i-1,0)+g^*(c_i,\fin)%c_iはisoでない
%& \text{if $k = 0$}\\
%\max\left\{
%\begin{array}{c}
%f(B,\stc,i-1,1)+g^*(c_i,\iso),\\%c_iはiso
%f(B,\iso,i-1,2)+g^*(c_i,\fin)%c_iはisoでない
%\end{array}
%\right\}
%& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
%& \text{if $k=1$ \& $|R(B)|=1$}\\
%\max\left\{
%\begin{array}{c}
%f(B,\stc,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
%f(B,\stc,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
%\end{array}
%\right\}
%& \text{otherwise}
%\end{cases}
%\end{align*}

\begin{align*}
&f(B,\stc,i,k)\\
&=
\begin{cases}
f(B,\stc,i-1,0)+g^*(c_i,\fin)%c_iはisoでない
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B,\stc,i-1,0)+g^*(c_i,\iso),\\%c_iはiso
f(B,\stc,i-1,1)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
%& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
& \text{if $k=1$ \& $|R(B)|=1$}\\
\max\left\{
\begin{array}{c}
f(B,\stc,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
f(B,\stc,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise}
\end{cases}
\end{align*}

% \begin{align*}
% &f(B,\stc,i,k)\\
% &=
% \begin{cases}
% f(B,\stc,i-1,0)+g^*(c_i,\fin)%c_iはisoでない
% & \text{if $k = 0$}\\
% \max\left\{
% \begin{array}{c}
% f(B,\stc,i-1,1)+g^*(c_i,\iso),\\%c_iはiso
% f(B,\iso,i-1,2)+g^*(c_i,\fin)%c_iはisoでない
% \end{array}
% \right\}
% %& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
% & \text{if $k\neq 0$ \& $k+|R(B)|=2$}\\
% \max\left\{
% \begin{array}{c}
% f(B,\stc,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
% f(B,\stc,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
% \end{array}
% \right\}
% & \text{otherwise}
% \end{cases}
% \end{align*}




%となる．このようになる理由は次の通りである：
%$G[\{x\}\cup R\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup R\cup \bigcup_{j=1}^{i-1}V_{x_j}]$の提携構造の差分を考える．$k=0$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．ただし，$f(B_x,\stc,|\textrm{Child}_{\cT}(B_x)|,k)$は，$k=0$かつ$R=\emptyset$のとき$x$がスターの中心点になり得ないので，$R=\emptyset$であれば$f(B_x,\stc,|\textrm{Child}_{\cT}(B_x)|,0)=-\infty$とする．

As an invalid case, we define $f(B,\stc,|\textrm{Child}_{\cT}(B)|,0)=-\infty$ if $R(B)=\emptyset$, since $c_p$ cannot be the center of a star.

The reason why the above equation holds is as follows. 
We consider the difference between the coalition structures in $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i} V_{c_j}]$ and $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i-1}V_{c_j}]$. 
When $k=0$, the cut node $c_i$ in $G[V_{c_i}]$ is not in the same coalition with any vertex in $B$. 


%$k>0$に対しては，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$でないとき，$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$）を考える．$f(B_x,\stc,i,k)$を実現する提携構造で$x$を中心点とするスターの葉となっている頂点を$s_i$とすると，$s_i=x_i$の場合と$s_i=s_{i-1}$の場合が考えられるが，いずれの場合も$x$は$x_i$もしくは$s_{i-1}$を中心点とするサイズ2のスターを形成し，$s_i$以外の関節点及び$R$の点はクリークをなす形で提携するため，社会効用は等しくなる．また，$s_i$以外の関節点及び$R$の点はクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$ならば役割が$\iso$である$\textrm{Child}_{\cT}(B_x)$に属する2頂点のうち1点が$x$とスターを形成し，もう1点は1頂点からなる提携を形成するので，社会効用を$1$増やす形はとらない．図\ref{fig:f_stc}に$k>0$で$k=2$かつ$R=\emptyset$以外(otherwise)のときの遷移の様子を示す．
When $k\ge 1$, $c_i$ is either in the same coalition with vertices in $B$ ($g^*(c_i,\iso)$) or not ($g^*(c_i,\fin)$). 
Consider the case where $c_i$ joins the same coalition with vertices in $B$ when $k+|R(B)|\neq2$. 
%$k\neq1$ or $|R(B)|\neq1$, or $k\neq2$ or $R(B)\neq\emptyset$. 
In this case, $c_p$ forms a clique of size $2$ with some cut vertex in $B$ or a vertex in $R(B)$ and other vertices in $B$ form a clique in an optimal coalition structure. Thus, the utilitarian welfare increases by $g^*(c_i,\iso)+1$ if $c_i$ joins a coalition in $B$.
Moreover, 
if $k=2$ and $R(B)=\emptyset$,
$c_p$ forms a star of size 2 with a vertex in $B$ and the other vertex in $B$ forms a singleton.
Thus, the utilitarian welfare also increases by $g^*(c_i,\iso)+1$ if $c_i$ joins a coalition in $B$.


% Let $l$ be the unique leaf in $B$ of the star with center $c_p$ realizing $f(B,\stc,i,k)$. Then there are two possible cases: $l=c_i$ or not. 
% In both cases, $c_p$ forms a star of size 2 with $c_i$ or $s_{i-1}$ as the center point, and the cut nodes except $s_i$ and the vertices in $R(B)$ form a clique, so the utilitarian welfare are equal. In addition, since the cut nodes except $s_i$ and the vertices in $R(B)$ form a clique, the utilitarian welfare of the relevant part is increased by $1$. 
If $k=1$ and $|R(B)|=1$, $c_p$ forms a star of size 2 with the vertex in $R(B)$ and the cut vertex in $B$ forms a singleton in an optimal coalition structure.
By the definition of $f$ in the base case, the utilitarian welfare of the star is already accounted for. 

%ne of the two vertices belonging to $\textrm{Child}_{\cT}(B)$ whose role is $\iso$ forms a star with $c_p$ and the other vertex forms a singleton. Thus the utilitarian welfare increases by $1$. 


%Figure\ref{fig:f_stc} shows the transition when $k>0$, $k\neq1$ or $|R(B_x)|\neq1$, or $k\neq2$ or $R(B_x)\neq\emptyset$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_stc.jpg}
%\caption{The transition when $\typeB=\stc$(without $k>0$ \& $k\neq1$ or $|R|\neq1$, or $k\neq2$ or $R\neq\emptyset$))} \label{fig:f_stc}
%\end{figure}


%\paragraph{When $\typeB=\stl$}\
\paragraph{Case $\typeB=\stl$}\

We define the recurrence relation for $\typeB=\stl$ as follows.
%\begin{align*}
%&f(B,\stl,i,k)\\
%&=
%\begin{cases}
%f(B,\stl,i-1,0)+g^*(c_i,\fin)
%& \text{if $k = 0$}\\
%\max\left\{
%\begin{array}{c}
%f(B,\stl,i-1,1)+g^*(c_i,\iso),\\%c_iはiso
%f(B,\iso,i-1,2)+g^*(c_i,\fin)%c_iはisoでない
%\end{array}
%\right\}
%& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
%& \text{if $k=1$ \& $|R(B)|=1$}\\
%\max\left\{
%\begin{array}{c}
%f(B,\stl,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
%f(B,\stl,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
%\end{array}
%\right\}
%& \text{otherwise.}
%\end{cases}
%\end{align*}
\begin{align*}
&f(B,\stl,i,k)\\
&=
\begin{cases}
f(B,\stl,i-1,0)+g^*(c_i,\fin)
& \text{if $k = 0$}\\
\max\left\{
\begin{array}{c}
f(B,\stl,i-1,0)+g^*(c_i,\iso),\\%c_iはiso
f(B,\stl,i-1,1)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
%& \text{if $k = 1$ \& $|R(B_x)|=1$ or $k = 2$ \& $R(B_x)=\emptyset$}\\
& \text{if $k=1$ \& $|R(B)|=1$}\\
\max\left\{
\begin{array}{c}
f(B,\stl,i-1,k-1)+g^*(c_i,\iso)+1,\\%c_iはiso
f(B,\stl,i-1,k)+g^*(c_i,\fin)%c_iはisoでない
\end{array}
\right\}
& \text{otherwise.}
\end{cases}
\end{align*}

As an invalid case, we deifne $f(B,\stl,|\textrm{Child}_{\cT}(B)|,0)=-\infty$ if $R(B)=\emptyset$, since $c_p$ cannot be a leaf of a star. 
%となる．このようになる理由は次の通りである：$G[\{x\}\cup R\cup \bigcup_{j=1}^{i} V_{x_j}]$と$G[\{x\}\cup R\cup \bigcup_{j=1}^{i-1}V_{x_j}]$の提携構造の差分を考える．$k=0$かつ $R\neq \emptyset$のときは$G[V_{x_i}]$の関節点$x_i$は$B_x$内のどの頂点とも同じ提携に入らないことを表している．ただし，$f(B_x,\stl,|\textrm{Child}_{\cT}(B_x)|,k)$は，$k=0$かつ$R=\emptyset$のとき，$x$がスターの葉になり得ないので，$f(B_x,\stl,|\textrm{Child}_{\cT}(B_x)|,0)=-\infty$とする．

The reason why the above equation holds is as follows.
%We consider the difference between the coalition structures in $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i} V_{c_j}]$ and $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i-1}V_{c_j}]$. 
When $k=0$, the cut node $c_i$ in $G[V_{c_i}]$ is not in the same coalition with any vertex in $B$. 


%$k>0$のとき，$f(B_x,\stl,i,k)$を実現する提携構造において，$x$は$\textrm{Child}_{\cT}(B_x)$に属する頂点のうち役割が$\iso$である頂点あるいは$R$に属する頂点を中心点としたサイズ2のスターを形成している．$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），入らない場合($g^*(x_i,\fin)$)のいずれかの形をとるため，総効用の小さくない方を採用する形となる．この際，$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$でなく，$G[V_{x_i}]$の関節点$x_i$が$B_x$内の頂点と同じ提携に入る場合（$g^*(x_i,\iso)$），関節点$x_i$は$x$とスターを形成するあるいは他の関節点及び$R$の点とクリークをなす形で提携するため，その分の社会効用として$1$増加する形をとる．$k=1$かつ$|R|=1$または$k=2$かつ$R=\emptyset$ならば，関節点$x_i$は他に提携を組む頂点が存在しないため1頂点からなる提携をなし，社会効用を$1$増やす形はとらない．$\typeB=\stl$のときの遷移の様子は，図\ref{fig:f_stc}で示した$\typeB=\stc$のときの遷移の様子と同様である．
When $k\ge 1$, in  a coalition structure realizing $f(B,\stl,i,k)$, $c_p$ forms a star of size 2 with a vertex in $\textrm{Child}_{\cT}(B)$ whose role is $\iso$ or a vertex in $R(B)$ that becomes the center of the star. 
By similar reasons to the case of $\typeB=\stc$, the correctness of the recurrence relations follows.



% In this case, if $k+|R(B)|\neq2$, 
% and cut node $c_i$ in $G[V_{c_i}]$ is not in the same coalition with vertices in $B$ ($g^*(c_i,\iso)$), $c_i$ forms a star with $c_p$ or a clique with another cut nodes and vertices in $R(B)$, and thus its utilitarian utility is increased by $1$.
% If $k=1$ and $|R(B)|=1$ or $k=2$ and $R(B)=\emptyset$, there is no other vertices with which $c_i$ form a coalition, so $c_i$ forms a coalition consisting of one vertex and the utilitarian welfare of the relevant part is not increased by $1$. 


\medskip

\noindent \textbf{[Case (2): Exactly one cut vertex in $\textrm{Child}_{\cT}(B)$ takes the role $\stcu_{\ell}$.]}

%次に，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点が1つ存在する場合について考える．まず，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点とその葉となる$B_x$内の頂点を決め打つ．ここで，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点は，葉として$B_x$内からは1頂点のみをとる．よって，$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点とその葉となる$B_x$内の頂点の組は高々$\Delta^2$通りである．$\stcu$である$\textrm{Child}_{\cT}(B_x)$内の頂点を$c_{\textrm{center}}$，$c_{\textrm{center}}$の葉となる$B_x$内の頂点を$v_l$として，補助関数$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$を定義する．$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$は，$c_{\textrm{center}}$と$v_l$を決め打ちしたとき，$G[V(B_x)]$の提携構造のうち以下の条件を満たすものの最大社会効用を表す：
Next, we consider Case (2). Fix a cut vertex $c_{\textrm{center}}$ in $\textrm{Child}_{\cT}(B)$ whose role is $\stcu_\ell$, that is, the center of a star having the unique leaf $v_{\textrm{leaf}}$ in $B$. 
The number of  choices of such pairs is at most $\Delta^2$.
% Note that, there are at most $\Delta^2$ pairs of vertices in $\textrm{Child}_{\cT}(B)$ in which the role of one node is $\stcu$ and the other node becomes its leaves since the node in $\textrm{Child}_{\cT}(B)$ whose role is $\stcu$ takes only one vertex from $B$ as a leaf. 
%Let $c_{\textrm{center}}$ be a cut vertex in $\textrm{Child}_{\cT}(B)$ whose role is $\stcu_\ell$ and let $v_{\textrm{leaf}}$ be the unique leaf in $B$ of the star with the center $c_{\textrm{center}}$. 

Then  we define $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)$ as the maximum utilitarian welfare  in $G[\{c_p\}\cup R(B)\cup \bigcup_{j=1}^{i} V_{c_j}]$ that satisfies the following conditions:
%(i) $x$のタイプが$\typeB$,
%(ii) $c_{\textrm{center}}$のタイプが$\stcu$，かつ$c_{\textrm{center}}$は$v_l$を葉にもつ,
%(iii) $x_1, x_2, \ldots, x_{|\textrm{Child}_{\cT}(B_x)|}\in \textrm{Child}_{\cT}(B_x)$について，$c_{\textrm{center}}=x'_1$とし，残りの頂点を$v_l\in S(B_x)\cup\{x\}$であればラベルの昇順に$x'_2,\ldots, x'_{|\textrm{Child}_{\cT}(B_x)|}$，$v_l\in \textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$であれば$v_l=x'_2$としたのち残りの頂点をラベルの昇順に$x'_3,\ldots, x'_{|\textrm{Child}_{\cT}(B_x)|}$としたとき，$x'_1,x'_2,\ldots, x'_i \in \textrm{Child}_{\cT}(B_x)$のうちちょうど$k$個が各部分木内の頂点とは提携を形成しない，かつその他のちょうど$i-k$個の関節点は\underline{各部分木内の点を含み}提携を形成している．
\begin{itemize}
    \item $c_p$ is the parent cut node of $B$ and the role of $c_p$ is $\typeB\in \{\iso, \cl, \stc,\stl\}$.
    \item The role of $c_{\textrm{center}}$ is $\stcu_\ell$ and $v_{\textrm{leaf}}$ belongs to $c_{\textrm{center}}$'s coalition  as a leaf. 
%    \item For $c_1, c_2, \ldots, c_{|\textrm{Child}_{\cT}(B_x)|}\in \textrm{Child}_{\cT}(B)$, let $c_{\textrm{center}}=c'_1$, and if $v_{\textrm{leaf}}\in R(B)\cup\{c_p\}$, let the remaining nodes be $c'_2,\ldots, c'_{|\textrm{Child}_{\cT}(B_x)|}$ in ascending order of label, and if $v_{\textrm{leaf}}\in \textrm{Child}_{\cT}(B)\setminus\{c_{\textrm{center}}\}$, let $v_{\textrm{leaf}}=c'_2$ and the remaining nodes be $c'_3,\ldots, c'_{|\textrm{Child}_{\cT}(B)|}$ in ascending order of label. Then there are exactly $k$ cut vertices in $c'_1,c'_2,\ldots, c'_i \in \textrm{Child}_{\cT}(B)$ whose coalitions contain no vertex in $V_{c_i}\setminus \{c_{i}\}$ for $1\le i\le k$.
%\item There are exactly $k$ cut vertices among $c_1,c_2,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ whose coalitions contain no vertex in $V_{c_j}\setminus \{c_{j}\}$ for $1\le j\le i$.
%\item There are exactly $k$ cut vertices among $c_1,c_2,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ whose coalitions contain no vertices in $V_{c_j}\setminus \{c_{j}\}$.

%  \item There are exactly $k$ cut vertices among $c_1, c_2, \ldots, c_i\in \textrm{Child}_{\cT}(B)$ such that each of $k$ cut vertices does not form the coalition with vertices in its subtree, and each of $i-k-1$ other cut vertices among $c_1, c_2, \ldots, c_i\in \textrm{Child}_{\cT}(B)$ forms a coalition with only vertices in its subtree. 

% %%%%
% \item The coalitions that the $i$ cut vertices $c_1,c_2,\ldots, c_i$ belong to form as follows: one of them, say $c_1$ without loss of generality, belongs to a star coalition and is the center, exactly $i-k-1$ cut vertices form their coalitions with vertices in their subtrees, and the remaining $k$ cut vertices form coalitions with vertices in $B$.

\item The coalitions that the $i$ cut vertices $c_1,c_2,\ldots, c_i$ belong to form as follows: $c_1 = c_{\textrm{center}}$, that is, it belongs to a star coalition and is the center, exactly $i-k-1$ cut vertices form their coalitions with vertices in their subtrees, and each of the remaining $k$ cut vertices does not form the coalition with vertices in its subtree.

\item If $v_{\textrm{leaf}}\in \textrm{Child}_{\cT}(B)$, $c_2 = v_{\textrm{leaf}}$.
\end{itemize}
%図\ref{fig:f_center}に$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$のイメージを示す．
%Figure\ref{fig:f_center} shows the image of $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{f_center.jpg}
%\caption{The image of $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$} \label{fig:f_center}
%\end{figure}


%ただし，$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$については，$v_l\in S(B_x)$であれば，最初に$c_{\textrm{center}}$と$v_l$をセットして，その後$G[V_{B_x}\setminus V_{c_{\textrm{center}}}\setminus\{v_l\}]$について$\textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$の頂点のうち$k$個が$\textrm{Child}_{\cT}(x'_j)$内の頂点と提携を形成しないときの社会効用の最大値を$f(B_x,\typeB,i,k)$の計算と同様の方針で計算する．また，$v_l\in \textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$であれば，方針は同様であるが$v_l$のタイプが$\iso$となるので，$\textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}},v_l\}$の頂点のうち$k-1$個が$\textrm{Child}_{\cT}(x'_j)$内の頂点と提携を形成しないときの社会効用の最大値を計算することに注意する．以下では，$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$を動的計画法で計算する．
%However, for $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$, if $v_l\in S(B_x)$, we first set $c_{\textrm{center}}$ and $v_l$, and then compute the maximum social welfare in $G[V_{B_x}\setminus V_{c_{\textrm{center}}}\setminus\{v_l\}]$ when $k$ nodes in $\textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$ do not form coalitions with the vertices in $\textrm{Child}_{\cT}(x'_j)$. This computation can be done in same way as computing $f(B_x,\typeB,i,k)$. If $v_l\in \textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$, the policy is the same, but since the type of $v_l$ is $\iso$, note that we compute the maximum social welfare when $k-1$ nodes in $\textrm{Child}_{\cT}(x'_j)$ do not form coalitions with vertices in $\textrm{Child}_{\cT}(x'_j)$.In the following, we  compute $f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$ by dynamic programming.

%$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$は$f(B_x,\typeB,i,k)$と同様の方針で再帰的に計算できる．$x'_1=c_{\textrm{center}}$を$B_x$内の頂点を葉に持つスターの中心点，$v_l$を$c_{\textrm{center}}$が持つ$B_x$内の葉であると決め打ちしているので，$G[V_{c_{\textrm{center}}}\cup\{v_l\}]$部分の社会効用として，
%\begin{align*}
%g^*(c_{\textrm{center}},\stcu)&=\max_l\{g^*(c_{\textrm{center}},\stcu_l)\}\\
%&=\max_l\left\{g^*(c_{\textrm{center}},\stc_l)+\frac{2}{(l+1)(l+2)}\right\}
%\end{align*}
%を計算する．
%%%%%%%%%%土中先生が直してくださったver.%%%%%%%%%%%%%%%%%%%%%%%%
%Without loss of generality, let $c_1 = c_\textrm{center}$ and $c_2 = c_\textrm{leaf}$.
%% For $c_1, c_2, \ldots, c_{|\textrm{Child}_{\cT}(B_x)|}\in \textrm{Child}_{\cT}(B)$, let $c_{\textrm{center}}=c'_1$, and if $v_{\textrm{leaf}}\in R(B)\cup\{c_p\}$, let the remaining nodes be $c'_2,\ldots, c'_{|\textrm{Child}_{\cT}(B_x)|}$ in ascending order of label, and if $v_{\textrm{leaf}}\in \textrm{Child}_{\cT}(B)\setminus\{c_{\textrm{center}}\}$, let $v_{\textrm{leaf}}=c'_2$ and the remaining nodes be $c'_3,\ldots, c'_{|\textrm{Child}_{\cT}(B)|}$ in ascending order of label. 
%Note that in the recurrence relation, if $v_{\textrm{leaf}}\in R(B)\cup\{c_p\}$, we assume as initialization that $c'_1=c_{\textrm{center}}$ is the center of the star which contains a vertex in $B$ as a leaf.
%Then we recursively compute the maximum utilitarian welfare when exact $k$ cut vertices among $c_2,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ do not form coalitions with vertices in $V_{c_j}\setminus\{c_j\}$ and exactly $i-k-1$ other cut vertices in $c_2,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ form coalitions only with vertices in $V_{c_j}\setminus \{c_j\}$.
%On the other hand, if $v_{\textrm{leaf}}\in \textrm{Child}_{\cT}(B)\setminus\{c_{\textrm{center}}\}$, the role of $c_1=c_{\textrm{center}}$ is determined as $\stcu_\ell$ and the role of $c_2=v_{\textrm{leaf}}$ as $\iso$ as initialization, then in dynamic programming we compute the maximum utilitarian welfare when $k-1$ vertices among $c_3,\ldots,c_i \in \textrm{Child}_{\cT}(B)$ do not form coalitions with vertices in $V_{c_j}\setminus\{c_j\}$ and exactly $i-k-1$ other cut vertices in $c_3,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ form coalitions only with vertices in $V_{c_j}\setminus \{c_j\}$.


\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%l.509~520の書き直し(0704)%%%%%%%%%%%%%%%%%%%%%%%%
There are two cases that $v_{\textrm{leaf}}\in R(B)\cup\{c_p\}$ and $v_{\textrm{leaf}}\in \textrm{Child}_{\cT}(B)\setminus\{c_{\textrm{center}}\}$.
Without loss of generality, let $c_1 = c_\textrm{center}$.
In the former case, to compute $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)$, we consider the maximum utilitarian welfare when exact $k$ cut vertices among $c_2,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ do not form coalitions with vertices in $V_{c_j}\setminus\{c_j\}$ and exactly $i-k-1$ other cut vertices in $c_2,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ form coalitions only with vertices in $V_{c_j}\setminus \{c_j\}$ .
In the latter case, let $c_2 = v_\textrm{leaf}$ without loss of generality. Then since the role of $c_2$ is $\iso$ as initialization, we compute the maximum utilitarian welfare when $k-1$ vertices among $c_3,\ldots,c_i \in \textrm{Child}_{\cT}(B)$ do not form coalitions with vertices in $V_{c_j}\setminus\{c_j\}$ and exactly $i-k-1$ other cut vertices in $c_3,\ldots, c_i \in \textrm{Child}_{\cT}(B)$ form coalitions only with vertices in $V_{c_j}\setminus \{c_j\}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

Function $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)$ can be calculated recursively in the same way as $f(B,\typeB,i,k)$. 
%Since we fix $c'_1=c_{\textrm{center}}$ as the center of the star whose leaves have vertices in $B$ and $v_{\textrm{leaf}}\in B$ as the leaf that $c_{\textrm{center}}$ has, 
The maximum utilitarian welfare in $G[V_{c_{\textrm{center}}}\cup\{v_{\textrm{leaf}}\}]$ is
\begin{align*}
g^*(c_{\textrm{center}},\stcu)&=\max_\ell\{g^*(c_{\textrm{center}},\stcu_\ell)\}\\
&=\max_\ell\left\{g^*(c_{\textrm{center}},\stc_\ell)+\frac{2}{(\ell+1)(\ell+2)}\right\}.
\end{align*}
%そして，漸化式においては，$v_l\in R(B_x)\cup\{x\}$であれば，初期化として$x'_1=c_{\textrm{center}}$は$B_x$内の頂点を葉に持つスターの中心点であると決め打ちして，その後$x'_2,\ldots, x'_i \in \textrm{Child}_{\cT}(B_x)$うち$V_{x_j}\setminus\{x_j\}$の頂点とは提携を形成しない頂点が$k$個のときの社会効用の最大値を再帰的に計算する．一方，$v_l\in \textrm{Child}_{\cT}(B_x)\setminus\{c_{\textrm{center}}\}$であれば，初期化として$x'_1=c_{\textrm{center}}$の役割を$\stcu$，$x'_2=v_l$の役割を$\iso$と決め打つので，その後の動的計画法では$x'_3,\ldots, x'_i \in \textrm{Child}_{\cT}(B_x)$の頂点のうち$k-1$個が$\mathcal{T}_{x'_j}$のノードに対応する頂点とは提携を形成しないときの社会効用の最大値を計算することに注意する．図\ref{fig:f_center}に$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$のイメージを示す．
 %Figure\ref{fig:f_center} shows the image of $f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$.
%また，$f(B_x,\typeB,i,k)$の計算と同様に，$x$の役割である$\typeB$によって$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$を求める漸化式も異なる．特に，$\typeB\in\{\iso,\cl,\stl\}$のときは$v_l=x$であれば$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)=-\infty$となる．



As with the computation of $f(B,\typeB,i,k)$, the recurrence relations computing $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)$ also differ depending on $\typeB$. In particular, when $\typeB\in\{\iso,\cl,\stl\}$, $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)=-\infty$ if $v_{\textrm{leaf}}=c_p$.
%さらに，$f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)\}$とすると，各$c_{\textrm{center}}$に対する社会効用の最大値は，$f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$で表すことができる．
%Furthermore, let $f_{c_{\textrm{center}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)\\=\max_{v_{\textrm{leaf}}\in B\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)\}$, the maximum utilitarian welfare for each $c_{\textrm{center}}$ can be expressed by $f_{c_{\textrm{center}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$.
Furthermore, let $f_{c_{\textrm{center}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)=\max_{v_{\textrm{leaf}}\in B\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,\\ |\textrm{Child}_{\cT}(B)|,k)\}$, 
it represents the maximum utilitarian welfare for each $c_{\textrm{center}}$.
%$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$の計算方針は$f(B_x,\typeB,i,k)$の計算方針とほぼ同様なので，以降では，$f(B_x,\typeB,i,k)$を再帰的に計算する方法を示す．
Since $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)$ can compute in almost same way as $f(B,\typeB,i,k)$, we omit the details.

%よって，$f^*(B_x,\typeB,k)$は，
Therefore, we have 
\begin{align*}
&f^*(B,\typeB,k)\\
&=\max\{f(B,\typeB,|\textrm{Child}_{\cT}(B)|,k),f_{c_1}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k),\\
&\ldots,f_{c_{|\textrm{Child}_{\cT}(B)|}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)\}. 
\end{align*}
%で表される．



\subsubsection{Recurrence relation in the cut nodes}
%$g^*(c,\typec)$を計算するにあたって，補助関数$g(c,\typec,i)$を定義する．$\textrm{Child}_{\cT}(c)$に属する頂点を$B_c^1, B_c^2, \ldots, B_c^{|\textrm{Child}_{\cT}(c)|}$とする．まず$B_c^1, B_c^2, \ldots, B_c^i \in \textrm{Child}_{\cT}(c)$に対して，$g(c,\typec,i)$は，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$における提携構造のうち$c$のタイプが$\typec$であるものの最大効用を表す．また，$l\le i$とする．すると，定義より
To compute $g^*(c,\typec)$, we define an auxiliary function $g(c,\typec,i)$. 
%Let $B_c^1, B_c^2, \ldots, B_c^{|C_{cT}(c)|}$ be the nodes belonging to $\textrm{Child}_{\cT}(c)$. First, for $B_c^1, B_c^2, \ldots, B_c^i \in \textrm{Child}_{\cT}(c)$, $g(c,\typec,i)$ is the maximum utilitarian welfare of coalition structures in $G[\bigcup_{j=1}^{i}V_{B_x^j}]$ in which the role of $c$ is $\typec$. Let $l\le i$. By definition, we obtain
Let $B_1, B_2, \ldots, B_{|C_{cT}(c)|}$ be the block nodes belonging to $\textrm{Child}_{\cT}(c)$. First, for $B_1, B_2, \ldots, B_i \in \textrm{Child}_{\cT}(c)$, $g(c,\typec,i)$ is the maximum utilitarian welfare of coalition structures in $G[\bigcup_{j=1}^{i}V_{B_j}]$ in which the role of $c$ is $\typec$. Let $\ell\le i$. By definition, we obtain
\[
g^*(c,\typec) = g(c,\typec,|\textrm{Child}_{\cT}(c)|).
\]
%となる．図\ref{fig:g}に$g(c,\typec,|\textrm{Child}_{\cT}(c)|)$のイメージを示す．
%Figure\ref{fig:g} shows the image of $g(c,\typec,|\textrm{Child}_{\cT}(c)|)$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g.jpg}
%\caption{The image of $g(c,\typec,|\textrm{Child}_{\cT}(c)|)$} \label{fig:g}
%\end{figure}
%以下では，$g(c,\typec,|\textrm{Child}_{\cT}(c)|)$を$i$に関する動的計画法で計算する．
In the following, we compute $g(c,\typec,|\textrm{Child}_{\cT}(c)|)$ by dynamic programming. 


%\paragraph{When $\typec=\iso$}\
\paragraph{Case $\typec=\iso$}\

We define the recurrence relation for $\typeB=\iso$ as follows.
\begin{align*}
g(c,\iso,i)=& \begin{cases}
0 & i = 0 \\
g(c,\iso,i-1)+\max_{k}f^*(B_i,\iso,k)
& i\neq 0.
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\iso,0)=0$とする．$i\neq0$のとき，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$と$G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$の提携構造の差分を考える．このとき，$c$は$B_c^1,\ldots,B_c^i$に対応するいずれのクリークからも同じ提携に入る頂点をとらないので，社会効用を$\max_{k}f^*(B_c^i,\iso,k)$だけ増やす形をとる．図\ref{fig:g_iso}に$i\neq0$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\iso,0)\\=0$. When $i\neq0$, consider the difference between the coalition structures in $G[\bigcup_{j=1}^{i}V_{B_j}]$ and $G[\bigcup_{j=1}^{i-1}V_{B_j}]$. In this case, since $c$ does not take a vertex that forms a coalition together from any of the cliques corresponding to $B_1,\ldots,B_i$, the utilitarian welfare increases by $\max_{k}f^*(B_i,\iso,k)$. 
%Figure\ref{fig:g_iso} shows the transition when $i\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_iso.jpg}
%\caption{The transition when $\typec=\iso$ ($i\neq0$)} \label{fig:g_iso}
%\end{figure}


%\paragraph{When $\typec=\cl$}\
\paragraph{Case $\typec=\cl$}\

We define the recurrence relation for $\typeB=\cl$ as follows.
\begin{align*}
g(c,\cl,i)=& \begin{cases}
0 & i = 0\\
\max_{k}f^*(B_1,\cl,k)& i = 1\\
\max\left\{
\begin{array}{c}
g(c,\cl,i-1)+\max_{k}f^*(B_i,\iso,k),\\
g(c,\iso,i-1)+\max_{k}f^*(B_i,\cl,k)
\end{array}
\right\}
& i>1.
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\cl,0)=0$とする．$i\neq0$のとき，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$と$G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$の提携構造の差分を考える．このとき，$c$はクリークを形成するので$B_c^1,\ldots,B_c^i$に対応するクリークのうち1つからのみ同じ提携に入る頂点をとり，他のクリークノードにおいて$c$の役割は$\iso$となる．よって，$c$がクリークを形成する頂点が$B_c^i$内の頂点である場合とそうでない場合の社会効用を比較し，小さくない方を採用する形となる．図\ref{fig:g_cl}に$i\neq0$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\cl,0)\\=0$. When $i\neq0$, consider the difference between the coalition structures in $G[\bigcup_{j=1}^{i}V_{B_j}]$ and $G[\bigcup_{j=1}^{i-1}V_{B_j}]$. In this case, since $c$ forms a clique, it takes a vertex from only one of the cliques corresponding to $B_1,\ldots,B_i$ into the same coalition, and the role of $c$ in the other clique nodes is $\iso$. Therefore, we compare the utilitarian welfare of the case where $c$ forms a clique with a vertex in $B_i$ and the case where $c$ forms a clique with a vertex not in $B_i$, and adopt the one that is not smaller. %Figure\ref{fig:g_cl} shows the transition when $i\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_cl.jpg}
%\caption{The transition when $\typec=\cl$ ($i\neq0$)} \label{fig:g_cl}
%\end{figure}


%\paragraph{When $\typec=\stc_l$}\
\paragraph{Case $\typec=\stc_\ell$}\

We define the recurrence relation for $\typeB=\stc_\ell$ as follows.
\begin{align*}
g(c,\stc_\ell,i)=& \begin{cases}
0 & i=0\\
\sum_{j=1}^{\ell}{\max_{k}f^*(B_j,\stc,k)}-\frac{(\ell-1)(\ell+2)}{\ell(\ell+1)} & i = \ell\\
\max\left\{
\begin{array}{c}
g(c,\stc_\ell,i-1)+\max_{k}f^*(B_i,\iso,k),\\
g(c,\stc_{\ell-1},i-1)+\max_{k}f^*(B_i,\stc,k)-\frac{(\ell-1)(\ell+2)}{\ell(\ell+1)}
\end{array}
\right\}
& i > \ell.
\end{cases}
\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\stc_l,i)=0$とする．$i=l$であれば，$c$は$B_c^1,\ldots,B_c^l$に対応するクリーク内からスターの葉となる頂点をそれぞれ1つずつとって提携を形成する．この際，サイズ2のスター$l$個の社会効用とサイズ$l+1$のスターの社会効用の差が$\frac{(l-1)(l+2)}{l(l+1)}$であることに注意する．$i>l$のとき，$G[\bigcup_{j=1}^{i}V_{B_x^j}]$と$G[\bigcup_{j=1}^{i-1}V_{B_x^j}]$の提携構造の差分を考える．スターの中心点$c$が$l$個の葉のうちの1点を$B_c^i$内の頂点からとらない場合ととる場合の社会効用を比較し小さくない方を採用する形となる．図\ref{fig:g_stc}に$i>l$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\stc_\ell,i)\\=0$. If $i=\ell$, $c$ forms a star by taking one vertex from each of the cliques corresponding to $B_1,\ldots,B_\ell$ as a star leaf. Note that the difference between the utilitarian welfare of the sum of $\ell$ stars of size 2 and a star of size $\ell+1$ is $\frac{(\ell-1)(\ell+2)}{\ell(\ell+1)}$. When $i>\ell$, consider the difference between the coalition structures in $G[\bigcup_{j=1}^{i}V_{B_j}]$ and $G[\bigcup_{j=1}^{i-1}V_{B_j}]$. Then we compare with the utilitarian welfare of the case where $c$ takes a vertex from $B_i$ as one of its leaves and the case $c$ takes no vertex from $B_i$, and the not smaller of the two is adopted. 
%Figure\ref{fig:g_stc} shows the transition when $i>l$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_stc.jpg}
%\caption{the transition when $\typec=\stc_l$($i>l$)} \label{fig:g_stc}
%\end{figure}



%\paragraph{When $\typec=\stcu_l$}\

%We obtain
%\begin{align*}
%g(c,\stcu_l,i)=& \begin{cases}
%0 & i = 0\\
%g(c,\stc_l,i)+\frac{2}{(l+1)(l+2)}
%& i \neq0.
%\end{cases}
%\end{align*}
%となる．このようになる理由は次の通りである：$i=0$のとき，$g(c,\stcu_l,i)=0$とする．$i\neq0$のとき，$c$が$P_{\cT}(c)$内の頂点から葉をとることからその頂点$v$をとすると，$G[\bigcup_{j=1}^{i}V_{B_x^j}\cup\{v\}]$において$c$を中心点とするスターの葉の数は$l+1$である．$g(c,\stc_l,i)$を実現する提携構造における$c$を中心点とするスターの社会効用が$2l/(l+1)$，葉の数が$l+1$のスターの社会効用が$2(l+1)/(l+2)$であることに注意するとその差分は$2/(l+1)(l+2)$となる．
%The reason why the above equation holds is as follows: When $i=0$, let $g(c,\stcu_l,i)=0$. When $i\neq0$, since $c$ takes a vertex from $P_{\cT}(c)$ as a leaf, let the vertex,be $v$. Then in $G[\bigcup_{j=1}^{i}V_{B_x^j}\cup\{v\}]$, the number of leaves of the star whose center is $c$ is $l+1$. Note that the social welfare of the star whose center is $c$ in the coalition structure realizing $g(c,\stc_l,i)$ is $2l/(l+1)$ and the social welfare of the star with $l+1$ leaves is $2(l+1)/(l+2)$, the difference of which is $2/(l+1)(l+2)$.


%\paragraph{When $\typec=\stl$}\
\paragraph{Case $\typec=\stl$}\

We define the recurrence relation for $\typeB=\stl$ as follows.
\begin{align*}
g(c,\stl,i)=& \begin{cases}
0 & i = 0\\
\max_{k}f^*(B_1,\stl,k) & i = 1\\ 
\max\left\{
\begin{array}{c}
g(c,\stl,i-1)+\max_{k}f^*(B_i,\iso,k),\\
g(c,\iso,i-1)+\max_{k}f^*(B_i,\stl,k)
\end{array}
\right\}
& i>1.
\end{cases}
\end{align*}
%となる．
%このようになる理由は次の通りである：$i=0$のとき$g(c,\stl,0)=0$とする．$i\neq0$のとき，$c$はスターの葉なので，その中心点として$B_c^1,\ldots,B_c^i$に対応するクリークのうち1つからのみ同じ提携に入る頂点をとり，他のクリークノードにおいて$c$の役割は$\iso$となる．よって，$c$が$B_c^i$内の頂点をスターの中心点としない場合とする場合の社会効用を比較し，小さくない方を採用する形となる．図\ref{fig:g_stl}に$i\neq0$のときの遷移の様子を示す．
The reason why the above equation holds is as follows: 
When $i=0$, let $g(c,\stl,0)\\=0$. When $i\neq0$, since $c$ is a leaf of the star, it takes as its center a vertex that enters the same coalition only from one of the cliques corresponding to $B_1,\ldots,B_i$, and the role of $c$ at the other clique nodes is $\iso$. 
Therefore, we compare the utilitarian welfare of the case where $c$ does not take a vertex from $B_i$ as the center of the star and the case where it does, and adopt the one that is not smaller. 
%Figure\ref{fig:g_stl} shows the transition when $i\neq0$.
%\begin{figure}[htb]
%\centering
%\includegraphics[width=\textwidth]{g_stl.jpg}
%\caption{When $\typec=\stl$ ($i\neq0$)} \label{fig:g_stl}
%\end{figure}



\subsubsection{Complexity}
%本アルゴリズムでは，ブロックノードと関節ノードで漸化式が異なるので，それぞれに必要な計算時間を考える．
Since the recurrence relations are different for block nodes and cut nodes in this algorithm, we consider the computation time required for each.

%はじめに，ブロックノードにおける計算時間について考える．ブロックノードでは，$f^*(B_x,\typeB,k)$の値を計算するために，$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$と各$f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$の値を子$i$に関する動的計画法で求める．まず，$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$の計算時間を考える．一つの$B_x,\typeB,i,k$の組に対して$f(B_x,\typeB,i,k)$を求めるのに必要な計算時間は，$O(\Delta)$時間である．よって，すべての$B_x\in\mathcal{B},\typeB\in\texttt{T}_B,k$について$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$を子$i$に関する動的計画法で求める際に必要な計算時間は，
First, we consider the computation time at the block nodes. In a block node, to compute the value of $f^*(B,\typeB,k)$, we compute the values of $f(B,\typeB,\\|\textrm{Child}_{\cT}(B)|,k)$ and each $f_{c_{\textrm{center}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$ by dynamic programming. We consider the computation time of $f(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$. Since the time required to compute the value of $f(B,\typeB,i,k)$ for a single set of $B$, $\typeB$, $i$, and $k$ is $O(\Delta)$, the time required to compute $f(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$ for all $B\in\mathcal{B},\typeB\in\texttt{T}_B$, and $k$ by dynamic programming is
\begin{align*}
O((\text{Number of candidates of}\  B)\cdot4\cdot\Delta^3)= O(n\Delta^3).
\end{align*}
%となり，$O(n\Delta^3)$時間である．
%次に，各$f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$の計算時間について考える．一つの$B_x,\typeB,i,k,c_{\textrm{center}},v_l$の組に対して$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,i,k)$の計算時間は，$f(B_x,\typeB,i,k)$の計算と同様に$O(\Delta)$時間である．また，$c_{\textrm{center}}$と$v_l$の取り方は高々$\Delta^2$通りであるので，すべての$B_x\in\mathcal{B},\typeB\in\texttt{T}_B,c_{\textrm{center}}\in |\textrm{Child}_{\cT}(B_x)|,v_l\in B_x\setminus\{c_{\textrm{center}}\},k$について$f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$を子$i$に関する動的計画法で求める際に必要な計算時間は，
Next, consider the computation time for each $f_{c_{\textrm{center}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$. The time required to compute $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,i,k)$ for a single set of $B$, $\typeB$, $i$, $k$, $c_{\textrm{center}}$, and $v_{\textrm{leaf}}$ is $O(\Delta)$ as in the case of $f(B,\typeB,i,k)$. Also, since there are at most $\Delta^2$ ways to take $c_{\textrm{center}}$ and $v_{\textrm{leaf}}$, the time required to compute $f_{c_{\textrm{center}}}^{v_{\textrm{leaf}}}(B,\typeB,|\textrm{Child}_{\cT}(B)|,k)$ for all $B\in\mathcal{B},\typeB\in\texttt{T}_B,c_{\textrm{center}}\in |\textrm{Child}_{\cT}(B)|, v_{\textrm{leaf}}\in B\setminus\{c_{\textrm{center}}\}$, and $k$ by dynamic programming is
\begin{align*}
O((\text{Number of candidates of} \ B)\cdot4\cdot\Delta^3\cdot\Delta^2)= O(n\Delta^5).
\end{align*}
%となり，$O(n\Delta^5)$時間である．
%さらに，$f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)\}$であり，$f^*(B_x,\typeB,k)$を求めるには，$f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$と各$f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$の最大値をとればよい．よって，ブロックノードにおける全体の計算時間は，$O(n\Delta^7)$となる．
%Furthermore, since $f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)=\max_{v_l\in B_x\setminus\{c_{\textrm{center}}\}}\{f_{c_{\textrm{center}}}^{v_l}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)\}$, we consider the maximum value of $f(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$ and each $f_{c_{\textrm{center}}}(B_x,\typeB,|\textrm{Child}_{\cT}(B_x)|,k)$ to compute $f^*(B_x,\typeB,k)$.
Therefore, the total computation time at the block node is $O(n\Delta^5)$.

%次に，関節ノードにおける計算で必要な計算時間について考える．関節ノードにおける計算では，$g(c,\typec,|\textrm{Child}_{\cT}(c)|)$を子$i$に関する動的計画法で求める．一つの$c,\typec,i$の組に対して$g(c,\typec,i)$のを求めるのに必要な計算時間は，$O(\Delta)$時間である．よって，すべての$c\in\mathcal{C},\typec\in\texttt{T}_c$について$g^*(c,\typec)=g(c,\typec,|\textrm{Child}_{\cT}(c)|)$を子$i$に関する動的計画法で求める際に必要な計算時間は，
Next, we consider the computation time at the cut nodes. In the computation at a cut node, we compute the value of $g(c,\typec,|\textrm{Child}_{\cT}(c)|)$ by dynamic programming. The time required to compute $g(c,\typec,i)$ for a single set of $c,\typec$, and $i$ is $O(\Delta)$. Hence, the time required to compute $g^*(c,\typec)=g(c,\typec,|\textrm{Child}_{\cT}(c)|)$ for all $c\in\mathcal{C}$, and $\typec\in\texttt{T}_c$ by dynamic programming is
\begin{align*}
O((\text{Number of candidates of\ } c)\cdot(2\Delta+3)\cdot\Delta^2)= O(n\Delta^3).
\end{align*}
%となり，$O(n\Delta^3)$時間である．

%ゆえに，本アルゴリズムの計算時間は$O(n\Delta^5)$時間となる．
Therefore, this algorithm returns the maximum utilitarian welfare coalition structure in time $O(n\Delta^5)$ and Theorem \ref{thm:block:sw:opt} holds.

%\begin{theorem}\label{thm:block:sw:opt}
%\textsc{Utilitarian Welfare Maximization} on unweighted block graphs can be computed in time $O(n\Delta^5)$.
%\end{theorem}

\begin{comment}
\subsection{Egalitarian welfare}
\subsubsection{Characterization of the optimal coalition}
%Next, we show that there is also an optimal coalition structure on egalitarian welfare in which each coalition induces a clique of size 2 or larger or a star.

%はじめに，$C$に橋$e=\{u,v\}$（ただし，$e$を削除して得られる連結成分からなる提携$C_u$，$C_v$の頂点数はともに2以上）が存在するとき，$C$を$C_u$と$C_v$に社会効用を下げることなく分割できることを示す．
%We first show that when there exists a bridge $e=\{u,v\}$ (however, two coalitions $C_u$ and $C_v$ obtained by deleting $e$ contain 2 or more vertices), we can split $C$ into $C_u$ and $C_v$ without decreasing the minimum utility.



\begin{lemma}\label{lem:egal:star}
$C$をブロックグラフからなる提携とする．$C$に$v$のみを関節点として持つサイズ2の極大クリークが存在するとき，それらを$v$を中心点とするスターとして分割しても最小効用が下がることはない．
\end{lemma}

\begin{proof}
$C$において，$v$のみを関節点として持つサイズ2の極大クリークが存在すると仮定する．
$C$における最小効用はサイズ2の極大クリークの$v$でない方の頂点の効用で，その大きさは$1/|C|$である．
唯一の関節点として$v$を持つサイズ2の極大クリーク集合を$v$を中心点とするスターとして分割することを考える．
$C'$を$v$を中心点とするスター，$C^{\prime\prime}_i$を$C\setminus C'$に含まれる各連結成分とする．

はじめに，$C'$内の頂点の効用の変化を考える．
$C'\setminus\{v\}$内の頂点については，分割により隣接頂点数は変化せず，提携サイズが小さくなるので，分割により効用は増加する．
$w\in C'\setminus \{v\}$とすると$v$の効用は，$u(v,C')\ge u(w,C')>u(w,C)=1/|C|$となるので，分割により$v$の効用が$1/|C|$より小さくなることはない．

次に，$C^{\prime\prime}_i$内の頂点の効用の変化を考える．
$C^{\prime\prime}_i$内の頂点のうち$C$において$v$に隣接していないものについては，分割により隣接頂点数は変化せず，提携サイズが小さくなるので，分割により効用は増加する．
$C$において$v$を関節点として含んでいた極大クリーク内の任意の頂点$u$に着目する．
$u(u,C^{\prime\prime}_i)\ge 1/C^{\prime\prime}_i>1/|C|$なので，$C$において$v$を関節点として含んでいた極大クリーク内の任意の頂点も分割により効用が$1/|C|$より小さくなることはない．

よって，$C$に$v$のみを関節点として持つサイズ2の極大クリークが存在するとき，それらを$v$を中心点とするスターとして分割しても最小効用が下がることはない．
\end{proof}

補題\ref{lem:egal:star}を繰り返すことにより，ブロックグラフからなる任意の提携を関節点を1つのみもつ極大クリークはサイズ3以上であるような提携に最小効用を下げることなく分割できるので，以降では，関節点を1つのみもつ極大クリークはサイズ3以上であるような提携を考える．




\begin{lemma}\label{lem:egal:scu:num}
任意の$B$について，$\textrm{Child}_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つであるような最適提携構造が存在する．
\end{lemma}

\begin{proof}
最適提携構造において，スターの中心点で$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするような$\textrm{Child}_{\cT}(B)$に属する頂点が$t(\ge2)$個存在したとする．これらのスターを$S_i (i=1, \ldots, t)$，それぞれの中心点を$c_i (i=1, \ldots, t)$，葉の数を$l_i (i=1, \ldots, t)$とする（$c_1,\ldots,c_t$の役割が$\stcu$であるので，$l_i\ge2$）．
このとき，各スター$S_1,\ldots,S_t$内の最小効用はそれぞれの葉の効用なので，
\begin{align*}
\frac{1}{l_1+1},\frac{1}{l_2+1},\cdots,\frac{1}{l_t+1}\le\frac{1}{3}
\end{align*}
である．
今，$S_1,\ldots,S_t$が葉とする$B$内の頂点がそれぞれ$S_1,\ldots,S_t$から逸脱して1つのクリークになることを考える．
このとき，$S_1,\ldots,S_t$は葉の数が1つずつ少ないスターになり，それぞれを$S'_i (i=1, \ldots, t)$とすると，$S'_1,\ldots,S'_t$内の最小効用は，
\begin{align*}
\frac{1}{l_1},\frac{1}{l_2},\cdots,\frac{1}{l_t}
\end{align*}
となる．よって，各スターにおける逸脱前後の最小効用の差は，任意の$i(=1,\ldots,t)$に対して，
\begin{align*}
\frac{1}{l_i}-\frac{1}{l_i+1}=\frac{1}{l_i(l_i+1)}>0
\end{align*}
で表せる．

一方，$S_1,\ldots,S_t$が葉とする$B$内の頂点がそれぞれ$S_1,\ldots,S_t$から逸脱して形成したクリーク内の最小効用は少なくとも$1/2>1/(l_i+1)$である．

また，もとの最適提携構造における他の提携については最小効用は変化しない．

よって，最適提携構造においてスターの中心点で$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするような$\textrm{Child}_{\cT}(B)$に属する頂点が$t(\ge2)$個存在するとき，その最小効用を下げることなく，$\textrm{Child}_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つであるような最適提携構造にすることができる．

ゆえに，任意の$B$について，$\textrm{Child}_{\cT}(B)$に属するカット頂点でスターの中心点となり，かつ$V_{\textrm{Child}_{\cT}(B)}$内の頂点と$B$内の頂点をともにスターの葉とするものは高々1つであるような最適提携構造が存在する．
\end{proof}
\end{comment}
